Single-GPU GNN Systems: Traps and Pitfalls

The current graph neural network (GNN) systems have established a clear trend of not showing training accuracy results, and directly or indirectly relying on smaller datasets for evaluations majorly. Our in-depth analysis shows that it leads to a chain of pitfalls in the system design and evaluation process, questioning the practicality of many of the proposed system optimizations, and affecting conclusions and lessons learned. We analyze many single-GPU systems and show the fundamental impact of these pitfalls. We further develop hypotheses, recommendations, and evaluation methodologies, and provide future directions. Finally, a new reference system is developed to establish a new line of optimizations rooted in solving the system-design pitfalls efficiently and practically. The proposed design can productively be integrated into prior works, thereby truly advancing the state-of-the-art.

==> tex/arch.tex <==
\section{Tensor and Graph Exchange} \label{sec.science}

Interface design and system integration is the most important aspect of a complex system over which one can develop any custom use cases and optimize the components independently. 
In this section, we discuss the mechanism to allow passing  \textit{tensors} and \textit{graph object(s)} from Python to {\graphpy-GNN} without any workarounds or major dependencies. 



%{\color{red}
\subsection{Tensor Sharing and Independent Kernel} \label{sec.science.auto}

%\noindent \textbf{Requirements.}
%To this end, the proposed solution is based on the understanding that {\graphpy-GNN} has no role in handling the state tensor requirement, as its job is to read input tensors and produce output tensors. Hence we zeroed in on designing a mechanism that can allow sharing of the tensors. We now discuss how to achieve this.
%The high-level requirement is to design an eco-system that must be modular, offer room for innovations, and ensure that it neither introduces performance overhead nor burden us with complex integration work. 
%Hence, we pose a simple question: can tensors be passed to the Kernel as a simple array-like or equivalent structure? If we can answer ``yes'' to this question, then the Kernel module can be made independent of the DL framework allowing graph objects exchanged as per available Python binding capability, and allowing the Kernel module to be shared among various DL frameworks.  

% Based on the observations so far, there is a need to find a way to make Kernel independent of any DL framework, as well as simplify its integration.  
% To fulfill the need, {\graphpy} advocates avoiding the usage of the tensor library, and its memory management in Kernel. However before that, 

%To achieve it, {\graphpy} handles the memory allocation in a framework-specific adapter inside the Workflow in Python that uses DL framework-specific API for tensor allocation. The adapter than would strive to pass the underlying memory address of all the input and output tensors to the Kernel as arguments. The kernel can then perform the computation without worrying about memory management, while the allocated tensor gets deallocated by the framework automatically based on its reference from the computation graph.



\noindent
\textbf{Passing Tensors as NumPy Arrays?} 
DL Frameworks do provide API to convert a tensor to a NumPy array.
%which can easily be passed to Kernel. 
%NumPy array is very well supported by Python binding packages, such as Pybind11~\cite{pybind11}, that makes the underlying pointer and array dimension information available quickly.
However, the resultant NumPy cannot be used in a training loop as it is a deep copy of the tensor. Hence, we cannot pass it to {\graphpy-GNN} as
only the NumPy array copy contains the computed results and not the original tensor. 
%Hence, for all practical purposes, the kernel was never called, and will never be part of the computation graph. Hence, such APIs cannot help us in designing DL framework independent Kernel.



% \subsection{Infrastructure and Interface Design}
% The simple and extensible nature of {\graphpy} centers around innovations in interface design as discussed in detail now. 


% Without good infrastructure, we can only use ad hoc methods such as using bit-mask matrix to achieve sparsity. This is a burden for data scientists. On the other hand, the usage of the dense matrix to store and compute on the sparse layer will cause memory overhead with no performance improvement. 
% Alternately, if we have the infrastructure, the system optimization becomes easy where anyone can customize existing kernels or develop new ones and plug them in without understanding the nuances of DL in the form of \textit{computation graph}, \textit{tensor management}, and \textit{gradient back-propagation} (\cref{sec.background.dl}). 
% Hence, supporting computation graph and tensor management out-of-the-box, and making the {\graphpy-GNN} independent of such complexity  through innovative interfaces design are themselves big contributions. Further, automatically generating them through DSL is  another very important part of the infrastructure.


\subsubsection{DLPack Tensor: Deviation and Simplification}
% In absence of zero-copy tensor-to-NumPy array conversion, we moved on to the tensor conversion APIs that make the tensor inter-operable with any third-party tensor library. 
% This inter-operability is achieved using an intermediate data structure called DLPack tensor~\cite{dlpack}. 
% %to exchange the tensor between the Workflow module and the Kernel module. 
% Our study reveals that the DLPack Tensor is simply a container that does not support any tensor operations. That is why its codebase is a simple header file that contains a declaration of data structure using built-in C++ types and has no other dependency.
% Since, 
We now discuss the \textit{undocumented} DLPack tensors~\cite{dlpack}. DLPack  is an intermediate data structure to achieve re-usability of the internal  memory object of the tensors among DL frameworks that offer APIs to convert framework-specific tensors to-and-fro DLPack tensors.   
%where DL frameworks can convert input tensors to their own tensors when receiving so as to use them in their backend; or can convert their output tensors to DLPack tensors when sending it to other DL frameworks (such as from PyTorch to TensorFlow). 
When a DL framework receives a DLPack tensor, it acquires the tensor ownership, so that it can free the memory based on its scope, such as whether it is a state tensor or not. 
% Hence, the natural question is: do we need to develop a  tensor library in {\graphpy} to use DLPack?

The documentation for DLPack tensors only mentions that it should be ``consumed'' once, while no guidelines exist on how the recipient should consume it, and how to manage this acquired ownership. Further, the examples mandate that the recipient of the DLPack tensor develop an elaborate tensor library to receive the DLPack tensor in Python. This is possibly not a problem for DL frameworks as they have a tensor library, and know how to handle the ownership. But for learners, this mechanism remains out of reach  as we do not want to force writing a tensor library. 
%when developing a {\graphpy-GNN} like module.
%Usage of DLPack tensors requires a specific ``consume'' protocol to be followed because the scope or life of the tensor is determined by the computation graph due to the need of \textit{state tensors}. 
% He ``consume'' protocol transfers the ownership of the tensor when moving tensors among different DL frameworks. 
%This makes tensor memory de-allocation path complex including
%While the tensor inside Kernel needs to be allocated when producing the kernel output, the tensor deallocation path is complex.
%Recall the need for state tensors during back-propagation and can be freed only after that in each epoch. 
%when the tensor can be safely de-allocated, who can de-allocate, and how to de-allocate are not documented by the owners of DLPack tensor~\cite{dlpack}. 

%However, for the average system learner, writing a new tensor library, converting the DLPack tensor to  the internal format using the ``consume'' protocol, and managing the acquired ownership presents a huge learning curve in absence of the required documentation.  Again, an advanced system researcher might be able to figure out these details by looking into the codebase of PyTorch, TensorFlow, etc.; it is not well-suited for system integration for education and research.
% %and who becomes the owner of the tensor after consumption. 
% Secondly, if {Kernel} decides to allocate memory for the kernel output, what protocol it should follow to convert this allocated memory to DLPack tensor, so that {Workflow} can also use the kernels of DL frameworks, such as ReLU on the output of {\graphpy-GNNs}. 

%leave alone how one would implement their own tensor library-- even a bigger problem.
%Therefore, the goal of integrating the {Kernel} module is still complex. 

 % leaving many deserving learners. 
%While tensor library design, conversion of tensors to DLPack tensors, and consumption of DLPack tensors are part of many DL frameworks, we definitely do not want every learner to hack through their way to learn about the protocol as this approach has huge effort. 
%We name it as ``full protocol" 

\noindent \textbf{Half DLPack Protocol: Sharing without Ownership}.
%Despite the issues mentioned in using DLPack protocol, it seems the only option for making {\graphpy-GNN} independent. 
It should be noted that {\graphpy-GNN} computations are fully stateless as it uses input tensors to produce output tensors using its computation logic. And once the computation is over, {\graphpy-GNN} never needs to keep any reference of the tensors. 
{\graphpy-Workflow}, which directly works with DL framework-specific tensors in Python, handles the state requirements. 
Based on this observation, we propose sharing memory and shape of the captive tensor temporarily by {\graphpy-GNN} without acquiring ownership. This is achieved by
{\graphpy-Workflow} that converts the DL specific-tensors to DLPack tensors and passes it directly to {\graphpy-GNN} that does not keep any elaborate tensor library. 
The latter extracts the underlying memory pointer, tensor shape, and size directly from the DLPack tensor object to read and modify the tensor content during computation. 

As {\graphpy} did not follow the ``consume'' protocol, the tensor ownership still remains with the DL framework which can be freed depending on the scope of the tensor. However, {\graphpy-GNN} is not impacted as it contains no references to the tensor after the computation is over.  

%The state requirement though is handled using {\graphpy-Workflow}, which directly works with DL framework-specific tensors in Python to take care of it where DLPack tensor has no role to play.







%Our in-depth study about DLPack tensor interfaces of PyTorch and TensorFlow, points out that  when we convert the DL Framework's tensor to DLPack, the output is actually a Python Capsule. Capsule is an important wrapper mechanism in Python to enable wrapping of arbitrary objects. Using capsule to exchange data between Python and C++ is offered by Pybind11. capsule directly to {\graphpy-GNN} worked, where we can extract the underlying DLPack tensor object, and finally the memory pointer and tensor shape and size which can be read and modified, if needed. Based on this success, Hence, {\graphpy-GNN} API directly accepts DLPack tensor capsule. 





%lets the allocation to be done by one DL framework (using adapter in the Workflow), and directly uses DLPack tensor to pass the memory address from Python and C++. Further, where the {\graphpy-GNN} does not have to provide a Python binding for the DLPack tensor to receive it due to its capsule nature. Internally, Pybind11 provides API to quickly get the underlying memory address, and array dimensions from the capsule object.  
%In a nutshell, the {{\graphpy}-Kernel} module can still be made independent of DL framework and very lightweight using DLPack tensor to exchange tensors in kernel invocation, however it still leaves us to perform the memory management. 
%as Kernel neither allocates memory for tensors nor writes any special handling to receive tensors. Further, the kernel code is fully independent of any tensor library either of general-purpose DL framework, such as libtorch's tensor library nor we need to write our own tensor library as in DGL.  The actual kernel implementation can rely on native C++ pointers to write the results of computation, which can be extracted from the DLPack capsule.
%\noindent \textbf{End-To-End Solution.}
%We rely on DLPack tensor, but we never introduces any new tensor library nor we care about memory management. 

%{\graphpy} follows a different approach, 

\noindent \textbf{The Flow.}
The flow is explained in the critical system integration code of Listing \ref{list-spmm} and \ref{list-pybind} for integration with PyTorch: %Since, {\graphpy-GNN} is an independent module, we do not need to develop our own tensor library. Hence,
the memory allocation for the output tensor is done in {\graphpy-Workflow}(Python code, Line 6), and never inside the {\graphpy-GNN}. 
The output tensor along with other input tensors are then converted to DLPack tensor (Line 8--9) using PyTorch Python API, which returns a Python capsule object and is passed to the gSpMMv API.
After that, a similar boiler-plate code in {\graphpy-GNN} (Listing \ref{list-pybind}) extracts the memory pointer from the DLPack tensor capsule and passes the pointer to its core kernel implementation. %if the proposed half DLPack protocol actually works.
%After a few epochs, memory consumption remained constant. 
%Hence, when the kernels populate the output array during its core computation, the new values are automatically updated in the PyTorch tensor due to the shared reference. 
% Therefore, {\graphpy} can handle tensor operations without depending on their headers. 


\vspace{-6pt}

\begin{lstlisting}[language=Python, caption= {\small The generated system integration code (Python part) in {\graphpy-Workflow}. Tensors are allocated in Python, converted to DLPack tensors, and passed directly to the system API.}, label={list-spmm}]
import graphpy_kernel as gpk
import torch as th
import torch.utils.dlpack
def gp_gSpMMv(g, in_tensor, reduceFn, Forward):
  #Allocate output tensor here and not in Kernel.
  out_tensor = th.zeros(g.get_vcount(), feat_len)
  #Convert to DLTensor
  in_dltensor= in_tensor.get.DLtensor()
  out_dltensor= out_tensor.get.DLtensor()
  gpk.gSpMMv(g, in_dltensor, out_dltensor, reduceFn, Forward) #calls  gSpMMv kernel. 
  return out_tensor 
\end{lstlisting}

\vspace{-6pt}

\begin{lstlisting}[language=c++, caption= {\small The generated system integration code (C++ part) in {\graphpy-GNN} for Python binding and DLPack Tensor handling.}, label={list-pybind}]
PYBIND11_MODULE(kernel, m) {
 m.def("gSpMMv", [](graph_t& g, py::capsule& in_tensor, py::capsule& out_tensor, int reduceFn, int Forward){
  array_t in_array = capsule_to_array(in_tensor);
  array_t out_array= capsule_to_array(out_tensor);
  return invoke_gSpMMv_impl(g, in_array, out_array, reduceFn, Forward);
 });}
\end{lstlisting}

\vspace{-6pt}


The mechanism to pass tensors is almost equivalent to passing tensors as an array-like structure, while off-course using Python capsule.
Thus, the combination of additional code at both ends (Python and C++) simplifies the job of system integration. Since tensor memory is allocated using PyTorch Python API, the whole memory management is still controlled by it, which can de-allocate the memory automatically later, without {\graphpy-GNN's} involvement.

%Our hit and trial approach of passing tensor this way worked, We call this new protocol \textit{Half} because we do not completely follow the DLPack protocol. The validity of this approach lies in achieving similar training accuracy, as well as no memory leak or other invalid memory access errors-- which was confirmed by measuring memory consumption while running various GNNs in \cref{sec.exp} to achieve good accuracy.

\noindent \textbf{APIs for Data Scientists.}
The $gp\_gSpMMv$ (Listing \ref{list-spmm}) is the actual API for data scientists and not the system APIs ($gSpMMv$) of Table~\ref{table-api}. It is these APIs that needed to be called from the forward and the backward of the ``autograd'' class, which then can directly be used inside the model layer definition, such as \textit{GCNConv}. The application developer then can use such layers as if they are using any other model layer to define a model. 




%Hence, users (Python code) of the Kernel API, as well as the Kernel still think that memory for output tensor is managed automatically.  

% DLPack tensor is very simple structure, and does not require huge effort for its Python binding.

%The core ‘scatter-gather’ function implemented based on c++ arrays, which is incompatible with the tensor operations used in graph DL. To solve this challenge, {\graphpy} use the DLPack tensor to fix this gap between tensor operations and the array-based c++ computation.
%As we mentioned above, {\graphpy} uses the c++ array to implement the message-passing schema. However, Python-based tensor operations are widely used in the graph DL area. There is a need for users to figure out how to integrate the Python tensor operation with the C++ array-based computation kernel. 


\noindent \textbf{Reusable {\graphpy-GNN}.} %\label{sec.science.TFsupport}
{\graphpy} can integrate almost any DL framework that offers conversion of its specific tensor to DLPack tensor. Since PyTorch and Tensorflow both offer this, we have validated their integration with {\graphpy}.
Both the Listings and core computation code of {\graphpy} are reusable. We though require a minor change in the import statement of Listing~\ref{list-spmm} to import TensorFlow and not PyTorch, 
%change in Line number 6 of the Python code Listing~\ref{list-spmm} so that tensors can be allocated as per the DL framework, 
which is taken care of by DSL. 
%This also means that anybody can use the two listings or can generate using the provided DSL, implement kernel computation, and can replace the generated binary to achieve plug-and-play {\graphpy-GNN}.



%{\color{red}
%For graph handling, {\graphpy} allows multiple methods to handle the graph exchange.(\cref{sec.multi}) As we mentioned before, {\graphpy} makes the{\graphpy-GNN} module truly independent, which avoids any limitation of any no-tensor data exchange between how Kernel and Workflow. Therefore, {\graphpy} can use any python binding or any object to handle the graph exchange between Kernel and Workflow. 
%}


%Developing a third-party tensor library inside the Kernel module requires huge learning curve as well as introduces an additional burden in terms on memory management for which no guidelines exist. 
% While the tensor inside Kernel needs to be allocated when producing the kernel output, the tensor deallocation path is complex.
% Recall the need of state tensors during back-propagation, and can be freed only after that in each epoch. 
% This requires understanding of the protocol of computation graph including when the DGL tensor can be safely deallocated, and how. 
% Unfortunately, how this deallocation process works, how to implement the compatibility among tensors are not documented by the owners of intermediate compatible tensor~\cite{dlpack}, leave alone how one would implement their own tensor library-- even a bigger problem.
% %Therefore, the goal of integrating the {Kernel} module is still complex. 



%Our limited survey of other works that modified DGL to demonstrate better performance, also relied on CSR/CSC format. We suspect that such researchers may have found that modifying whole DGL Kernel a tedious process when format changes are involved. \td.

%Hence, the lightweight Kernel module in the plug-and-play eco-system of {\graphpy} provides enough space for innovations without the need to spend efforts on graph preparation or in supporting the APIs that are not applicable for deep learning purpose.

%Writing interfaces for a new kernel in DGL is still a complex problem due to involvement of tensor library and memory management. Therefore, in our opinion, DGL is a system, and not necessarily a productive framework suited for systems research and education.


%Avoid introducing overhead is an       i8m9knnu minute 9k, necessary requirement for a system so that the later optimization techniques will not try to minimize that overhead, and rather should focus exclusively on actual system optimization tasks. In other words, when compared against small overhead systems, it is not likely to get misleading benefits. However, 
%In the traditional graph data science domain, Mcsherry et al~\cite{mcsherry2015scalability} point out the introduction of large system overhead, which is then also optimized as part of analytics performance optimization.  Hence, actual performance improvement solely due to better algorithmic implementation remains less. Our experiment measurements (\cref{sec.exp}) show that DGL introduces huge system overheads in the form of a one-time start up cost, and run-time overhead, which is also identified by DGL. Hence, any system that does not use DGL to implement GNNs 




  


% \noindent \textbf{Integration with DL Framework}
%Further, the DL model layer development follows the usual step of the DL framework to implement the layer in Python. Thus, {\graphpy} uses this framework's computation graph automatically.
%It should also be noted that the kernels that are invoked in the backward computation are related to the kernels called in the forward computation. E.g., if an unweighted SpMM kernel is invoked in the forward direction, the backward computation also invokes this unweighted SpMM kernel but on the inverse graph. 
% So, it is the job of  {\graphpy-Workflow} to implement this workflow and call the right set of kernels in forward and backward with the right set of input and output tensors. 
%Each {\graphpy-GNN} also offers $flag$ as part of their APIs (e.g. Table~\ref{table-kernel}) through which {\graphpy-Workflow} can specify if the computation should be done in forward or inverse of the graph. The corresponding implementations are handled in {\graphpy-GNN}. 

% It should be noted that we are able to fully share the Kernel code, while at this moment Workflow code must be rewritten for every DL framework excluding the adapter. Hence, {\graphpy-GNN} becomes fully plug-and-play, and can easily be replaced by a better-optimized Kernel by others.
%We are looking at possible extension of DSL to automatically generate complete Workflow code as well.







% \subsubsection{\graphpy-GNN} \label{sec.kernel}

% % Our aim for this component is to provide the boilerplate code so that it is easy to implement any kernel now or in future with any novel system ideas without spending time on how to write those boilerplate code. 
% Table \ref{table-kernel} shows how {$wrap\_graph$()} API accepts the Numpy arrays for the graph exported from {\graphpy-SM}. It wraps them up in a $g$ structure.
% Hence, all kernel APIs then accept this $g$ object, apart from DLPack tensors for input and output tensors, and other inputs.
% This module contains the boilerplate code for Python binding of the APIs (Listing \ref{list-pybind}), that converts the input and output DLPack tensor to native arrays by extracting the pointer, and finally calls the actual C++ kernel implementation in the back-end.
% Thus remaining job then is to simply implement those kernels without worrying about tensor. 
% For the GPUs, there are a few more steps, that we discuss next in  \cref{sec.extend}, that still follow the similar philosophy.
% % Hence, all kernel APIs then accept this $g$ object, DLPack tensors for input and output tensors, and other inputs, and uses the boilerplate code to call the actual C++/CUDA kernel implementation in the back-end. 
% Also, the boiler-plate code is automatically generated when a system researcher specifies a new kernel that is not supported out-of-the-box from {\graphpy}. 


% The {\graphpy-GNN} provides all the GAS APIs for GNN use-cases using three set of APIs as listed in Table~\ref{table-kernel}. We also provide a choice of reduce function using $eFn$ enumeration type, which may contains values SUM, MIN, MAX, DIV etc. Further, we also provide kernels for sparse layers, which implements traditional sparse linear algebra as we discuss shortly. We also provide other traditional GAS APIs and Kernels such as BFS. 




% The only duplicated effort is on writing the Python code for model, i.e. the data scientists' job. We do not think that data scientists will need to write model code for many frameworks, as they  will write their model code using  their preferred framework.

\subsection{{\graphpy-SM}: Graph Preparation and Exchange} \label{sec.engg}

% Moreover, Numpy array has become the standard way to exchange the data between different Python module using zero-copy mechanism.  Therefore, {\graphpy-SM} is implemented on C++ but exports the prepared graph to users using Numpy arrays. Fig.~\ref{fig-engg} presents an overview, and Table~\ref{table-api} presents the APIs for graph creation, and data access using CSR and COO format.  

% \begin{figure}[h]
%   \includegraphics[scale= 0.48]{result/APIs-crop.pdf}
%   \caption{{\graphpy} Data Engineering Framework.}
%   \label{fig-engg}
% \end{figure}


% \td not sure what the next sentence means
% Many data science use-cases are as simple as performing graph topology analysis, such as BFS in the graph, as evident by the huge adoption of NetworkX. Even the DL requires some of those tasks. E.g. when preparing the dataset for DL, many works, such as GraphSage~\cite{graphsage17} do sampling or community analysis to downsize the graph. Further, it also performs connected component analysis and does union of a few components to get the representative dataset to avoid bias etc.
% Therefore, providing data-engineering support by {\graphpy} is not just limited to faster graph preparation from raw data, but requires good support of traditional as well as ad hoc graph analysis. 

%Graph creation step is very different than the kernels involved in DL training,  as the former involves many mundane tasks, such as file handling to parse graph data, and parallel processing to convert them to a desired format such as CSR/CSC. Further, 
%As we mentioned in the \cref{sec.science}, Plugin architecture of DL frameworks limits the way we can exchange data between Python and C++, which made passing the graph data from Workflow to Kernel a custom step for each prior work. 

The independent nature of {\graphpy-GNN} allows it to offer native Python binding capabilities. Hence, by modeling a graph as a class object, any custom graph storage can now be passed to its APIs using the same object, hence achieving a stable API. It is much better than using tensors to model graphs that needed workarounds and unstable APIs. 

Apart from customizing the graph storage format, one more variation in graph storage can be observed based on the edge properties.
%\noindent \textbf{Challenges.}
%\noindent \textbf{Gap between C/C++ and Python.}
To illustrate, edges are unweighted and undirected in GCN and GIN  but contain edge ID and are directed in the case of GAT.
%as each edge stores a trainable weight whose access is required through edge ID indirection.
%GAT requires introducing the edge ID abstraction for each edge where the edge ID points the offset in an attention score array to read (forward computation) and modify (backward computation that uses reverse graph) the attention score. 
Furthermore, graph edge requires an edge type being stored as well apart from the edge ID for the knowledge graph auto-completion GNNs~\cite{rgcn2018}. 
%Similarly, sparse tensors require the support of bipartite graphs and edge ID.
Not to mention, the ad hoc data science use-case may require the support of arbitrary multi-field properties, e.g., In LANL network dataset~\cite{turcotte17}, each edge has 9 fields and requires 32 bytes. 
%Similarly, a vertex can have properties, including its string-based identifier, type in the heterogeneous graph, timestamp, etc.

The research question here is whether we can pass graph storage with diverse edge properties to {\graphpy-GNN} for various use cases using stable APIs.
Moreover, the next opportunity to develop a productive GNN framework is to allow passing prepared graph to {\graphpy-GNN} directly and not forcing it to do the mundane tasks of file handling, data parsing, and parallel processing. 
Hence, another independent module handling graph creation is desired, and it can also be used for other graph data science use cases. 


%challenge here lies in abstracting the graph storage and passing it to {\graphpy-GNN} (or to any third party library) in a way that does not require new implementation of {\graphpy-SM} whenever graph property changes. At the same time, offer expert system researchers sufficient space to innovate in format design and kernel computation. 
% Hence, we again focus on interface design to exchange the data, apart from how to design {\graphpy-SM}.
%\noindent \textbf{Diverse Graph Storage Need.}


%Similarly, many prior graph systems, such as Galois~\cite{nguyen2013lightweight}, Ligra~\cite{shun2013ligra}, etc. cannot support graphs with arbitrary properties, even if we decide to write their Python binding.
%Hence, we can claim that \textit{graph system + Python binding is not equivalent to {\graphpy-SM}}, as the former  forces compilation for each edge property. 

%


%\subsection{Challenges and Prior Works} \label{sec.multi}


% \noindent \textbf{Opportunities.}
% We clearly see a \textit{gap} in the current graph data-science eco-system, which can allow passing graph objects stored in optimized data layout (e.g. CSR/CSC) to any third party C/C++ back-end as well as accessible in Python. Rather, graph object in prior works are captive in nature, i.e., does not allow it to be shared with third-party modules, and supports limited properties, as we explain next. The captive nature also makes the Kernel module a heavy-weight as it will have large code-base for file handling and graph preparation, or one has to rely on an ad hoc  way as in GNNAdvisor.

% It is hard to come up with a static property structure that can satisfy all the use-case of data science.




% Even if one writes python binding for such systems, we will be limited to either a single field property, or force the user to develop a plugin.
% any time we encounter a new set of properties followed by compilation Further, it now requires new python binding for each different set of properties and then compiling and deploying it. Such exercise is fine for system researchers, but we cannot expect the same from data scientists.
% or allow the final representation to be written to disk that can be used by GNNs later by loading them. 
% We focus on the former, as it allows the data scientist to further develop ad hoc techniques such as sampling or community identification to downsize the graph~\cite{graphsage17}.
% this additional python binding task introduces an important challenge to support graphs with arbitrary properties in the Python. This is due to the 



% \td not quite sure whether it relies on NetworkX or not, because DGL can build it own dgl graph, DGL can also build the graph from existing Networkx graph Alternately, it relies on NetworkX~\cite{networkx08}. 
%As we mentioned, this limits the scalability and size that we can operate on. 


%So, there is a need to develop a high-performance graph data engineering framework that can take care of all such tasks.

%the input to be available at once as edge list format of vertex IDs.
%and do not include the ML operations, which is popular in recent years. 
%Although NeuGraph, DGL and AliGraph does provide the python APIs but it assumes that the users already had the graph representation structure. 


%NetworkX \cite{hagberg2008exploring} is a python graph data science package that can create the graph representation and performs graph topology analytic tasks. NetworkX builds the graph representation data structure based on the edge list which contains information about the source node, destination node, and the optional edge weight. After building the graph representation data structure, many future graph analytics scientific computations can be performed, such as calculating the degree of the nodes, the number of nodes in the graph, or even perform a BFS algorithm on the graph data structure.
 
%However, NetworkX can only create the graph data structure from the python edge list, which makes that the network is not flexible to other raw data formats, such as CSV, text, Jason, and binary data. This format requirement restricts the usage of NetworkX and the data scientist needs to perform some graph data engineering to convert the raw data to the format which is satisfied with NextworkX if they want to use the network. Another disadvantage of NetworkX is that it was proposed in 2008, a time that the machine learning algorithms are not popular and widely used. This situation makes that NetworkX only includes traditional topology graph analytics features but not contain any machine learning related features or computations. 
 
 

%To implement the data engineering aspect of {\graphpy}, an important challenge needed to be handled. Many new-generation of graph DL algorithms need to use the dynamic graph edge information, which is not supported by previous works. \td Examples.



\subsubsection{Edge Property Specification: Numpy Dtype}
%\noindent \textbf

{\graphpy} relies on \textit{Numpy dtype} for edge property specification in the interfaces. 
%and each additional edge property can easily be modeled by defining the dtype. 
Hence, like a NumPy array object, a graph object can also allow the passing of diverse edge properties as shown in Listing~\ref{list-dtype}.
The Numpy dtype is a data type object which looks like a C-structure in Python but keeps many other details like the size of the array elements. Each element can be a native type, such as \textit{float} for a Numpy array of single floating points, or it can be a multi-field (e.g. edge weight, edge ID, edge type, etc.), each with a fixed size data type. 
%allow data scientists to define any arbitrary edge properties in Python, while {\graphpy-SM} dynamically supports those properties without any changes or compilation.
It should be noted that the dtype mechanism has become a de-facto standard for tensor specification in Python, though DL frameworks only allow a few dtype. \textit{{\graphpy} offers the exchange of graph objects among different modules by using the same de-facto standard of dtype resulting in stable APIs.}


%The {\graphpy-GNN} then can do any additional pre-processing to generate a custom graph storage. 
%Therefore how the interfaces should be designed to allow passing such diverse graphs to {\graphpy-GNNs} so that each can keep its own custom storage with the single notion of graph object to unify the model layer definition and training without redefining everything from scratch for changes to graph storage or format? 




Numpy dtype can specify many properties, and hence C++ ideally needs a new \textit{class} definition to support their compilation. 
%Differences between Python (interpreter-based language) and C++ (compiler-based language) environments introduce an important challenge to support graphs with arbitrary properties. 
For example, we can use 
%GraphOne~\cite{kumar2017graphone}, which uses 
template meta-programming to define edge properties using a C++ \textit{struct}, and can write a Python binding for the same. However, each custom property requires a new  definition in C++, and new Python binding, followed by \textit{compiling} it for use in Python.
% However, we realize that the job of {\graphpy-SM} is just to prepare the graph and not to provide graph analysis, which may require the definition of real classes to access property fields in a C++ way. 
However, dtype is nothing but information about how an array element should be interpreted in Python, including the size and type of each element in the array. 
%Hence, it is very easy to go to a specific element to read or write to it, if back-end can store the dtype information, including the size of each field. 
% Also, it is very easy to parse the input files and perform the tokenization to support reading a good set of raw input files and preparing the graph representation from it.
Hence, {\graphpy-SM} uses void pointers, element size, and other information to support dtype, along with a convention that edge dtype should always specify the source vertex first, destination vertex next, then the edge properties. Hence, by knowing the size of the edge properties, we can easily prepare a graph in {\graphpy-SM} without defining the actual C++ structure for the same.

\subsubsection{Graph Preparation, Exchange, and Ownership.} 
Table~\ref{table-api} lists graph storage related APIs. Listing ~\ref{list-dtype} shows an example of how {\graphpy-SM} prepares graph representation from the user-defined edge structure using Python dtype, and passes the prepared graph to {\graphpy-GNN}. The {\graphpy-SM} uses multiple cores and can generate the optional edge ID. The parsing APIs \textit{$add\_edges\_from\_*$()} accept delimiters and flags to support different types of input files.
For complex input data format, we require that users directly parse using the Python IO library, and send the back-end a Numpy array of edges in batches or at once using \textit{add$\_$edges()} API. Python has very good APIs for file handling and tokenization. 



\begin{table}[t]
\caption{\small {\graphpy} Python APIs for Graph Storage Handling} % title of Table
\vspace{-6pt}
\centering \small % used for centering table
%\setlength{\tabcolsep}{1mm}
\begin{tabular}{|l| l l } % centered columns (4 columns)
    \hline %inserts a single line
     \textbf{{\graphpy-SM} Initialization APIs} \\
    \hline
%    graph \hspace{1mm} init() \\
%   \hline
 %   $vclass$  init$\_$vclass(vertex$\_$count, vclass$\_$name, flag)\\
%   \hline
    $G$ \hspace{2mm} init$\_$graph(vcount, flag, edge$\_$dtype, graph$\_$name) \\
%    \hspace{22mm} e$\_$dtype, graph$\_$name)\\
    \hline
    \textbf{Graph Preparation APIs of {\graphpy-SM} on $G$} \\
    \hline %inserts double horizontal lines
    int \hspace{1mm} add$\_$edges$\_$from$\_$file(file$\_$name, delimiter, flag)\\
    int \hspace{1mm} add$\_$edges$\_$from$\_$dir(dir$\_$name, delimiter, flag) \\
    int \hspace{1mm} add$\_$edges(np$\_$array, count) \Comment{\blue{Can be called many times}}\\
    \hline %inserts a single line
    \textbf{Some APIs of {\graphpy-SM} on $G$}\\
    \hline
    {np$\_$arr1, np$\_$arr2, np$\_$arr3, np$\_$arr4} \hspace{1mm} get$\_$csr(csr$\_$dtype) \\
    %\hline
    %{Numpy$\_$array, Numpy$\_$array} \hspace{1mm} get$\_$csc(graph, dtype) \\
    %\hline
%    np$\_$array \hspace{16mm} get$\_$coo(edge$\_$dtype)\\
    \hline
    % \hspace{6mm} \textbf{ Vertex Related APIs of $vclass$} \\
    % \hline
    % int \hspace{5mm} string$\_$to$\_$vid(vertex$\_$name) \\
    % string \hspace{1mm} vid$\_$to$\_$string(vid) \\
    % \hline
    \textbf{Some Graph APIs of {\graphpy-GNN}} \\
    \hline
    g  \hspace{12mm} wrap$\_$graph(np$\_$arr1, np$\_$arr2, np$\_$arr3, np$\_$arr4) \\
    status \hspace{6mm} save$\_$graph(g, path) \\
    g \hspace{12mm} load$\_$graph(path) \\
    vcount \hspace{5mm} get$\_$vcount() \\
    ecount \hspace{5mm} get$\_$ecount() \\
     \hline
\end{tabular}
\label{table-api} % is used to refer this table in the text
% \vspace{-12pt}
\end{table}


%In Line 5, we defined the Numpy dtype for edges that contain two properties, which are present in the dataset. In Line 6, we use the API \textit{init$\_$graph()} to create the \textit{graph} object using this dtype. Preparing graphs from raw data files is performed when the user calls  \textit{add-edges-from-file()} or \textit{add-edges-from-dir()} API (Line 7). \textit{First} step inside this API is to convert the file content to the edge list/COO format. 
% We dedicated a fixed size of the buffer to gather such edges. \textit{Second} step is to convert the gathered edges to CSR format in the background using multiple cores. To support different types of files, we allow the specification of \textit{delimiter} in such APIs.

%The conversion of the edges to CSR/CSC still happens in {\graphpy-SM} using many cores.
%The edge structure format can be replaced by other Numpy dtype based on the dataset. For example, the ‘float’ data can be replaced by another ‘int’, or it can contain more properties of any fixed size fields. 
% At Line 8, we add the edges from the files present in the input directory, which includes the raw data in the text format using space as a delimiter. The comma can be used as a delimiter for CSV files.

% To overlap these two processes, we trigger the conversion to CSR even before it is full. In that sense, these two processes are continuous.   

% Raw graph data can be in any format, including plain text files or CSV, or separated by any other delimiter. To handle these cases, the APIs accept the delimiter to handle the text or CSV files. 
%At this moment we only support text, CSV, and JSON files, with support for XML files underway. Also, the parsing can be done in Python and stored temporarily using a Numpy array, and {\graphpy-SM} provides \textit{add-np-edges()}. This API can be called many times, each time providing new edges, thereby simplifying the parsing job and not occupying huge memory.




%Python code highlighting
\begin{lstlisting}[language=Python, caption= {\small Illustration of graph creation in Python using {\graphpy-SM} and passing it to a {\graphpy-GNN}. Edges have one property.}, label={list-dtype}]
import Numpy as np
import graphpy_sm as gp
import graphpy_kernel as gpk
def prep_graph():
 edge_dt=np.dtype([('src', np.int32), ('dst', np.int32), ('eid', np.int32)]
 csr_dt=np.dtype([('dst', np.int32), ('eid', np.int32)]) #dtype for csr
 G = gp.init_graph(|V|,edge_dt,"reddit", gp.eDir)
 G.add_edges_from_dir('./InputDir/', ' ', gp.eEid)
 g = gpk.wrap_graph(G.get_csr(csr_dt))
\end{lstlisting}

%\vspace{-6pt}

% V = init_vclass(vcount, "vclass1", 0)
%csr_offset, csr_neighbor, csc_offset, csc_neighbor 
%kernel_graph = gpk.wrap_graph(csr_offset, csr_neighbor, csc_offset, csc_neighbor);


{\graphpy-SM} exports the graph in CSR/CSC in the form of four zero-copy NumPy arrays using \textit{get$\_$csr()} API (At Line 9). The first Numpy array contains the \textit{offset} of size $|V+1|$, while the second array contains N(v) of the vertices along with the embedded edge properties as specified using dtype. The rest of the two arrays are for CSC format. In the case of an undirected graph, both groups of NumPy arrays share the same underlying memory. The four arrays are sufficient to pass any CSC/CSR variants taking care of the direction, edge IDs, or any multi-field property, etc. 

These arrays can be passed to the $wrap\_graph$() API of the GraphPy-GNN (Line 9) to initialize its internal graph wrapping these arrays or may further pre-process the graph to derive a new format and return the kernel-graph object(g) which is used by other {\graphpy-GNN} APIs. 
%The {\graphpy-GNN} can simply store the underlying memory pointers as offset and neighbor arrays inside the  kernel-graph object to offer vanilla CSR/CSC; or may decide to further pre-process the graph to derive a new format, and return the corresponding kernel-graph object. 
%based on parameters being passed through $dict\_param$, a python dictionary data-type, 
Thus, the kernel-graph object is owned by {\graphpy-GNN}. The module can save it to disk ($save\_graph()$ API in Table~\ref{table-api}), or load it from there ($load\_graph()$ API in Table~\ref{table-api}) without affecting {\graphpy-SM} or its other consumers (\cref{sec.overview}). 
%To demonstrate, and to gain confidence that systems researchers can provide a custom graph storage, a graduate student implemented SNB graph format~\cite{gstore}, and demonstrated many GNN models using the same set of Kernel APIs of Table~\ref{table-kernel}. It is 2-D partitioned graph, with custom storage. 
%This is in contrast to DGL, whose monolithic {Kernel} module handles graph preparation, and offers data-access APIs on the prepared graph through the same kernel.
%which has many repercussions(\cref{sec.dgl}).
%including issues in supporting diverse graph storage.


%from COO format, to CSR/CSC format with an edge ID as its fixed edge property, and offers various data-access APIs from this  graph in Python. If a system researcher wants to customize the graph storage for better Kernel performance, it would be challenging to support its existing Python data-access APIs, which assume that the underlying graph is CSR/CSC. Also, spending effort on supporting these APIs is not useful when the aim is just the kernel optimization through better storage format but will leave the whole DGL code in a broken state due to its monolithic nature. Hence, the lightweight Kernel module in the plug-and-play eco-system of {\graphpy} provides enough space for innovations without the need to spend efforts on graph preparation or in supporting the APIs that are not applicable for deep learning purposes.



%So far, we have only discussed passing CSR/CSC NumPy arrays to $wrap\_graph$(); another variant of this API also accepts COO format, where the COO data can come from $get\_coo()$ API of {\graphpy-SM}. Also, they can instruct {\graphpy-SM} to not create graphs in the CSR/CSC format by passing appropriate value in the \textit{flag} in \textit{init$\_$graph()} API.
%However, if users are only interested in COO format for some reason, they can use \textit{get$\_$coo()} directly. However, COO data is available only if the user has chosen to persist the data, as we don't keep all the COO data in memory. 
% This argument is accept in init$\_$graph() API (not shown for brevity). 
%A {\graphpy-GNN} is free to do anything that it wants with the COO data, and {$wrap\_graph$()} must return a kernel-graph object. 


% %After we create the graph representation, future graph operations such as graph topology analysis, or GNN operations can use them and are discussed in \cref{sec.dl}. 
% {\graphpy-SM} provides direct access to the graph representation using the Numpy arrays.
% The \textit{get$\_$csr()} API returns the internal CSR representation using a pair of two arrays, as per Figure~\ref{fig-format}(d). The first Numpy array contains the \textit{offset} of size $|V+1|$, while the second array contains the neighbor information of the vertices along with the embedded edge weights.  The rest of the two arrays are for CSC format. In the case of an undirected graph, both are the same. Thus, a data scientist can directly use the Numpy arrays for any ad hoc analysis either in Python or can use any other Python package that accepts Numpy arrays. 

% so that data scientists can write ad hoc analyses themselves, or can be used by other modules if {\graphpy} does not provide those functionalities out-of-box, such as GNN operations can use the use them, and are discussed in \cref{sec.dl}. 


%We have provided graph analysis module written in C++ that accepts these Numpy arrays, and supports BFS, PageRank, WCC, SSSP etc. out-of-the-box to show that is is possible to use these arrays directly inside a specialized {\graphpy-GNN} module.
%Similarly, CSC representation can also be accessed in the Numpy arrays. 

 
% \begin{figure}
% \includegraphics[scale= 0.4]{result/dtype-crop.pdf}
% \caption{example about how to use dtype for graph creation}
% \label{fig:dtype}
% \end{figure}

% \begin{algorithm}[h]
% 	\caption{\small Illustration of graph creation in Python}
% 	{\small
% 		\label{algo-dtype}
% 		\begin{algorithmic}[1]
% 		    \State {import Numpy as np}
% 		    \State {import {\graphpy} as gp}
% 			\State {\blue{\# Create graph with correct dtype}}
% 			\State {edge$\_$dt= np.dtype([('src', np.int32), ('dst', np.int32), (‘wt', np.float)]}
% 			\State {G = gp.init$\_$graph(gp.eDdir, edge$\_$dt) \blue{ \# Directed graph}}
% 			\State {G.add$\_$edges$\_$from$\_$dir(“./input$\_$dir/”, “ ”) \blue{\# space is delimiter}}
% 			\State {{\blue{\# export the graph as Numpy array with correct dtype}}}
% 			\State {csr$\_$dt= np.dtype([('dst', np.int32), (‘wt', np.float)])}
% 			\State {np$\_$csr$\_$array= G.get$\_$csr(csr$\_$dt)}
% 		\end{algorithmic}
% 	}
% \end{algorithm} 




%As we mentioned above, some newly proposed Graph DL algorithms use edge information to perform machine learning tasks. As we mentioned above, some newly proposed Graph DL algorithms use edge information to perform machine learning tasks. Therefore, the graph representation structure needs to store the edge feature information.


%Because there is not a well-defined format for edge information. In other words, different users may prefer to use different data structures and data types to store edge information. By combing these data types and data structure, there may exist thousands of different ways of edge information storage structure users can adopt. The existing graph analytics can not store these edge information or can only store an edge in as the edge information (DGL).  E.g. [x,y] only support plain graphs that have no option to store edge ID or edge properties. GraphOne, is based on template meta-programming. By definition, it must define the vertex and edge-properties in C++ before compiling and deploying it. 
 
% This means when users want to define a vertex/edge properties by themselves, they need to find the source code, define a new vertex/edge property structure, enable Python binding on this,  and re-compile to deploy it. The above pipeline procedure is not a good experience for data scientists or machine learning engineers.
 
% Our works support the dtype, which means we do not need to touch the source code. Instead, users just need to write the user-defined vertex/edge property structure and put it in the Python dtype code and the whole library can support this arbitrary edge structure.  




% \vspace{1mm}
% \noindent \textbf{Parallel Parsing.}
% % There is one difference between the two cases. 
% API add$\_$edges$\_$from$\_$dir() can use multiple cores to do the parsing work in parallel for each file, and create binary edges out of it.
% It should be noted that parsing is a very slow task, and hence parallel parsing  as shown in Fig.~\ref{fig-parallel_pa} results in faster graph creation. Here, each thread handles one file and batches them in an edge log buffer. The internal CSR converter code picks those multiple edge log buffers and converts them to CSR format using multiple threads. 
% % Thus, parsing and conversion both work concurrently utilizing multiple threads. 





% \begin{figure}[t]
%   \includegraphics[scale= 0.5]{result/high_per.pdf}
%   \vspace{-6pt}
%   \caption{{\graphpy} Parallel Parsing to produce binary edges. The CSR conversion code works concurrently to this process and operates on all the edge log buffers.}
%   \label{fig-parallel_pa}
% %   \vspace{-6pt}
% \end{figure}

% \subsubsection{Supporting Bipartite and Multiple Graphs}
% %\noindent \textbf{Supporting Bipartite and Multiple Graphs.}
% Supporting sparse tensors as in weight pruned fully connected layer requires support for a bipartite graph, which is a graph-like relationship between two different vertex ID spaces. To support that, the API  $init\_graph$() accepts two $vclass$ objects representing the two vertex ID spaces. In the case of homogeneous graphs, we only need to create one $vclass$ object.
% The data access APIs for bipartite graph still works in the same way. The different vertex count is well reflected in the offset Numpy arrays, hence {\graphpy-GNN} module uses it to derive this information about the bipartite graph. Thus the rest of the APIs remain the same for supporting bipartite graphs. 

 

% Moreover, a sparse model may be composed of many sparse layers, thus we need to support multiple independent bipartite graphs. This is achieved easily by calling init$\_$graph() many times, passing the correct vclass objects and other arguments. Thus, each returned $graph$ object represents one graph. 



% \vspace{1mm}
% \noindent \textbf{Vertex ID Space.}
% When the vertex  identifiers are in string format, the \textit{vclass} converts them to numerical IDs.
% % which is created using \textit{create-vclass()} API. 
% We provide $string\_to\_vid$() API to be used in Python. 
% %Internally, it is managed using Intel thread building block library's hash. If user requires the conversion of vertex ID to string, $vid\_to\_string$() API can be called.
% In many cases, the graph is already in the numerical ID, and hence we do not need to do the conversion. 
% %In this case, $init\_vclass()$ can directly be informed of the same using the \textit{flag}. In this case, exact number of vertex count needs to be passed using \textit{vertex$\_$count} argument. 
% We also support arbitrary vertex properties, but for brevity we treat the vertex string name as the only property in this paper. 

% \subsubsection{Data Access and Graph Analysis}
%{\graphpy-SM} offers NumPy arrays for CSR/CSC, and can be used for data access in Python directly, if needed, for any ad hoc graph analysis in Python. 

% \noindent \textbf{Graph Analysis.}
% For high-performance graph analysis, another module has been written that provides all built-in graph analysis, such as BFS, PageRank, Connected Components, etc. out-of-the-box to show that it is possible to use these arrays by other modules. 
% %inside a specialized {\graphpy-GNN} module, 
% which can be helpful in ad hoc data science applications as in GraphSage~\cite{graphsage17}. However, we do not evaluate it as it is outside the scope of the paper.
% %The module also offers GAS Framework.



%\textbf{Automatic System Integration through DSL.}
\subsection{Automatic System Integration through DSL}
Listings~\ref{list-spmm} and \ref{list-pybind} discussed earlier represent the system integration code of {\graphpy} with a DL framework. Both the listings and related code are generated automatically from  the kernel signature using our simple domain-specific language (DSL). 
{\graphpy} just uses a file written in  DSL as the input, which is almost the same as a function signature in C++, except that it must use our array$\_$t to denote the tensor. 
%Our auto-generator code implements this DSL, and generates various files to be used in {\graphpy-GNN} as well as in {\graphpy-Workflow}. 
Listing ~\ref{dsl} shows an example of the DSL specification for one kernel.
%The generator generates the boilerplate code for the {\graphpy-Workflow} completely as shown earlier in Listing~\ref{list-spmm} for CPU version. 
The generated code is slightly different for GPU listing where tensor allocation happens in GPUs and is not shown here for brevity. The code also generates the skeleton code for autograd that is needed to make the kernel call in any layer, so that backward computation of the kernel  can be called automatically. However, DSL does not know details about backward computation logic, and hence it is the job of the researcher to fill the generated skeleton. 

%Python code highlighting
\begin{lstlisting}[language=Python, caption= {\small DSL example for gSpMMv system API. We generate the boilerplate code of Listing \ref{list-spmm} and \ref{list-pybind}, and the stub calling CUDA kernel. We also generate autograd skeleton (not shown).}, label={dsl}]
#System API specification in DSL file
status gSpMMv(graph_t& g, array_t<float>& input, array_t<float>& output, int reduceFn, int Forward); 
#Generated stub for calling actual C++/CUDA kernel 
status invoke_gSpMMv_impl(graph_t& g, array_t<float>& input, array_t<float>& output, int reduceFn, int Forward); 
\end{lstlisting}
\vspace{-6pt}


%the auto-generator generates the Listing \ref{list-spmm}.
%For {\graphpy-GNN}, the auto-generator generates a common CPU and GPU version of the APIs with the Python binding as shown in Listing~\ref{list-spmm}. 
%The difference between CPU and GPU version arise inside $\_gspmm()$ function.
Thus, a system researcher is only responsible for actual system API implementation. 
It should be noted that a new signature is needed when we may want to fuse different APIs together whose signature is then very different from the one listed in Table~\ref{table-api}, but not when customizing graph storage. Further, if any change in the signature of the API is required, the DSL helps with generating new system integration code, and thus {\graphpy} speeds up the prototyping.

%Hence, any custom kernel specification is automatically integrated into the DL framework, giving the impression that APIs are natively part of it.
% \noindent \textbf{Need of a New Baseline.} 



\subsection{Alternative Designs and Discussions} \label{sec.discuss}
%DGL implements Workflow in Python and Kernel in C++/CUDA. 
%DGL differs from the earlier method as the solution relies on the {Kernel} module to implement its own tensor library, which is made inter-operable with the DLPack tensor using \textit{full} DLPack protocol's ``consume'' step. 

\noindent %$\bullet$
\textbf{Tensor Exchange.}
DGL implements the ``consume'' protocol, as DGL and DLPack tensors are open-sourced under the same organization in GitHub, hence they know the protocol well. However, they developed an elaborate tensor library (visible in Python) for the same as per the ``consume'' requirement. 
%and converts DLPack tensor to their tensor data structure (visible in Python) following the "consume" protocol of DLPack using Python APIs. 
On the other hand, \textit{Half DLPack} protocol does not need any tensor library. Instead, {\graphpy-GNN} uses an internal data structure (e.g., $array\_t$) that is not visible in Python. Hence, anybody can design it, as it merely needs to keep the pointer, shape, and size. 
It should be noted that we studied many code bases, and hence best practices are incorporated from them, such as allocating output tensors in Python and not inside the {\graphpy-GNN} (Listing~\ref{list-spmm}).

%The proposed simple solution seems very attractive compared to options where solutions are based on workarounds and hit and trial due to missing documentation and restricted interfaces. 
%which we formalized by generating a system integration code to achieve productivity. 
%The proposed mechanism is powerful enough to solve all of the interface problems that we discussed in \cref{sec.obs} and \cref{sec.usecase}. 


%Data preparation and passing it to the kernel can be challenging when storage needs are different. 
%Designing an intelligent interface can simplify kernel prototyping efforts. Prior works have not focused on this step of data science.

% % On the other hand, {\graphpy-SM} makes graph available in CSR/CSC using zero-copy NumPy arrays using dtype for edge properties. 
% Numpy package is very standard and is part of almost every scientific Python package to specify matrix elements, and exchange the matrix data. Further, dtype has also been implemented by the tensor data structure. 
% E.g., passing image data to PyTorch's convolution layer, we use tensor data-structure and dtype.
% Hence, by designing {\graphpy-SM}, we demonstrate that graph (or sparse matrix) can also be specified and exchanged the same way as dense matrices.
% %Further, the utilities that offer Python binding, such as Pybind11 provides out-of-the-box support for Numpy arrays. Hence, our module is as standard and usable as the NumPy package is.

% In a nutshell, {\graphpy-SM} is a very lightweight and highly customized graph storage. It enables data sharing with other modules using Numpy arrays. We believe, this captures sufficient requirements for ad hoc and specific graph data science use-cases that we discuss in this paper. 

\noindent %$\bullet$
\textbf{Graph Edge Property Specification and Exchange.}
GNN systems, such as DGL follows \textit{ad hoc methods} and private methods to prepare graph.
%do not provide the capability to create graph representation from the raw data, such as the CSV, and text files. They support graph in captive form, i.e. for its internal use-cases only, and does not make them available to other modules. E.g., DGL 
It expects the user to parse the dataset and also store the reverse edges in an edge list array. It then \textit{always} creates {a directed graph with edge ID} from the doubled edge list array irrespective of whether edge ID is needed or not. 
%Further, actual data are seldom found in this format, and hence users need to perform file handling themselves.
GNNAdvisor manually parses the file in Python and relies on SciPy~\cite{2020SciPy-NMeth}, %SciPy can only provide unweighted graph support, and 
which cannot support edge ID creation. 
%and has not demonstrated attention-based GNNs. 
%NetworkX~\cite{networkx08}, a pure Python package, cannot provide high performance.
%is also similar except that it is difficult to introduce the parallel graph preparation due to its pure Python nature and hence cannot be used in the Kernel module directly. 
%Dynamic graph systems~\cite{macko2015llama,ediger2012stinger,kumar2017graphone,kumar2020graphone,dhulipala2019low} etc. can create graph efficiently using C/C++.E.g., GraphOne~\cite{kumar2017graphone} provides arbitrary multi-field edge property support using template meta-programming. But it requires that users write a plugin, including a \textit{struct} to capture the property and a few other functions, and then must \textit{compile} it. 
Most static graph systems~\cite{shun2013ligra,nguyen2013lightweight} are limited to supporting a one-field edge weight such as a floating point or none, that must be compiled separately generating two binaries but does not support edge ID natively.



%There are other ways to build {\graphpy-SM} but they have not been tried yet. E.g., 
% \noindent
% {A database table} 
% %supports edge properties through table columns and can make data exchange free of compilation. However, they are 
% is  an examples of captive solutions where we need to send the computations (e.g., queries) to the database module. If we need to get the whole graph in CSR/CSC format,
% %Similarly, one can use binary JSON structure as a way to store the properties, and thus enable data transfer easily, however, we need to convert it back to CSR/CSC first. 
% the \textit{dtype} like mechanism is still needed. Hence, just a python package of existing databases is not enough to get the graph storage to {\graphpy-GNN}. %without the support of \textit{dtype} like mechanism.

==> tex/challenge.tex <==
%Next section examines if we can achieve them together, and also discusses prior works
%{\color{red}
%The simple and extensible nature of {\graphpy}

% Integrating systems research (e.g., writing new kernels to avoid using bitmap in Python, or any other kernel optimization) to any DL framework does not have a standard approach today.
% Unifying and simplifying such integration can provide a very useful platform. 

%If one observes operating systems, POSIX specification made userspace application development very portable and modular. One hardly has to rely on OS-specific header files or follow its internal development guidelines to start developing new application, and enables reusability across POSIX compliant OS. Our work is inspired by such observations, and centers around innovations in the infrastructure and interface design.
%This and next sections explains such challenges, and the novel solutions.
%as well as the extensible use-cases in detail.
%}
% including deep learning and traditional graph analysis.

%\subsection{Challenges and Prior Works} \label{sec.challenges}

% \subsection{Challenge \#1: Tensor and Graph Exchange } \label{sec.science.challenges}

% %\noindent \textbf{and Memory Management.}
% %To provide the DL use cases, we observe that two modules are needed: \textit{\graphpy-Kernel} and \textit{\graphpy-Workflow}. 
% %Table~\ref{table-kernel} provides the {Kernel} APIs, 
% As we pointed out earlier, implementing DL kernels such as gSPMM, etc. alone is not enough as DL training requires support for computation graph, tensor management and back-propagation to update the model parameters. 
% %There exist some DL frameworks such as PyTorch providing automatic support for invocation of back-propagation. 
% %Specifically, the edge of the  computation graph denotes the kernel invocation in the forward computation, the back-propagation calls kernels to perform the gradient computation using the same computation graph but in the reverse order (Fig.~\ref{fig-forward}).
% Back-propagation needs to use the input and output tensors as states (\cref{sec.background.dl}), hence de-allocation of the tensors need to be delayed until back-propagation has used them for each epoch. 
% Moreover, the Kernel APIs also require access of graph $g$. 
% %Graph creation from raw data could be made part of the Kernel, but is actually a standalone operation that could be treated as pre-processing step. 
% It needs a forward graph or its inverse depending on whether a DL kernel is invoked in the forward or back-propagation.  


% Hence, apart from {\graphpy-Kernel} (or Simply Kernel if referring to prior works), we need \textit{{\graphpy}-Workflow} (or simply Workflow), to provide many of these support by itself (computation graph, tensor management, correct graph passing, etc.) or using some well laid out protocols to achieve them together with Kernel module. At the end, we expect to integrate kernel APIs to DL frameworks so that DL training process can happen. 
% Next, we examine how such integration tasks can be achieved currently using DL frameworks.
% %and whether they are simple and obvious or requires huge efforts by researchers and learners. 




% \noindent
% $\bullet$ \textit{Approach \#a.}  Both the Workflow and Kernel modules can be implemented using C++ plugin directly by including the necessary LibTorch header files, and following the specific LibTorch development guidelines. We did not find any existing work that uses this approach, so we implemented this approach ourselves. 

% \noindent
% $\bullet$ \textit{Approach \#b.} In this approach, the Kernel is implemented using C++ by including the necessary LibTorch header files, while using Python to implement the Workflow using LibTorch guidelines. Pytorch-Geometric~\cite{pytorchg2019}, GNNAdvisor~\cite{GNNAdvisor} follow this approach. 

%\subsubsection{Tensor and Graph Exchange: Challenges and Prior Works.}
%\subsubsection{Use DL Framework's Tensor}
%{\color{red}
%DL training requires computation graphs and tensor support, hence GNN systems rely on existing DL frameworks for the same. 



% \subsection{Challenge \#2: Missing Baseline}

% \noindent \textbf{Out-of-Memory Condition and Framework Overhead.}
% Our measurements show that many current GNN systems show out-of-memory condition frequently on even slightly larger dataset in  single GPU setup. 
% Reddit graph, which has less than 230 million edges, can not be trained on A100 GPU which has 40 GB memory by PyG, GNNadvisor on any of their supported models. DGL cannot run slightly complex GAT model, while it still consumes way more than 16 GB memory for GCN, and simple GAT model. Hence, it is unsuitable on low- and mid- grade GPUs that has small memory, such as Nvidia GTX 1080 Ti.
% Hence, many prior GNN systems have only demonstrated smaller dataset for performance, which then are affected due to framework overheads that we discuss shortly. 
% Moreover, many works that do evaluate larger dataset have only focused on kernel benchmarking, but has many issues (\cref{sec.science.challenges}). 

% %DGL~\cite{dgl2019} is another GNN system, however it suffers from many framework level issues, that does not let it function as a baseline system.
% We investigate if end-to-end training performance comparison on smaller dataset can really rank systems based on their kernel performance.
% Table~\ref{table-motivation-overhead} shows overhead for GCN on two smaller dataset of Cora and Pubmed in an A100 Nvidia GPU that includes the time taken by rest of the  Python and C++ code but not kernel time; as well as total training time. The methodology and dataset are described in \cref{sec.exp-gnn.time}. It is very clear from this table that the total training time for Pubmed actually does not depend on the kernel time, as total training time is almost equal to the overhead time. Hence, any optimization of the gSpMM kernel will not show up if using DGL to prototype kernels. However, many systems who use PyTorch's plugin approach to prototype GNN on this dataset shows huge performance improvement compared to DGL. Hence, how can we be sure if the performance improvement is purely due to better kernel implementation and not due to difference in the overhead, when we are not able to evaluate larger dataset. 
% %Also, if the performance improvement is due to overhead differences, how can we propose a better framework that does not cause such huge overhead, and allow us to run larger dataset so that it can be used as better baseline. 

% \begin{table}[t]
% \small
% \vspace{-6pt}
% \caption{Framework Overhead of DGL (in Seconds)} % title of Table
% \vspace{-6pt}
% \centering % used for centering table
% \begin{tabular}{|l| c cc|c|} 
%     \hline\hline 
%     Graph & Startup & Runtime & Total & Training\\ [0.5ex] % inserts table
%     Dataset & Cost  & Cost  & Overhead  & Time \\
%     %heading
%     \hline % inserts single horizontal line
%     Cora & 0.828 &  0.512 & 1.340 & 1.347  \\ 
%     PubMed & 0.786 & 0.684 & 1.470 & 1.480  \\
%     % & 76.47 &  76.52 & & \\
%     \hline %inserts single line
% \end{tabular}
% \vspace{-6pt}
% \label{table-motivation-overhead} % is used to refer this table in the text
% \end{table}

% %And because of these two costs, DGL performs poorly (more than 2$\times$)  compared to reference implementation (not optimized) of {\graphpy} for GNNs on several dataset, despite DGL kernels performing better than {\graphpy} kernels. Since DGL has a large overhead, it is not surprising that many prior GNN systems~\cite{GNNAdvisor,huang2021understanding}, which do \textit{not} use DGL for their integration, have a huge speedup. \td

% %To this end, {\graphpy} through its lightweight design minimizes both the overheads, and hence is well-suited not only for future systems research prototypes, but also as a baseline to understand the true impact of prior system optimizations.

% Hence, none of the prior systems present a good baseline for end-to-end training on which future system research can do performance evaluation that is needed for progress of system research. 

% %Our limited survey of other works that modified DGL to demonstrate better performance, also relied on CSR/CSC format. We suspect that such researchers may have found that modifying whole DGL Kernel a tedious process when format changes are involved. \td.

% %Hence, the lightweight Kernel module in the plug-and-play eco-system of {\graphpy} provides enough space for innovations without the need to spend efforts on graph preparation or in supporting the APIs that are not applicable for deep learning purpose.

% %Writing interfaces for a new kernel in DGL is still a complex problem due to involvement of tensor library and memory management. 
 

% % %On the other hand, DGL/PyG takes only COO arrays as input in their initialization API. 
% % %Further, the generation of critical boiler-plate code, makes integration effortless. 
% % \noindent \textbf{Sparse Data.}
% % We also implemented {\graphpy-Kernel} for GNN as proof of concept and reference. We mostly focused on CSR/CSC format for reference and comparison, 
% % It includes an unweighted gSpMM kernel to support GCN and GIN; a weighted gSpMM kernel, and two versions of gSDDMM kernel for GAT as mentioned in Table~\ref{table-kernel}. 
% % %Both of these are sufficient for a graph-specific softmax layer, and for edge-level attention score from vertex-level features.
% % We use pull-style computation that avoids usage of atomic instructions: so CSC for forward and CSR for backward computation or wherever inverse graph is needed.
% % We used OpenMP for vertex-level parallelism in CPU. % and use vertex-centric computation.
% % To support GPUs, we implemented kernels in CUDA. The same {\graphpy-Workflow} works except that the model requires to be converted to GPU, which is achieved using $model.to(cuda)$, where cuda is the device context. Similarly, the adapter of {\graphpy-Workflow} allocates tensors directly on GPU.

% % We also implemented another format borrowed from prior graph analytics work~\cite{gstore}, which is very different from CSR/CSC format to demonstrate that an entirely different format can be implemented with same ease, using the same set of Kernel APIs. We used the same {\graphpy-Workflow} code, including the GNN model, graph convolution layers. We do not use that format for comparison.
% % % \noindent 
% % % $\bullet$ \textbf{GPU Support.} 
% % % The specialized kernel is also implemented in GPUs by using the same boiler-plate code. The same {$wrap\_graph$()} API instead of simply wrapping the CPU version of Numpy arrays, it copies them to GPU memory, and then wraps them up in $g$ object. Thus, the rest of the kernel APIs (Table~\ref{table-kernel}) get the GPU version of the graph, and Python binding code of the kernel invokes the GPU kernels. Thus, the same piece of {\graphpy-Workflow} works except that the model requires to be converted to GPU, which is achieved easily using $model.to(cuda)$, where cuda is the device context. Similarly, the {\graphpy-Workflow} allocates tensors directly on cuda or device memory.


% % \vspace{1mm}
% % \noindent \textbf{Motivation and Challenges.}
% % \textbf{Challenge \#1. Graph Data Engineering.}
% % All graph data science works assume that the graph representation already exists. In other words, if the data scientist wants to use the prior system techniques of graph analytics works, they need to first perform the graph data engineering task to create a graph representation in the right format from the raw data. The raw data could be in any readable format, starting from a plain graph format to a CSV, JSON, XML or binary files.

% % Also, the graph representation varies slightly from case to case. E.g. in GCN case, the graph is assumed to be a simple graph having no edge properties. But in case of knowledge graph, each edge has a edge or relationship type, that is stored as part of the graph. Further, attention based GNNs such as GAT need to keep attention score for each edge of the graph. 
% % However, preparing graph representation does not stop here. Recent works~\cite{hamilton2018embedding} have used various other data engineering tasks including sampling, community identification, union of sub-graphs etc to prepare the final graph representation.\td {write down a few lines here}
% % \td. What are other variations?

% % Hence, capability to create graph from raw data, as well as post-processing steps to create the final graphs is desired to ease the job of deep learning on graphs, and requires supporting graphs with arbitrary vertex and edge properties.
% % This procedure is not only difficult and time-consuming, but also ad hoc{\td} a few more keywords. 

% % Further, this capability must be a part of python programming environment, as it has become a de-facto programming environment for data science. It has an interpreter based execution, and no good support for multi-threading, the actual computation happens using back-end, which is written in high-performance languages like C/C++ and CUDA. 
% % Unfortunately, the like the current GNN systems, the prior graph analytics works also lack support for data engineering operations. GNNs expect the data scientists to do all the data engineering tasks to create this limited representation as they support just one type of graph with no edge properties, E.g., NeuGraph does not support attention based GNNs yet.

% % On the other hand, there are a few python based graph data engineering frameworks, such as NetworkX, which is being used by DGL. However, it is purely python based package, and  stores the graph data in  python using dictionary of dictionary format. 
% % The graph representation of NetworkX needs more memory space, have scalability problem. If the graph structure is large, it cannot fit into the memory, and suffers due to absence of good multi-threading in the python programming environment.
% % Hence, one can conclude that GNN systems are limited by the scalability of pure python packages. 
% % Therefore, the data engineering tasks preceding the deep learning kernels must be performed in a high-performance back-end to provide a uniform experience, high performance and scalability to larger dataset.


% % \textbf{Challenge \#2. Implementing Deep Learning Workflow.}
% % The second challenge is on how to use the existing code base of prior works that have proposed novel systems design to test the efficacy of their techniques in the field of deep learning. Since, these works mostly offer GAS or sparse linear algebra based programming framework, they are well-suited to support the kernels required by GNNs. Hence, the question here is what it takes to integrate such code base to do the GNN operations, specifically how to minimize the changes that are required to make this code base ready for deep learning, such as gradient computation without requiring huge coding.

% % \begin{figure}
% %   \includegraphics[scale= 0.26]{result/framework.pdf}
% %   \caption{The framework of {\graphpy}}
% %   \label{fig:boat1}
% % \end{figure}    




==> tex/exp2.tex <==
\noindent \textbf{Traditional Graph Analytics}
In this test, we run two traditional graph analyses, namely breadth-first-search (BFS) and connected components (CC). We did not find a Python system with a high-performance back-end that can support arbitrary graph properties, so we choose NetworkX to show the advantage of choosing a high-performance back-end to perform the analysis. All the analyses are called from the Python environment.

Table~\ref{table-nx} shows the comparison. It is obvious that with a C++ backend, {\graphpy} will gain huge performance over pure Python-based NetworkX. 
%However, the aim of this experiment is slightly different: {\graphpy} is not just Python binding for an existing C++ back-end, but involves huge effort to
By enabling arbitrary edge properties using Numpy Dtype, {\graphpy} is as usable as the NetworkX or even more. So for users, NetworkX and {\graphpy} are the same but with better performance and scalability, which is purely achieved due to innovation in interface design.


\begin{table}[h]
\small
\caption{\small BFS and CC run-time of NetworkX and {\graphpy}. The run-time is in \textit{Milliseconds}. Speedup is shown inside the bracket.} % title of Table
\vspace{-6pt}
\centering % used for centering table
\setlength{\tabcolsep}{1mm}
\begin{tabular}{|l| r  r | r r| } % centered columns (4 columns)
\hline\hline %inserts double horizontal lines
Dataset & \multicolumn{2}{|c|}{NetworkX} &  \multicolumn{2}{c|} {\graphpy}  \\ 
\cline{2-5}
 & BFS  & CC &  BFS  & CC \\
\hline % inserts single horizontal line
Cora & 13.05  &  0.86 & 0.29(45.00$\times$)  &  0.42(2.05$\times$)\\ 
PubMed &  449.49  & 42.72 & 10.71(41.97$\times$) &  22.64(1.89$\times$) \\
Amazon & 4152.54 &  594.10 & 118.80(34.95$\times$) &  160.30(3.71$\times$) \\
% Patent Citation &  OOM & OOM & 1102.86(-)  & 3723.57(-) \\
% [1ex] % [1ex] adds vertical space
\hline %inserts single line
\end{tabular}
\label{table-nx} % is used to refer this table in the text
\end{table}


%\vspace{2pt}
\noindent \textbf{Multi-Field Properties.}
%{\graphpy} provides users an option to store the edge properties when creating the graph. This option is important because some graph DL algorithms, such as GCN, do not need any edge property. Therefore, there is no need to create a graph with edge property in this case. DGL always creates edge IDs, while NetworkX has an option for specifying the optional weight. However, 
NetworkX allows specification on only a single weight field, while {\graphpy} allows specification of arbitrary multi-field custom weights using NumPy Dtype. 
% Though we limit our evaluation to simple graphs with option edge IDs. \td.
We use LANL dataset that has 9 properties for each edges to demonstrate this capability. Also, it does not have a numerical identifier in its raw data file. Thus, the vertex ID must be created from the string identifier. Hence, only {\graphpy} allows graph creation from this dataset. It achieves 2.247 Million Edges/Second of ingestion rate.

% \begin{table}[ht]
% \caption{Ingestion Rate (in \textit{Million Edges/Second}) for Kron-20 dataset. {\graphpy} allows parallel parsing of the dataset files, and leads to better performance.} % title of Table
% \centering % used for centering table
% \begin{tabular}{l r r } % centered columns (4 columns)
% \hline\hline %inserts double horizontal lines
% System & Ingestion Rate & Speedup \\ [0.7ex] % inserts table heading
% \hline % inserts single horizontal line
% NetworkX               &    0.331 & 1.00$\times$ \\
% DGL                    &   0.869 &  2.62$\times$  \\
% {\graphpy} (1 thread ) &   3.767 & 11.37$\times$  \\
% {\graphpy} (2 threads) &   7.497 & 22.64 $\times$ \\
% {\graphpy} (4 threads) &   9.847 & 29.73$\times$  \\
% % {\graphpy} (8 threads) &   11.227 & 33.90 $\times$ \\
% [1ex] % [1ex] adds vertical space
% \hline %inserts single line
% \end{tabular}
% \label{table-parallel} % is used to refer this table in the text
% \end{table}


% \begin{table}[ht]
% \caption{\td result for parallel parsing Ingestion Rate (in \textit{just original time}) for  Patent-Citation. {\graphpy} allows parallel parsing of the dataset files, and leads to better performance.} % title of Table
% \centering % used for centering table
% \begin{tabular}{l r r } % centered columns (4 columns)
% \hline\hline %inserts double horizontal lines
% System & Ingestion Rate & Speedup \\ [0.7ex] % inserts table heading
% \hline % inserts single horizontal line
% NetworkX     &    0.318    & 1.00$\times$ \\
% DGL                    &  0.878   &  2.76 $\times$  \\
% {\graphpy} (1 thread ) &   3.777  & 11.89 $\times$  \\
% {\graphpy} (2 threads) &  6.684  &   21.04$\times$ \\
% {\graphpy} (4 threads) & 8.067   &  25.40$\times$  \\
% % {\graphpy} (8 threads) &   11.227 & 33.90 $\times$ \\
% [1ex] % [1ex] adds vertical space
% \hline %inserts single line
% \end{tabular}
% \label{table-parallel-patent} % is used to refer this table in the text
% \end{table}


% \vspace{1mm}
% \noindent \textbf{Parallel Parsing.}
% In the overall graph preparation pipeline, file parsing is the bottleneck as it is slow due to involvement of tokenization and other string operations. Hence, {\graphpy} provides parallel parsing when possible.  Users can choose the number of threads dedicated to this work.
% To test the system performance of this option, we use different number of threads and calculate the ingestion rate as the metric. 

% \begin{figure}[h]
%   \includegraphics[scale= 0.62]{exp/parallel-ingestion-crop.pdf}
%   \vspace{-6pt}
%   \caption{Ingestion Rate (in \textit{Million Edges/Second}) for Patent Citation dataset. {\graphpy} allows parallel parsing of the dataset files, and leads to better performance.}
%   \label{exp-parallel}
% %   \vspace{-12pt}
% \end{figure}

% We use Patent-Citation dataset that resides in multiple files. 
% We selected small size, because NetworkX runs out-of-memory for slightly bigger than this graph.
% Fig. \ref{exp-parallel} shows the average ingestion rate result, with different parsing thread count.  We find that as the number of threads increases, the system performance improves. The average graph creation time for {\graphpy} with 4 threads is over 25$\times$ and 9$\times$ faster than NetworkX and DGL respectively.
% % with 8 threads is 33$\times$ faster than NetworkX and 13$\times$ faster than DGL.
% The results around 4 threads are slightly sub-linear. This is because the system has only 4 physical cores. Hence, the graph creation starts saturating the resources as 4 threads are also dedicated to graph preparation from the buffered edges.


\subsection{Ingestion Rate of {\graphpy-SM}}
We use \textit{ingestion rate} as the metric to measure how many edges (from raw data files) can be processed per second to create the graph in CSR/CSC format. This ingestion rate is end-to-end, implying that it also includes the time of file parsing, which can only be done using a single thread if there is only one file. 
We evaluate the {\graphpy} against two existing graph systems DGL, and NetworkX, as both of them have Python interfaces.
Fig.~\ref{exp-ingestion} shows the ingestion rate in million edges/second for four datasets in a single socket 4-core Intel CPU up to 3.60GHz, and DRAM of 16GB loaded with Ubuntu 18.04.
% i7-4790 
We find that  {\graphpy} with edge ID is 6$\times$ and 11$\times$ faster than DGL and NetweorkX respectively. {\graphpy} is faster as it does the text file parsing in C++ which is faster than parsing in Python in DGL and NetworkX. 
%Second, the overlap of the parsing with CSR/CSC creation leads to a faster ingestion rate. 
If we create the graph without storing edge IDs, as in the GCN case, the ingestion rate can be improved by about 3\% but saves memory equivalent to $|E|$. It achieves over 4 million edges/second of ingestion rate on the Amazon dataset. 

%We did not create edge IDs in NetworkX as it is not a GNN framework.

 

\begin{figure}[h]
 \vspace{-6pt}
  \includegraphics[scale= 0.60]{exp/ingestion-crop.pdf}
%   \vspace{-6pt}
  \caption{\small Ingestion Rate: {\graphpy+} refers to creating the graph with edge IDs, while {\graphpy} refers without edge IDs. DGL always creates edge IDs. For NetworkX, we did not create edge IDs. OOM refers to out-of-memory condition.}
  \label{exp-ingestion}
  \vspace{-6pt}
\end{figure}


% \begin{table}[h]
% \caption{Ingestion Rate (in \textit{Million Edges/Second}): {\graphpy+} refers to creating the graph with edge IDs, while {\graphpy} refers to creating the graph without edge IDs. DGL always creates edge IDs. For NetworkX, we did not create edge IDs. OOM refers to out of memory condition that does not allow NetworkX to complete the ingestion on Patent Citation.} % title of Table
% \centering % used for centering table
% \setlength{\tabcolsep}{1.3mm}
% \begin{tabular}{l r r r r r} % centered columns (4 columns)
%     \hline
%     \hline %inserts double horizontal lines
%     System & Cora & PubMed & Amazon &    Patent-Citation & LANL \\ %[0.6ex] % inserts table
%     %  & & & & Citation \\
%     %heading
%     \hline % inserts single horizontal line
%     NetworkX & 0.201 & 0.364 & 0.400 & OOM & -\\
%     DGL & 0.611 & 0.833 & 0.787 & 0.752 & -\\
%     {\graphpy+} & 3.693 & 4.064 & 4.057 & 3.876 & NA\\
%     {\graphpy} & 3.850 & 4.167 & 4.252 & 4.081 & 2.247\\
    
%     % {\graphpy} (4THD) &   &   &   & 273.11 \\
    
%     % {\graphpy} (8THD) &   &   &    & 403.79 \\
% \hline %inserts single line
% \end{tabular}
% \label{table-ingestion} % is used to refer this table in the text
% \end{table}

\subsection{Sparse Tensor}
We choose the LeNet-300-100%~\cite{lecun1998gradient}, 
a fully connected neural network with 300 and 100 as the hidden layers. After weight pruning~\cite{han2016iclr}, all three fully connected layers become sparse with sparsity ratios of 4.46\%, 4.45\%, and 7.78\% respectively, i.e., keeping less than 10 connections for every 100 connections in the fully connected layer. We use the MNIST dataset which includes 60000 training and 10000 testing handwritten digits examples.  Each image in the dataset has 784 features, while the last fully connected layer produces predictions corresponding to 10 digits (0--9). 
%which are sent to the softmax layer. 
We set the retraining epochs as 100 and the batch sizes as 50. In other words, in each training epoch, the model will iterate 1200 times.
% and apply tensor-based operations for state-of-art model and the sparse layers computation for {\graphpy}.
{\graphpy} finishes the retraining in 16 minutes and 17 seconds, compared to 20 minutes and 1 second for the model that uses the bitmask matrix to achieve sparsity~\cite{{han2015learning,han2016iclr}}, achieving 17.5\% speedup, and huge memory saving.

%The reason for this speedup is the reduced computation which {\graphpy} could achieve due to its system-level support for sparsity. 
%On the other hand, prior works have used bit-mask matrix at the Python level for achieving sparsity where the underlying kernel still uses dense matrix for sparse layer computation. Again, 
The improvement is only 17.5\% as LeNet-300-100 is not a large neural network, as the bipartite graph has vertex counts in the range of 784 and 10. Hence, the sparse weight matrices are not as large as the graph data set we had above for the GNN case. However, it shows the possibility of the {\graphpy} framework for diverse research use cases.
%This affects the vertex-level parallelism for SpMM. With better technique, we expect better performance, as our implementation is only for reference. 

%Secondly, it is not just the performance improvement, but the huge memory saving that allows the compressed model to fully fit in the resource constrained devices. Hence, model inference can now be done fully in such devices.
% Also, the sparse layers computation procedures contain mostly random reads instead of sequential reads. 



==> tex/extend.tex <==

\begin{table}[t]
\footnotesize
\caption{\small {\graphpy-GNN} System APIs. Goal: a) Passing graph object as is, and remaining independent of DL framework; b) Their implementation must invoke the CUDA or device kernels internally.} 
\vspace{-6pt}
\centering % used for centering table
\setlength{\tabcolsep}{1mm}
\begin{tabular}{|l|} % centered columns (4 columns)
    \hline %inserts a single line
    % \textbf{Graph Handling APIs (\cref{sec.engg})} \\
    % \hline
    % g  \hspace{8mm} wrap$\_$graph(np$\_$array, np$\_$array, np$\_$array, np$\_$array, dict$\_$param) \\
    % status \hspace{2mm} save$\_$graph(g, path) \\
    % g \hspace{8mm} load$\_$graph(path) \\
    % % \hline
    % % \hspace{6mm} \textbf{APIs on $g$} \\
    % % \hline
    % % int \hspace{14mm} get-vcount1() \\
    % % int \hspace{14mm} get-vcount2() \\
    % % np$\_$array \hspace{6mm} get-degree1() \\
    % % np$\_$array \hspace{6mm} get-degree2() \\
    % \hline
    \textbf{{\graphpy-GNN} APIs for System Integrator (Not for Data Scientist)} \\
    \hline
    status \hspace{2mm} gSpMMv(g, \textit{in-tensor}, \textit{out-tensor}, eFn, Flag)\\
    % \hline
    status \hspace{2mm} gSpMMveid(g, \textit{in-tensor}, \textit{in-tensor}, \textit{out-tensor}, eFn, Flag)\\
    status \hspace{2mm} gSpMMeid(g, \textit{in-tensor}, \textit{out-tensor}, eFn, Flag)\\
    % \hline
    status \hspace{2mm} gSDDMMvv(g, \textit{in-tensor}, \textit{out-tensor}, eFn, Flag)\\
    status \hspace{2mm} gSDDMMve(g, \textit{in-tensor}, \textit{in-tensor}, \textit{out-tensor}, eFn, Flag)\\
    \hline
    % status \hspace{2mm} spmm(g, \textit{in-tensor}, \textit{in-tensor}, \textit{out-tensor}, Flag)\\
    % % \hline
    % status \hspace{2mm} sddmm(g, \textit{in-tensor}, \textit{in-tensor}, \textit{\textit{out-tensor}}, Flag)\\
    % \hline
\end{tabular}
\label{table-kernel} % is used to refer this table in the text
%  \vspace{-2pt}
\end{table}



\subsection{{\graphpy}: GNN Specific Design} \label{sec.baseline}

We design {\graphpy} Based on the above analysis. It has two components, {\graphpy-Kernel} which is responsible for CUDA kernel API definition and implementation, and {\graphpy-GNN} which interfaces Pytorch using Python binding, and internally calls {\graphpy-Kernel} CUDA APIs. 

\subsubsection{Storage Format} 
We take advantage of dataset symmetry and store just the CSR topology that serves as both the CSR and CSC. For the COO, it is stored in CSR-way, and hence it shares the format with the CSR storage. 

For the transpose need of an edge-level tensor, we decided to use the edge ID rather than developing transposed gSpMM versions. The reason is that the algorithm for transposed gSpMM is not well developed by the community. Our naive version relied on a naive scatter method where each row scattered message atomically to every non-zero column using an atomic instruction. Secondly, it requires the support of various reduction operations, for which atomic operations are not supported out of the box. We believe transposed gSpMM requires its own independent discussion, and leave it as a future work.   

Hence, we decided to rely on the edge ID abstraction but store the edge ID for CSC only. CSR is assumed to be containing an implicit edge ID to CSR. Since the COO shares the CSR storage, both of them have an implicit edge ID. Thus, only one edge ID array is stored.
In total the format costs CSR $(|V| + |E|)$ + COO ($|E|$) + Edge ID array ($|E|$). Thus reducing the memory consumption by almost 3$\times$ due to storage design alone compared to DGL without introducing any trade-off.
%where the last $|E|$ is for COO as half of its storage is shared with CSR.

\subsubsection{APIs}
We now present kernels that are directly suited for Class A and B GNN use cases based on the insight gathered from the design analysis. The APIs (Table~\ref{table-kernel}) are directly invoked by {\graphpy-GNN} system to avoid the kernel mismatch without any need for any additional intermediate kernel.
We define usual gSpMMve, and gSDDMM. However, we introduce two different kernels compared to prior works to take care of GNN-specific requirements.

%without incurring any requirement mismatch overhead. %The proposed CUDA kernels have almost similar signatures as the system APIs of Table~\ref{table-api}. {\graphpy} internally defines and designs GNN-specific kernels, 
%Hence, the proposed internal CUDA kernel signature follows a similar signature as the system API to directly map the requirements. This was needed to show that avoiding the generalization cost of prior kernel design can save memory and gain performance.


\noindent \textbf{gpk$\_$gSpMMveid.}
This {\graphpy} kernel is a weighted gSpMM that accepts a vertex-level and an edge-level tensor. However, it accesses the edge-level tensor using edge ID which is part of the graph storage. We also support a vector feature for each edge, which is used by the multi-head GAT model.

%\textit{gSpMMveid} invokes just one kernel that directly expects a graph with edge ID to avoid the need for a separate eShuffle CUDA kernel and never generates additional intermediate results. It is used to perform transposed gSpMMve.
Memory saving and performance gains are achieved by {\graphpy} just because of the new API design compared to all prior systems. (1) It accesses the edge-level tensors directly using the edge ID, hence eShuffle kernel is completely avoided, and so is the need to materialize an additional tensor of size O($|E|$), thus saving memory. (2) This kernel is faster than even a workload-balanced gSpMMve plus a separate eShuffle kernel. (3) The multi-head gSpMMveid cannot be simulated by the CuSparse-compatible gSpMMve kernel.


% To recap, our investigation in \cref{sec.obs} and \cref{sec.usecase} pointed out that not just DGL (or CuSparse), but many others~\cite{gespmmsc2020,featgraphsc20,huang2021understanding} have continued developing CuSparse compliant-gSpMMve for GNN use-cases.  
%for at least class B GNN, namely gSpMMveid, while many still provide gSpMMve for class A GNN. 
%Also, APIs for CuSparse are not well-suited GNN use cases as discussed in \cref{sec.dgl}, which other works continue to optimize, such as gSpMMve, and not gSpMMveid which they should. 
%We define new signatures of \textit{gSpMMv} and \textit{gSpMMveid}. 

 
% Similarly, \textit{gSpMMv} system API invokes a kernel definition that does not need any dummy edge-level tensors and supports normalization by degree as an option. The forward gSpMMv in GCN uses this option, but backward gSpMMv does not rely on this kernel fusion. However, it invokes normalization separately before calling the gSpMMv cuda kernel. 

\noindent \textbf{gpk$\_$gSpMMv.}
This kernel is unweighted gSpMM. Hence, it only accepts a vertex-level tensor as input along with reduction operation type, such as \textit{sum, min, max} but not any edge-level tensor. The API also accepts an optional boolean flag to indicate normalization by degree flag. When the flag is true, it only normalizes the result of gSpMM as part of the same kernel. Hence, in the backward computation, the flag should be set as false, and a separate normalization kernel should be called. This API is used by class B GNNs. 

This kernel definition, though very intuitive 
%differs from prior works. CuSparse, FeatGraph, Huang et al offer gSpMMve. GNNAdvisor does not make normalization optional and ends up with the wrong fusion during backward. GE-SpMM has mostly focused on gSpMMve, and silently implements gSpMMv without the normalization option. 
provides substantial memory saving to {\graphpy} on two accounts. (1) Compared to CuSparse compliant gSpMMve, {\graphpy-GNN} never need to allocate dummy edge-level tensor saving O($|E|$) memory. This also results in a substantial performance gain. 
(2) Even in the case of a separate normalization, {\graphpy} uses the same tensor as input and output both by using in-place normalization inside {\graphpy-GNN}. 
%On the other hand, DGL performs normalization at the Python level using  PyTorch's CUDA API that can only perform out-of-place normalization, Thus increasing the memory consumption by O($|V|$*feature-length). Hence, DGL-integrated systems, such as GE-SpMM and FeatGraph likely to consume additional memory as well.


% We did not define gpk$\_$gSDDMMveid, as we generated COO in a way that can rely on an implicit edge ID equivalent of the position of each edge in the COO. %to use gpk$\_$gSDDMMve. 
% %COO offers edge-parallel implementation, which achieves fully workload-balanced implementation. 

% \noindent \textbf{gpk$\_$gSDDMMvv.}
% It remains the same as discussed in \cref{sec.obs}.



% \noindent
% \textbf{1. Framework Overhead Reduction.}
% %\red{DGL has significant overhead for small datasets. To reduce the Framework overhead, }
% Prior works reduced framework overhead by moving the model layer to C++, which did not follow the guidelines property, as it could be complex to write those correctly. We left the model layer code in Python. However, we reduced the framework overhead by removing the system initialization steps of DGL which allocates many intermediate memory objects to bridge the requirement mismatch which takes a huge time (\cref{sec.exp-gnn}). 
% %dummy edge-level tensors, 
% Further, {\graphpy} uses code generation to define and implement interfaces. In doing so, it generates separate interfaces for each gSpMM and gSDDMM variant, thereby simplistic nature of {\graphpy} interfaces can invoke the right kernel variant quickly as we avoid having a message passing infrastructure and other overheads of DGL to locate the exact kernel variant to invoke. 
% %Further, for fused kernel design, {\graphpy} generates a new kernel from the DSL specification of the kernel. 
% Therefore, {\graphpy} optimized the training for small datasets.


% As we mention in \cref{sec.usecase}, DGL relies on CuSparse which creates requirement mismatch, hence DGL invokes additional kernels while materializing many intermediate results. We explain  how we remove these overheads.
% %class A type of GNN models use the unweighted sum for aggregation and use vertex-level tensor only. 
% %Class B type of GNN models touches both vertex level and edge level tensor. 
% %DGL uses gSpMMve kernel to handle  this. \red{ which involves extra unneeded computation. To optimize this situation, } {\graphpy} separates the gSpMM kernel into two specific designed kernels: gSpMMv designed for class A GNN which does not fetch the edge level tensor;  gSpMMve, designed for class B operates on vertex-level and edge-level tensors. \red{Since gSpMMv kernel does not fetch the unneeded edge-level weight anymore, the class A type of GNN models can achieve both better memory-saving and better time-saving. }
% (a) DGL uses a dummy edge-level tensor with each value as 1.0 to implement gSpMMv using CuSparse API, we directly implement gSpMMv without this dummy edge-level tensor. 
% (b) CuSparse does not offer edge-ID indirection, hence DGL first re-arranges the edge-level tensors using the edge ID, called \textbf{eShuffle}, for each gSpMMve kernel invocation. {\graphpy} supports merges eShuffle inside its new gSpMMve implementation using edge ID in its graph storage.  (c) DGL does \textbf{two additional transposes} using CuBLAS library because CuSparse API that DGL uses expects tensors in column-major layout. 
% %Here is a comment from its code base re-produced almost verbatim that explains the rationale: “\textit{We use CuSparse to perform the following operation: C = A x B, where A is a sparse matrix in CSR format, and B is the dense matrix for the node feature tensor. However, since CuSparse only supports column-major, while our tensor is stored in row-major, the actual computation is: C = trans(A x trans(B)). Currently, we use CuBLAS to implement transposition and allocate intermediate workspace memory for this.}''.
% (d) CuSparse API does not fuse normalization by degree array; hence, DGL calls normalization separately using PyTorch API in Python. {\graphpy} gSpMMv kernel is written using template meta-programming which uses normalization as a template parameter and hence can handle both cases efficiently. 

% \textbf{3. No Transpose and Shuffle Kernels.}
% \red{Unlike existing works, {\graphpy} removes the need for some computations by re-defining the computation kernel. For example, In both the class A and class B type of GNN models, {\graphpy} avoid the need to transpose on vertex-level features as our gSpMM variants support row-major operations directly.}
% % For both the GNN classes, we avoid the need to transpose on vertex-level features as our gSpMM variants support row-major operations directly.
% %For class A type of GNN, Without integrating with CuSparse, GraphPy can omit the requirement that the input should be column-based. Therefore, two additional transpose computations are not needed. 
% %By removing these additional computations, our end-to-end time does speed up. 
% For the class B type of GNN, GraphPy introduces an edge ID directly as an edge property in the graph using DType, and gSpMMve uses the edge ID directly in the computation. Hence, it also removes eShuffle kernel. By removing this kernel, we do not need to materialize the shuffle output.

% \textbf{4. Kernel Fusion with careful investigation}
% Although existing works fuse several kernels to improve the performance, they~\cite{wang2021gnnadvisor,huang2021understanding,fu2022tlpgnn} fuse the kernel wrongly. By realizing these issues, 
% {\graphpy} fuses the kernel carefully by understanding the requirement from an end-to-end systems perspective.  For example in GCN, {\graphpy} performs the aggregation first and then normalizes the result with the degree array in the forward direction. However, in backward, {\graphpy} normalizes the input tensor first and then performs the kernel computation. 
% Similarly, for gSpMMve, {\graphpy} implicitly fuses eShuffle and gSpMM computation.
% %Therefore, {\graphpy} can be viewed as the improved baseline. (\td measure our way is slow. Gnnadvisor is wrong but fast)



% \subsection{Optimizations}
% \label{sec.optimization}

% % \begin{figure}[h]
% %   \includegraphics[scale= 0.5]{result/mul_graph.pdf}
% %   \caption{Supporting sparse models need for multiple graphs. It can also be a bipartite graph, such as layer parameters of sparely connected layer.}
% %   \label{fig-mul_graph}
% % \end{figure}

% % It should be noted that this specific kernel is also a from of SPMM, but it is truly SPMM unlike the weighted aggregation that is used in GAT. Specifically, in GAT, the vector feature vector of each vertex is multiplied with a scalar attention score of each edge before aggregation (which is more like SpMV). But in sparse connected layer, it is truly SpMM where input dense matrix is multiplied with sparse tensor matrix.


% The focus of the paper is on the interface design, and abstraction of common tasks to independent modules, however we do implement some known parallelization strategy, which makes our kernel implementation different than DGL and Pytorch Geometric (\cref{sec.exp}). We also propose following new optimizations to demonstrate that new optimization can easily be implemented.

% \noindent \textbf{Edge ID Reordering.}
% We observe that sparse version of fully connected layer and GAT, both keep edge-level tensors or weights, which is used by forward computation, and accepts gradients during backward. This is different from traditional graph analysis where edge does not need to materialize the edge level messages. So, the performance is sensitive to how the edge IDs are allocated to the edges to avoid performing random read and write to edge level tensors. Current allocation scheme is to allocate edge IDs sequentially based on edge log, which results in random edge IDs in both the CSR and CSC, as both are involved in the computation.
% % However, we can only provide sequential edge ID in one of them. 
% We propose reordering the edge IDs in CSC to allocate them sequentially. That is, the in-neighbor list of vertex 0 was allocated edge IDs from 0 to N(0) (the length of in-neighbor list of vertex 0). Similarly, the in-neighbors of vertex 1 was assigned from N(0) to N(0)+N(1), and so on. 
% % Thus, edge IDs in CSR became random. 
% We were able to achieve this easily by writing a custom code inside $wrap\_graph()$ API of the kernel.

% We also have the option to regenerate COO format to provide it sequential edge IDs as per allocation in CSC. This was useful for SDDMM kernels to increase the parallelism. Hence, we are able to achieve sequential edge IDs in two of the graph formats, while prior works had sequential edge IDs only in COO, and not in CSR and CSC.

% \noindent \textbf{Kernel Fusion.}
% For GCN model, we observe that it performs tensor normalization by dividing the tensor elements with vertex degree. We fused this operation with the GCN's core kernel (gathering features of neighbors of a vertex to update the self). Kindly note that the order of normalization and gathering features changes in the backward computation compared to forward computation. Hence one must take care of this fact while fusing the kernel.

==> tex/impact.tex <==
%\section{GNN Training: Observation and Analysis} 
\section{Impact Analysis} \label{sec.impact}

In this section, we discuss the impact of these pitfalls. We include how these pitfalls affect the realistic performance when deployed. Moreover, we categorize these pitfalls into different levels of pitfalls based on their severe degree. Table~\ref{table-pitfall} shows the result. (\td not dangerous pitfalls make our paper weak. we can say that section 5 is not comprehensive long-term thinking, it is piece-by-piece works, lacks of unifying end-to-end system-level pipeline thinking )



\begin{table}[t]
\small
%\vspace{-6pt}
\caption{\small category the pitfalls based on their severe degree.} % title of Table
\vspace{-6pt}
\centering % used for centering table
\begin{tabular}{|l| r|r |r|r|} 
    \hline\hline 
    %heading
  %  \cline{2-7}
    Pitfalls & normal & dangerous  \\
    \hline % inserts single horizontal line
%    Cora & 1,719 & 1,349   & 1,719 &1,375 &&\\ 
%    PubMed & 1,767 & 1,395  &1809& 1,503 && \\
%    Citeseer& 1,697&1,381   & 1,759 &1,409 &&\\ 
    P1 &  & \checkmark \\
    \hline 
    P2 &  & \checkmark \\
    \hline 
    P3 & \checkmark &\\
    %OGB-Pr & 25,551 &OOM & 20,789 & OOM  &32,285& OOM\\
    % & 76.47 &  76.52 & & \\
    \hline %inserts single line
\end{tabular}
%\vspace{-6pt}
\label{table-pitfall} % is used to refer this table in the text
\end{table}


==> tex/intro.tex <==
%{\color{red}


\section{Introduction} \label{sec.intro}
%Getting insights from data is very important, and hence 
Many applications have become data-driven today. 
%These applications are now popularly known as \textit{data science}. 
Within this ecosystem, a lot of real-world data can be stored as \textit{sparse matrices} or \textit{graphs}, such as social networks, chemistry, biology, recommendation system, scene description generation, knowledge bases, etc~\cite{fan2019graph, zitnik2018modeling, schlichtkrull2018modeling,hamilton2018embedding,ying2018graph,krahmer2003graph,perera2017recent,rgcn2018,wang2020entity}. 
%We call these data-driven use-cases as \textit{graph data science} 
To this end, many graph neural network (GNN) models, e.g., GCN~\cite{gcn17iclr}, graph attention network~\cite{gat18iclr}(GAT), GIN~\cite{xu2019powerful}, and others~\cite{gatedgraph2017,zhang18, graphsage17}, etc. have been proposed. 



% \noindent \textbf{Deep Learning on Sparse Data.}
% The neighborhood in graphs is different from other regular data, such as an image which has a fixed number of neighborhoods. To handle it, \textit{graph neural network}(GNN), has been proposed~\cite{gcn17iclr,gat18iclr,gatedgraph2017,gaan2018}. The GNN models can be trained efficiently if the graph can be used for storage. However, the current DL frameworks, such as PyTorch~\cite{pytorch2019} or TensorFlow~\cite{tensorflow2016} lack the same level of operational support for the sparse matrix that they have for dense matrix, as the original code-base of GCN~\cite{gcn17iclr}, GAT~\cite{gat18iclr} etc. have relied on bitmask at Python level to model sparsity on top of dense matrices that actually do not reduce computation or memory consumption. %because the underlying kernel still uses the dense matrix.


% traditional GNNs use the adjacency matrix to represent the graph structure and tensor operation to perform the forward and backward computations. 
% However, due to the sparsity, this will trigger the out-of-memory problem to represent a sizeable sparse graph and will cause computation inefficiency for tensor operation. 

% Since deep learning techniques can achieve excellent prediction, many graph neural network (GNN) works were proposed. Graph neural network (GNN) is about applying deep learning algorithms on the graph structure to do classification and prediction tasks, such as node classification, edge/link prediction, and graph classification. 
% The node classification denotes that given a graph structure and a subset of nodes with labels, the graph deep learning algorithm should predict the label of the remaining nodes. 
% In contrast, the link prediction tasks are predicting whether an edge exists between two given nodes or not, such as in auto-completing knowledge bases.


% \noindent \textbf{Deep Learning On Sparse Tensors.}
% DL Model compression techniques, such as weight pruning ~\cite{han2015learning,han2016iclr},  convert a dense model layer to a sparse layer by removing a lot of low-impact model parameters. 
% These techniques help to deploy large models on resource-constrained devices because the compressed models need less memory and CPU. Before deploying them, the compressed models undergo \textit{re-training}. This re-training step can be more efficient if the graph is used to model sparse layers. However, prior works~\cite{han2015learning} used bit-mask matrix in Python, and underlying dense matrix to achieve sparsity. Thereby, the \textit{re-training process did not really consume less memory}, hence we may not be able to use resource-constrained systems to do re-training, which are low on memory.

%These models also have inspired a number of systems optimizations~\cite{wang2021gnnadvisor,huang2021understanding,gespmmsc2020,fu2022tlpgnn,wu2021seastar,chen2020fusegnn}. However, our study finds that many of these design decisions indicate inadequate understanding because 

It should be noted that GNN is a special kind of deep learning (DL) model, and hence its training has a unique computation need. \textit{Forward computation} calls many \textit{kernels} (operations on data) from the input layer to the output layer to derive the prediction values which are compared with the ground truth to calculate the loss.
% and plug the loss into the backward procedure. 
Then, \textit{backward computation} uses the loss to derive the gradient by invoking kernels from the output layer to the input layer to update the model parameters.
%It uses the chain rule of gradient back-propagation to update the model parameter from it. 
Kindly note that the backward computation accesses results that are either accessed or produced in the forward computation and are called \textit{state tensors} (Fig.~\ref{fig-format}(a)). This computation paradigm differs from the prior forward-only related fields, e.g., graph analytics.
 
\noindent \textbf{Motivation: Missing End-to-End Focus.}
 Many prior GNN system optimization works~\cite{wang2021gnnadvisor,huang2021understanding,fu2022tlpgnn,wu2021seastar, chen2020fusegnn, kim2022analyzing,yan2020hygcn,liang2020engn,zhang2021boostgcn, geng2020awb} have established a clear trend of not measuring the GNN training accuracy, and many have only implemented forward computation.
%Many prior works either do not provide a full GNN model for training or do not measure training accuracy, 
Our analysis shows that it has led to significant practical issues, including questioning their proposed optimization techniques as presented next. %including the

Consider the case of the GAT model that calls 18 kernels in each layer~\cite{fu2022tlpgnn} in its forward computation. An obvious optimization technique is to fuse them into just one, as done by prior works~\cite{fu2022tlpgnn,huang2021understanding}. However, they have not implemented backward computation. The absence of end-to-end focus allowed them to avoid materializing the edge-level tensor($W_e$, a trainable GAT model parameter), and thereby not keeping edge ID(\cref{sec.background}) in their graph to access the same. 
Similarly, GNNAdvisor~\cite{wang2021gnnadvisor} does not measure the training accuracy. We point out that its codebase does not fuse the kernel correctly in the backward computation of GCN, and its model does not use bias, a vital model parameter, gaining performance unknowingly at the expense of accuracy. 

Hence all their demonstrated optimizations are not yet practical and require more investigation to implement backward computation to show training accuracy, which is likely to alter the very basic foundation of many proposed optimizations.
%Such additional steps would have enforced a brainstorming around the need for \textit{state tensors} and other GNN-specific requirements. 
%Fused kernels that avoid producing such tensors in the forward computation must implement backward computation to show that such fusion is feasible and justify them through training accuracy measurements.
%do not understand the system requirement from the GNN perspective. 
%Unfortunately,
%Hence, their optimization has no significance at this moment. We present various such observations in \cref{sec.obs}, however, the pressing question is whether such optimizations really advance the state-of-the-art. 
%and whether these mistakes are systematic.


%Further observations point us that many researchers do not understand GNN workflow exactly
%For example, 

%GE-SpMM~\cite{gespmmsc2020} forgets to consider the edge-level tensor when implementing the kernels. Section (\td) explains this analysis in detail. 



%\noindent \textbf{Systematic Lack}:
%We argue that these mistakes are systematic in nature. We present the following arguments to explain it. 

% No architecture papers \cite{yan2020hygcn,liang2020engn,zhang2021boostgcn}
%{\td  \cite{zhang2021boostgcn, geng2020awb, yan2020characterizing} only for inference and no accuracy}: Will see them later whether to include or not.
%\cite{baruah2021gnnmark} uses dgl and pyg, so not citing here.

%--------------
%(1) \textbf{No Training Accuracy Measurements and/or Missing Backward Computation.} 
% Indeed many prior works~\cite{wang2021gnnadvisor,huang2021understanding,fu2022tlpgnn,wu2021seastar, chen2020fusegnn, kim2022analyzing} do not measure the training accuracy either because they do not implement the backward computation or simply do not measure it despite having an end-to-end implementation.
% Hence, they may be totally unaware of the mistakes. 
% For example, GNNAdvisor~\cite{wang2021gnnadvisor}, and end-to-end GNN system does not fuse the normalization kernel correctly in the backward computation, while omitting the bias parameter from each GCN  layer (\cref{sec.obs}).
% %provides a more detailed analysis for this example). 
% Similarly, Huang et al~\cite{huang2021understanding}, and TLPGNN~\cite{fu2022tlpgnn} optimized the GAT model's forward computation without implementing its backward computation due to which they committed serious mistakes of wrongly fusing the kernels, including removal of edge-level tensors. Wrongly fused kernels can also alter the requirement significantly as they do not keep edge ID in their graph to access the attention score tensor in GAT(\cref{sec.obs}).


%Clearly, the research community has also not forced these works to measure training accuracy. 

%in form a natural boundary across which they cannot be blindly fused in the forward computation as they are needed in the backward 

% (2) \textbf{No Backward Computation.} Many prior works~\cite{huang2021understanding,fu2022tlpgnn}[\red{what about seastar and other works}] have not implemented a backward computation at all, and their optimizations focused on only the forward computation due to which they committed serious mistakes of wrongly fusing the kernels, including removal of edge-level tensors. We believe general awareness of GNN workflow and understanding is lacking, such as the need for \textit{state tensors}. Kernels producing such tensors form a natural boundary across which kernels cannot be fused in the forward computation. Wrongly fused kernels can also alter the requirement significantly. For example, Huang et al\cite{huang2021understanding}, and  TLPGNN\cite{fu2022tlpgnn} do not keep edge ID in their graph to access attention score tensor in GAT(\cref{sec.obs}). %(Section {\td} provides a more detailed analysis for this example). 
% %This mistake will be realized easily if these works implemented the backward kernel.
% % (3) One of the observations from such works is that they try to write GNN systems from scratch using current DL frameworks, such as PyTorch, TensorFlow, etc. 

% We explore the current methodology and find that it is very complex to write a GNN system from scratch because  passing the graph object and tensors to an independent module is very complex, and on top of this, users have to learn new build systems (Ninja), Python binding, memory management (due to delayed free of state tensors), etc. to integrate their code with a DL framework. We experienced the same issues ourselves when we tried to build a new baseline that resulted in exhaustion in just setting up the system. And, hence such exhaustion may force the researchers to not build an end-to-end system. 


%\noindent \textbf{End-to-End Systems Teaching.} 
%The academic community is also not encouraging end-to-end \textit{system} teaching. E.g., publicly listed assignments on DL/GNN {systems} courses offered by many universities~\cite{dlsCMU, cs15884CMU, cse599wWashington,cs231nStandford} \textit{focus only on the forward kernel} of an operator, and in Python without its integration in an end-to-end DL/GNN system. Hence, students cannot fully understand, appreciate, and gather complete requirements. Rather, industry partners have voiced concern about the availability of candidates with good systems and data science knowledge in an NSF workshop~\cite{storage2025NSF}.


%On the other hand, writing a GNN system from scratch gives the new system an immediate performance advantage, and we empirically show that prior work has been implicitly removed once other works develop a GNN system from scratch rather than integrating with DGL. can achieve performance improvement easily without any actual systems optimization. 

\begin{figure*}[t]
  \includegraphics[scale= 0.55]{result/edge_id_crop.pdf}
  \vspace{-12pt}
  \caption{\small (a) One GNN layer using GAS (gather-apply-scatter) to model the kernel: X and Y are intermediate features, and $W_e$ is the model parameter of the layer, e.g. attention score in case of GAT. X, Y, and $W_e$ tensors are \textit{state}, as they are used in backward. $A$ and $A^T$ are graph and its inverse respectively. (b) Sample graph (c and d) CSR and CSC representation along with edge ID indirection.}
  \label{fig-format}
 \vspace{-12pt}
\end{figure*}



\noindent \textbf{Contribution.}
This paper, called \textbf{\graphpy}, presents our observations that system optimizations based on a partial understanding of the GNN model may not lead to a practical system. {\graphpy} highlights the need for end-to-end model implementation to measure accuracy before showing the performance gain. 
To this end, {\graphpy} presents an ecosystem to perform it productively, and have following contributions. 

% focuses on two goals:
% (1) Writing a new GNN baseline by focusing on overhead reduction.
% (2) Explaining the critical pieces of the resultant architecture that has been extracted to develop an education and research tool to encourage the implementation of end-to-end DL/GNN systems. A detailed explanation of these contributions is below.


\noindent
\textbf{1. In-Depth Analysis (\cref{sec.obs} and \cref{sec.usecase}).}
We are the first ones to analyze existing GNN system optimizations, the current practices to integrate GNN systems to a DL framework, and the interfaces between GNN systems and the low-level GPU kernel implementation. A brief summary is provided here.

\noindent $\bullet$
\textbf{Accuracy and Performance Benchmarking.}
We observe many critical benchmarking issues due to missing end-to-end model implementation, and the absence of training accuracy measurements. 
{We also point out that relying exclusively on smaller datasets to show performance gain as done by prior GNN systems~\cite{wang2021gnnadvisor,gespmmsc2020} does not compare the impact of kernel performance but rather compares \textit{framework overhead}. To this end, we are the first to develop a  \textit{methodology} to measure the framework overhead. Overall, the investigation {questions the practical aspects of many proposed optimizations}.
%These issues also make DGL~\cite{dgl2019} the only end-to-end reliable \textit{baseline} that can be used to quantify the performance of future GNN systems. despite claims in several recent publications~\cite{wang2021gnnadvisor,huang2021understanding,fu2022tlpgnn,gespmmsc2020, wu2021seastar,chen2020fusegnn,featgraphsc20}. 
%These issues lead to two important use cases for which several interface-level limitations exist today as explained below.
%The full model implementation and accuracy measurement is needed to show the correctness of the developed kernel.  

% \red{\noindent $\bullet$
% \textbf{Framework Overhead Analysis and Methodology.}
% We are the first ones to state that the performance evaluation should rely on large data sets instead of the small data set because the overall training time in small data sets is dominated by the GNN system's framework overhead. Based on this observation, we also propose a methodology that can evaluate the framework overhead.}

\noindent $\bullet$
\textbf{DL Framework to GNN System (high-level) Interfaces.} End-to-end prototyping is needed to measure the accuracy to avoid the mentioned issues. But current DL frameworks do not allow passing any custom object, such as a graph to GNN systems, leading to reliance on workarounds for integration. This results in unstable system APIs whose signature changes for every custom graph storage. It deters innovation in graph storage and causes productivity and compatibility loss. %Hence, prior tools do not encourage end-to-end GNN system development.
%tensors to an independent module is very complex,
%out that a few GNN systems have critical issues in understanding system requirements, implementation 
%(a) The performance improvement stated in many prior works is not useful and prohibits their deployment to real-world GNN applications.
%{(b) Need of a Better GNN Baseline:}
%In this work, we observe (\cref{sec.obs}) many such issues in existing works, including an absence of end-to-end model implementation, avoiding training accuracy measurements, etc. 
%As we study code base of prior works and evaluate their work, we find that the optimization achieved by these works cannot be relied upon as they do not fully implement the GNN model correctly. Hence, 
%they would have benefited by following our recommendations such as enforcing GNN training accuracy, and using larger datasets for performance measurement.
%Similarly, assignments and tools should be developed to impart an end-to-end understanding of DL/GNN systems to future systems researchers and engineers.
%while the performance measurement should happen on larger datasets.


\noindent $\bullet$
\textbf{GNN Systems to CUDA kernel (low-level) Interfaces.}
CuSparse library defined general-purpose sparse kernels over a decade ago. However, it is not directly suited as kernels for GNN use cases. This low-level interface mismatch introduces extra memory allocation, additional kernel calls, and the materialization of intermediate results causing a slowdown and increased memory consumption in DGL. However, others~\cite{gespmmsc2020,featgraphsc20,huang2021understanding} continue to optimize the same kernel definitions and suffers from the cost of generality and mismatch.

\noindent
\textbf{2. Research Tool (\cref{sec.usecase} and \cref{sec.science}).}
To this end, {\graphpy} \textit{auto-generates codes to integrate GNN systems to DL frameworks} based on a simple domain-specific language. 
%users to write the kernel, called \textit{\graphpy-Kernel} independently without involving any DL frameworks, and have no version dependency whatsoever. {\graphpy} 
It relies on a proposed \textit{Half DLPack protocol} to offer DL framework-specific tensors to GNN systems using flat arrays. This achieves DL framework-independent GNN system, which in turn, removes all restrictions on passing graph objects to it. Further, {\graphpy} proposes \textit{graph storage management} module to prepare and export graphs to GNN systems as per GNN-specific graph edge property requirements. 

Through these mechanisms, {\graphpy} achieve \textit{productivity and re-usability} of GNN system across DL frameworks and their versions and also streamlines the interfaces for graph handling.
Further, we are unaware of any system that can support arbitrary multi-field edge properties. It also cannot be designed without significant innovations.

%The proposed tool also reduces the framework overhead due to its simplistic design. 

 
%\bullet$
%\noindent
%\textbf{3. Graph Storage Management (\cref{sec.engg}).}
% Analyzing different GNN models shows the need for graph storage with different edge properties. The current ad hoc approaches to handling graph storage present another productivity issue and a challenge to interface design and system integration. 
% We separate the graph storage management to another independent module to prepare graphs by specifying GNN specific edge properties succinctly using a single API. The API exports the prepared graph using \textit{zero-copy} arrays to the GNN system. 
% We are unaware of any system that can support arbitrary multi-field edge properties. It also cannot be designed without significant innovations.

%to satisfy the diverse storage needs of various classes of GNN, which cannot be supported by current tools.
%to achieve better performance in graph preparation and productivity in
%By relying on  Dtype, {\graphpy} makes sparse matrix (i.e., graph) same as dense matrix (e.g., image data) for storage specification and exchange purpose. 
%Interface design leaves enough room in {\graphpy-Kernel} to innovate on graph storage design without impacting {\graphpy-SM}.


% $\bullet$
\noindent
\textbf{3. GNN Inspired Kernels and an Optimized Baseline (\cref{sec.baseline}).}
We capture the system requirement using a new set of kernel definitions  that can directly be used inside GNN systems without any requirement mismatch and memory overhead. 
Based on these new kernels, we present a new GNN baseline 
%by removing the various overheads and fusing the kernels by carefully studying the GNN models
ensuring correct training accuracy and better performance amid low memory consumption. 


%presents much more than memory and performance optimization. It rather establishes a new  

% \noindent $\bullet$ 
% \textbf{Graph Data Management for DL.}
% We separate the graph storage management to another independent module, \textit{\graphpy-SM}, to handle multi-field graph properties using a single set of API by using \textit{NumPy Dtype}, while exporting the prepared graph storage to {\graphpy-Kernel} using \textit{zero-copy} NumPy arrays. 
% %and allow innovations in interface design
% By relying on  Dtype, {\graphpy} makes sparse matrix (i.e., graph) the same as a dense matrix (e.g., image data) for storage specification and exchange purposes. 
% Interface design leaves enough room in {\graphpy-Kernel} to innovate on graph storage design without impacting {\graphpy-SM}.
% We are unaware of any high-performance Python package that can support arbitrary multi-field graph properties. It also cannot be designed without significant innovations(\cref{sec.engg}).

%We demonstrate the usefulness of {\graphpy} with the implementation and evaluation (\cref{sec.exp}) of many GNN models. 
%on an average 1.64$\times$ and 1.42$\times$ speedup and 1.30$\times$ and 2.29$\times$ speedup over DGL, and PyTorch Geometric for various GNN models in GPU and CPU respectively. 
%Further, frequent out-of-memory conditions by DGL, Pytorch-Geometric, and GNNAdvisor force measurements to be performed on smaller dataset only. Measurements on smaller prevalent dataset do not show advantage of kernel optimization due to framework overhead.

Our evaluations (\cref{sec.exp}) show that {\graphpy} reduces memory consumption on average by 6.92$\times$ on GCN, 3.4$\times$ on GIN, and 1.96$\times$ on GAT-1 models in comparison to DGL, while DGL, Pytorch-Geometric~\cite{pytorchg2019} (PyG) have many out-of-memory conditions. 
Further, {\graphpy} achieves on average 1.38$\times$ 1.51$\times$, 1.58$\times$, 1.32$\times$ speedup for GCN, GIN, GAT-1, and GAT-3 compared to DGL on larger datasets. 
We also show that GNN-specific kernel definition alone without any workload balancing technique can perform much better (1.16$\times$ -- 2.95$\times$) than optimized and workload-balanced generic kernels of FeatGraph~\cite{featgraphsc20}, GE-SpMM~\cite{gespmmsc2020}, GNNAdvisor~\cite{wang2021gnnadvisor}, and Huang et al~\cite{huang2021understanding}, which can not be run end-to-end along with CuSparse and DGL.
Lastly, focus on interface design minimizes the framework overhead of {\graphpy} by 1.54$\times$, and 1.35$\times$ than DGL and PyG.
%to achieve better performance on smaller datasets. 

%To show the extensibility of {\graphpy}, we also demonstrate the implementation of sparse tensors (not sparse data) on LeNet-300-100.

%Therefore, future systems optimizations can benchmark their performance against our baseline to advance the state-of-the-art rather than comparing against various overheads.

%Empirical evaluations show that our optimized implementation achieves 1.62$\times$ and 1.35$\times$ over DGL and PyTorch for various GNN models on many datasets in GPU, and 1.55$\times$ and 1.88$\times$ on CPU respectively with similar accuracy readings.\td[end]
%\footnote{See \url{https://arxiv.org/pdf/1909.01315.pdf} for DGL overhead} 
%making {\graphpy} an excellent framework for research. 
%A better GNN performance using the reference implementation, less framework overhead, and low memory consumption make {\graphpy} an ideal baseline for performance benchmarking for future research. 


% The remainder of the paper is organized as follows. We present background on graphs and DL in \cref{sec.background}. 
% %The motivation, challenges, and overview of {\graphpy} are presented in \cref{sec.overview}. 
% The detailed use cases are presented in \cref{sec.after_observation}, technical challenges and prior works in \cref{sec.challenges}.  Implementation details are presented in \cref{sec.science} and \cref{sec.engg}, evaluations in \cref{sec.exp}, and we finally conclude in \cref{sec.conclusion}.


The paper specifies many practical issues with GNN systems and provides a practical yet powerful framework to overcome those issues. 
More importantly, the proposed baseline allows {\graphpy} to train GCN on a billion-edge graph on a single GPU due to memory saving while prior works cannot train even a 500 million-edge graph. 
The new baseline also offers  newer opportunities for practical optimizations. 
%where {\graphpy} offers researchers a powerful mechanism to design end-to-end systems productively. 
Indeed, there is an immediate scope for optimizing the proposed GNN-specific kernels through various format-specific and workload-balanced designs that can be compared against the proposed baseline to show the practical impact.
Lastly, the proposed tool and mechanisms may be used for end-to-end system education to train learners on system requirement gathering for GNN/DL models and implementation, which has been flagged as a major concern in an NSF workshop~\cite{storage2025NSF}. 


==> tex/new_added.tex <==
\section{New added sections} \label{sec.new}
\subsection{Research aspect}
Many existing works, [GNNadvisor, zhai, gespmm, ] mainly focus on optimizing the kernel implementation. (TODO GNNadvisor has a python model, zhai has a simulated GNN). However, based on our analysis, we are the first one to find that kernel implementation alone is not sufficient enough for system research to avoid mistakes and improve end-to-end DL training time.
The following sections will provide more details to support our findings. 
 
\subsubsection{End-to-end training is needed in GNN systems}


\textbf{Without end-to-end training, many implementation requirements are ignored by the researchers}
 
 
Different classes of GNN(GAT, GCN and GIN)
The GNN models can be classified into different classes based on their aggregation method. The GNN models which have unweighted sum aggregation are one class, such as GCN and GIN. The GNN models with the weighted sum aggregation method is another class, such as GAT, etc(todo we can cite more attention-based paper) Because of the aggregation difference, different types of GNN models have different system-level implementation requirements.  



Edge id indirection is needed, (Copy from 2d-snb)
As we mentioned in the background, Attention-based GNN models use attention(importance) scores to aggregate the neighbor values. Attention-based GNN models first generate the O(E) level attention score A. In the aggregation process, 

 Given a target node i, the model first fetches the attention score $A_{k}$ of its neighbors ($k \in N(v)$), then aggregate by sum$(A_{k} * H_{k})$ to updated the $H_{i}$. This process will be iterated until all nodes’ embedding is updated. This updated H will be used for the later computation. 

In the forward process, the kernel fetches the A by the normal graph order and performs the later computation, and saved it for the backward computation. 
In the backward process, the kernel needs to reload the saved A and fetch it again but in the reverser graph order. 
Here the problem comes, Since the graph is now reversed, the order of the edge list now is different than its order in the normal graph. If we still use the forward fetching order to fetch the A in the backward process, each attention score $W_{k}$ will be wrong. The incorrect fetched $W_{k}$ will cause a wrong backward computation, which corrupts the whole model training process.
While this  problem can also apply to compressed layers. E.g., in weight-pruned fully connected layers, as shown in Fig.~\ref{fig-prun}, the data is the dense matrix and the layers are sparse matrices.
To solve this problem, it is mandatory to maintain the edge indirection property so that  the kernel can fetch the correct $W_{k}$ in both the forward process and the backward process.

Zhai -- GAT problem
(copy from 2d-snb ended)
 
The corresponding DGL kernel of this computation is ‘gspmm’. To support this requirement, DGL provides an extra shuffle kernel to reorder the edge id list each time before fetching the edge score tensor. After that, DGL transposes the input tensor and uses the cusparse library to perform the computation. This extra shuffle kernel, transpose computation, and the system overhead time between them lead to extra time cost at the end-to-end training process. (todo find the line of code with shuffle + gspmm) 
If the requirement(above process) is not fully understood by researchers, even if they replaced the cusparse library with an optimized kernel, the overall end-to-end training process will not be optimized. 
Hardly do these previous papers discuss this edge id indirection requirement. Instead, Their kernel implementation can only support specific types of gspmm, such as GCN and GIN. 
 

Zhai’s work does not consider this requirement when implementing the kernel also. It fetches the edge tensor in sequence, this incorrect fetching will lead to the wrong aggregation result.
Although the integration between the kernel and the GNN model is correct, the overall simulated GNN has Some mistakes. (todo Not sure what this problem is: Input tensor and output send them as the same tensor)
Because of these mistakes, even if the simulated end-to-end training time shows improvement, this result is not trusted and cannot represent real-world GAT training. 
Gespmm forgets to consider edge id indirection also.

Therefore, if the researchers only focus on kernel implementation, it is likely for them to ignore some requirements and make some mistakes.
With an End-end training platform, it becomes easy to let researchers know that some extra requirements, such as edge id indirection property, needed to be taken care. With understanding this requirement, researchers are free to follow the DGL solution or propose their own solution. 


\textbf{Implement kernel only can cause end-end training accuracy problem}

Firstly, without end-to-end training, the kernel implementation may be incorrect.
One straightforward example is forgetting to meet some extra requirements we mentioned above(in the above section)
Secondly, even if the kernel implementation is correct, the overall training loop may be still wrong. For example, GNNadvisor implements it’s gspmm kernel alone correctly. But its experiment shows in (todo section ) show that it does not achieve correct accuracy. That is because it does not fuse the normalization computation with the gspmm kernel correctly for the backward process. In the backward process,  the fused kernel should do normalization first and then perform the aggregation.
(\todo zhai problem and gat)




To sum up, existing GNN system level optimization works, GNNadvisors, zhai, gespmm read the DGL code base to understand the requirement. ( need some reference email them) 
However, GNN model works, such as GCN, and GAT(these papers just provides the basic mechanism of the dense matrix) and GNN System works, such as DGL do not provide clear system-level requirement description. It is not guaranteed that all people can understand them correctly. Examples in the above section (todo list GNNadvisor, zhai, gespmm citation here) show that even researchers may ignore some requirements easily. 
 
Therefore, these requirements are very important in GNN systems but none of the Previous works explain them in the paper.  We are the first one to explain these requirements and illustrate their importance. We also state that with an end-to-end training platform to test the accuracy, these ignored requirements will be found. 

\subsubsection{A baseline is needed in GNN system area}


\textbf{End-to-end training time is controlled by overhead}

Our experiment in section (todo) shows that existing GNN systems, DGL, PyG have large overhead for the small data sets. To be more specific, the end-to-end training time is controlled by system overhead.
This large overhead has two negative effects. Firstly, since the work that implements most computation in cuda and c++ can avoid the system overhead and achieve huge end-to-end improvement, it is hard to measure the real effectiveness of performance improvement for these types of works. We do not know whether the improvement comes from the c++, cuda implementation, or the optimization techniques mentioned in these works(such as graph reordering, techniques to improve data locality, and better parallelism).

Secondly, the large overhead misleads the potential optimization directions for researchers.
That is because most researchers verify the effectiveness of their optimization techniques by performing an end-to-end training on small datasets.
In that case, the end-to-end training time will not change even if the kernel is optimized well, 
To solve this problem, GraphPy was optimized to achieve a small overhead so that the Kernel improvement can play more role in the end-to-end training. 

\textbf{Overhead neutralize the effectiveness of kernel improvement}
Besides the overhead on small datasets, framework overhead prohibits the improvement of the overall end-to-end training even if the kernel itself is well optimized. 
 
A straightforward example is DGL. DGL adopts the cusparse, an accelerated linear library optimized and provided by Nvidia over decades, as the core kernel for gspmm(mainly kernel used in GCN and GAT).
However, DGL’s gspmm kernel cannot achieve the same speed as cusparse. Instead, it has a 2 X, 3X slowdown compared with cusparse. (todo Test cuspare, and gspmm kernel in DGL to show the performace different in ogb dataset) 
That is because the gspmm in DGL is designed for both unweighted aggregation and weighted aggregation. It needs to apply one shuffle kernel each time before launching the cusparse to support edge id indirection(refer to next section). Moreover, since cusparse library can only accept column-level input, DGL needs to transpose the input tensor before using the cusparse library. These two more steps, shuffle, and transpose, cost some extra time. If the researchers just fuse these two steps together or remove the need for transpose for cusparese library and do not apply any optimization techniques, the end-to-end training time will improve a lot. 
 
But if the researchers do not understand these steps correctly, and design some optimized kernel to just replace the cusparse. Even if the optimized kernel is faster than cusparse, the end-to-end training time will not be improved. (todo not sure whether this DGL example is overhead or not)
 


(Todo Another example is the Gespmm, although its optimized kernel is faster than cusparse, after it integrated its kernel to DGL the overall training time does not have significant improvement. )



 
Our Experiment in section (todo), Figure (todo) also shows that even if our reference kernel gspmm is slower than cuspares, our GCN end-to-end training time achieves a (TODO) speedup compared to DGL among different datasets. 


(todo not sure Because of edge id indirection provided by our framework). Even if our kernel is slow alone, Our end to end training time still achieves huge speed up.
 
Therefore, Just focusing on the kernel implementation cannot lead to a good end-to-end performance. Moreover, since researchers study the kernels for more than 10 years, the new optimization mostly triggers an incremental improvement such as 10 percent - 15percent. From the above, we find that the end-to-end training time bottleneck comes from not only the kernel but also other parts.
 
Researchers need to understand not only just the kernel(The kernel here is different than the kernel in DGL, but not sure how to explain the difference) but also the other parts. This understanding can only be achieved by end-to-end testing. 

In that way, there is a need for an easily plugged-in platform to let researchers understand the roles of the kernels in the whole GNN training process. With a better understanding of the kernel role, researchers can implement the proper kernel which speeds up the overall training performance. 


\textbf{huge memory consumption causes problems}
As we know, DL needs to consume huge memory which will lead to a high energy cost. (citation to do takes 1-week energy of the whole city) Therefore, memory consumption becomes an important metric for DL systems. In this work, GraphPy provides a low memory consumption. It saves the number of E memory, which leads to 4 bits in GAT 1, and 12 bits in GAT3. For a graph with one billion edges, GraphPy saves 4 GB of memory. Moreover,  GraphPy can Save a number of vertex memory in features tensor compared to DG.L(todo add some details in interfaced design to explain).  In total, GraphPy can minimize 50% to 100 % memory consumption saving compared to DGL, which is a huge saving for energy costs. 
 
Another problem high memory consumption causes is graph splitting. For a large graph, the dataset cannot fit in a single GPU. Researchers need to split the large graph into multiple subgraphs and send them to multiple GPUs to do parallel training (todo citations). This multiple GPU setting makes the problem become more complex, and many concerns needed to be worried, such as how to synchronize the results, how to minimize the overhead, and how to optimize the communication between each split subgraph(Graph Partition is an NP-hard problem).
 
However, GraphPy provides low memory consumption to enable researchers to run GAT models on large datasets with a single GPU setting and avoid the complex multiple GPU problem settings. 


\textbf{Other problems with existing works}
Besides the overhead problem, there are other reasons that make the existing works cannot be used as a baseline.
As we mentioned in the above section, GNNadvisor has an accuracy problem in end-to-end training. It does not consider the edge id indirection at all so that it can only support a specific type of GNN model, such as GCN, GIN. It cannot work on another class of GNN, such as GAT.
Although zhai’s work supports GAT kernel, its kernel implementation is wrong because of the missing edge Id indirection. Moreover, Zhai’s work does not contain the end-to-end training loop. It is also impossible for researchers to implement a training loop by themselves because zhai’s work does not provide a backward process. 
Gespmm does not support edge indirection property either, which means that it cannot support GAT. 
PyG meets the OOM problem even for the median size data set. It also has a Large overhead for small datasets.
Therefore, none of the existing works can be treated as the baseline. 
There is a need for a Baseline in GNN systems, which is better than DGL in end-to-end training but does not include any novel opt techniques so that new optimization techniques can be added.

\textbf{Summary}
 
To sum up, wring the kernel alone is not enough. There is a need to provide a platform to let researchers really understand the kernel requirements and related topics.
 
To fix this gap, GraphPy focuses on interface design. By providing modular-based kernel, GraphPy
provides the opportunities and options system researchers can pursue which is not explored by the early framework.
 
To be more specific, the Kernel interface in GraphPy is not as simple as DGL expects. In the DGL, the core kernel for ‘gspmm’ is the cusparse kernel. To integrate with DGL, researchers can only implement new kernels to replace the cusparse. As we mentioned above, replacing cusparse cannot achieve end-to-end performance improvement.
However, GraphPy provides a more customized kernel interface so that researchers can decide whether they want to implement a new kernel that replaces all the above computations or just replace the cusparse. The optimized small overhead of GraphPy provides researchers the opportunity to check the effectiveness of the kernel in the end-to-end overall training.
(todo need to explain this part well. What is the difference between graphpy kernel and the DGL kernel? Not very precise What impact the overhead places here)


(todo Hardware evaluation. Or just kernel evaluation. (Possible for overhead analysis))



\subsection{Education aspect}
For education purposes, there are several educational attributes GraphPy provides.

\textbf{Just writing kernels in c++ or python is not enough}

The real-world GNN system[AWS, Azure, etc todo need citation] contains two aspects: c++/cuda based kernel implementation to provide fast speed computation and python-based wrapped kernel and GNN layers to let the data scientist customize their GNN models. 
 
 
 
 
 
 
The goal of the teaching is to let students understand both these two aspects.
 
Only teaching how to implement the kernel in c++/python is not enough. It is not just teaching students how to write the kernel and how to use pybind to wrap the kernel out in python.
Writing the kernel only cannot let students understand the exact requirement as we mentioned in the above research section. (todo cite the section number here) 
For example, GNNadvisor does not fuse the normalization and the computation kernel correctly in the backward process. But it is hard to explain this requirement to students on the kernel implementation. Only with an end-to-end system teaching, students will know this difficulty of kernel fusion. To be more specific, if we assign an assignment to let students fuse these kernels directly, students just implement the fused kernel without thinking of any requirement about this fusion process. 
But with an end-to-end system, the instructor can teach students these requirements and let them play with different kernel fusions and understand whether the requirement is satisfied or not from the accuracy. 
 
The existing platform does not provide an end-to-end system. They standford, berkely[need some citations] just provides pooling, softmax, batch normalization (not sure of convolutional layer) in the forward. Students still do not know how the backward process doing and how to use the wrapped kernel in an end-to-end training loop. 
 
It is hard for students to have a whole-picture view of how the GNN system works. With Graphpy, students can practice these steps and learn some practical tricky implementation techniques. And understand how each step works in an end-to-end training process.  This education training will help the students get a deep understanding of GNN systems, which will help them a lot in the future job market or academic research. 
 
Besides this, GraphPy also provides several educational attributes so that students can learn the GNN system easily.


\textbf{Easily plugged in kernel module}

In the GNN systems education teaching, there is a need to let the student write the kernel. However, this implementation process should be kernel focused only. That is because most students do not have enough background and time to explore the integration code and pybind wrapping technique.
GraphPy focuses on the interface design to provide the independent kernel module and auto-generated integration code to let students write the kernel easily and not need to learn the programming framework.


\textbf{Customized Python GNN layers}
Besides the kernel implementation, GraphPy wrappers the GAS kernel out in the python environment and provide the GNN model layers.
Students can modify them easily to learn the GNN models’ configurations and how the GNN model uses the GAS kernel.


\subsection{Graph system works cannot be extended to GNN}
Merril’s work handled the workload imbalance, which lead to a great performance improvement in spmv. However, it needs to preprocess the metadata first and use this metadata to do later things. These metadata structures cannot be passed to DL backends such as TF and Pytorch. (To do how to provide it cannot ). Many other works [citations] also rely on the preprocessed additional data structure.
 


\subsection{GraphPy can also work on unlabeled datasets}

For the unlabeled dataset, GraphPy can randomly generate the label for the training node id and test node id. With this synthetic label, these unlabeled datasets can be viewed as labeled dataset. 



==> tex/old_usecase.tex <==

\section{Old Use-Cases} \label{sec.extend}
There is always a need to write new layers and kernels either for research or education. 
%The focus on critical interfaces design, enabling plug-and-play architecture, 


\subsection{Research}
%keeping the {\graphpy-Kernel} independent of DL framework, light-weight due to available graph in CSR/CSC format, and 
% There are many factors that make {\graphpy} ideal for research prototype, specifically in graph domain. While \textit{productivity} remains an important factor that is achieved using generation of critical boilerplate code, and outsourcing of graph storage to {\graphpy-SM}; \textit{reusability} of Kernel code across many DL frameworks through automatic integration make {\graphpy} an ideal platform for developing re-usable kernel code.
%reusability of  research and education in graph data science. Further, the interfaces designed around tensor exchange are generic enough to use {\graphpy} in other DL use-cases and not just graphs. 
% Further, \textit{modularity} offerings of {\graphpy} ensures that unrelated use-cases can be housed in different modules, rather than following the monolithic approach of prior works,  yet  those modules can be combined with the benefit of flexibility and for variety of use-cases. Because of such reasons, {\graphpy} is able to support many isolated sparsity use-cases including sparse data for deep learning, sparse tensor for deep learning models which can be modeled using graph, as well as traditional graph data science use-cases. We have reference implementation for the same to demonstrate that it is possible.

% % Hence a third party module can easily implement those missing functionalities without writing the boilerplate code and use zero-copy data-sharing for graph and tensor both. 
% % %Anytime, there is a new release of DL framework, the plugin requires re-compilation. Worst, they are not distributed along with main binaries, but are highly depended on each version of their release.
% % Thus all the instances of {\graphpy-Kernel} module remains reasonably independent as far as development complexity is concerned. This makes it easy for learners to focus on system implementation to learn the system side of graph data science as the Python model code and interfaces remain same. 
% % On the other hand, advanced learners can write end-to-end model, including the logic to handle its backward computation, and kernel code utilizing the interfaces and DSL. This way, they can better understand the concept of model development, the role of backward computation and kernel in the overall DL workflow. 


% %Mobile app development has seen tremendous use-cases, because of well thought interfaces. 
% % Relying on DLPack tensor, and not asking for memory allocation/deallocation inside the GraphPY-Kernel makes the kernel development free from any limitation or additional works of third party tensor library. 



% %The novel design of {\graphpy} makes it becomes a general framework that can support multiple use cases easily. For the data level sparsity, although we highlight {\graphpy} can handle sparse data, it can handle dense data as well. Moreover, {\graphpy} also supports model level sparsity, which is not supported by existing works. 


%\subsubsection{Sparse Data}



\subsubsection{Sparse Data}  \label{sec.gnn-background}
Graph convolution network~\cite{gcn17iclr}(GCN), graph attention network~\cite{gat18iclr}(GAT), GIN~\cite{xu2019powerful}, GGNN~\cite{gatedgraph2017}, GaAN~\cite{zhang2018gaan} etc. are collectively called \textit{graph neural networks} (GNN) that specialize deep learning on graph data.
%The DL frameworks do not yet support sparse operations efficiently. Sensing the gap, a number of GNN frameworks were proposed recently, such as DGL~\cite{dgl2019}, NeuGraph~\cite{neugraph19atc}, AliGraph~\cite{yang2019aligraph}, Pytorch-Geomertric~\cite{pytorchg2019}, etc.
%GNNs ~\cite{gcn17iclr,gat18iclr, xu2019powerful,gatedgraph2017} are frameworks for representation learning on sparse data or graphs. 
%The forward computation uses a series of sSpMM and gSDDMM kernels. 
The trainable tensors in such GNNs can be at vertex-level ($X$ and $Y$); and edge-level ($W_e$ as attention score in GAT and GaAN. 
%and can be a vector as in case of multi-head attention. 
%In GAS forward, $W_e$ is calculated using a series of gSDDMM kernel, that takes various reduce operations of sum, min, max, etc in forward computation. Its one input tensor is a vertex-level, while the second input tensor can be either vertex-level or edge-level tensor. $W_e$ is used as edge weights (scalar or vector) in the gSpMM to calculate vertex-level tensor Y. In GCN, $W_{e}$ is absent in (unweighted) gSpMM. In its another variant, gSpMM only accepts an edge-level tensor to calcuate the output Y, and accepts various reduce operations.
Backward computation also invokes variations of gSpMM, and gSDDMM, and requires accessing the tensors produced during forward computation ($W_{e}$, $X$ and $Y$). Hence, they are saved as \textit{states}, as shown in Fig.~\ref{fig-forward}. 
Since, backward computation happens on the inverse graph (CSR), as opposed to using CSC during forward computation; the CSR and CSC  must share the same copy of the state tensors. This is handled by the vertex ID indirection for vertex-level tensors ($X$, $Y$), which is already present in the graph storage. However, for edge-level tensors ($W_{e}$), graph storage needs to introduce \textit{edge ID indirection} (Fig.~\ref{fig-format}). 
%For completeness, some gSDDMM kernel during backward does not need inverse graph.

\begin{figure}[t]
  \includegraphics[scale= 0.64]{result/gnn-crop.pdf}
 \vspace{-12pt}
  \caption{\small GNN Forward and backward mode: X and Y are intermediate features, and $W_e$ is the model parameter of the layer, e.g. attention score in case of GAT. X, Y and $W_e$ tensors are \textit{state}, as it is used in forward and backward both. $A$ and $A^T$ are graph and its inverse.}
  \label{fig-forward}
%   \vspace{-12pt}
\end{figure}





\noindent \textbf{Why end-to-end GNN system needed?}
This edge ID requirement for attention-based GNNs differentiates DL sparse kernels from prior works in sparse linear algebra and graph analytics.
Hence, if one only focuses on kernel optimizations without thinking of evaluating accuracy on an end-to-end training loop, it is very likely to omit edge ID requirements~\cite{huang2021understanding}. 
%Rather, we have noticed that a GNN performance improvement work~\cite{huang2021understanding} does not store edge ID in their graph storage for GAT. 
Such errors could have been easily found if the work integrated their kernel in a training loop, and measured the accuracy. Similarly, another GCN work~\cite{GNNAdvisor} did not use bias in its model. Both of these works are likely to over state the performance benefits in the absence of accuracy measurements due to omission of crucial requirements.

Therefore, instead of focusing on kernel optimization only, measuring training accuracy is needed, that can act as a feedback to researchers about correct implementation. 
%Further, such a framework will also show the true impact of better kernel design on the end-to-end training performance. 
%To satisfy this need, We propose an end-end system {\graphpy} that let researchers write the new kernel easily. The Independent and Auto-Integrated Kernel (\cref{sec.science.auto}) and graph storage GraphPy-SM (\cref{sec.engg}) make {\graphpy} becomes \textit{productivity}, \textit{reusability} and \textit{modularity}. which is an ideal end-end prototype for GNN system research.
Rather many techniques proposed by graph analytics systems~\cite{kyrola2012graphchi,roy2013x,nguyen2013lightweight,liu2017graphene,powerlyra2015eurosys,gstore, zheng2015flashgraph,mosiacEuroSys17, roy2015chaos, han2013turbograph, kumar2017falcon, zhu2015gridgraph,hong2012green, wu2015g, ai2017squeezing, zhu2016gemini,liu2015enterprise}, such as using specifically tailored data layout~\cite{zhang2015numa,gstore,libgraplus15DB}, graph-aware compression~\cite{libgraplus15DB,gstore}, fine-grained and workload-aware parallelism~\cite{liu2015enterprise,wang2015gunrock}, graph re-ordering~\cite{gorder16sigmod,rabbit16ipdps}, graph partitioning, etc. for CPUs and GPUs, could also be evaluated easily for GNN use-cases, if a platform can offer easier integration of system works to DL workflow.

\subsubsection{Support for Sparse Tensors}
Recent work on model compression, such as weight pruning~\cite{han2015learning,han2016iclr}, removes significant number of parameters from specific layers (e.g. fully connected layer) to achieve model/layer compression as shown in Fig.~\ref{fig-pruning}. Such techniques have enabled a number of large models to be deployed in resource-constrained devices. However, before their deployment, re-training is required to fine-tune their parameters. 

%\noindent \textbf{Different Sparsity.}
The sparsity in the model layers is \textit{different} from data sparsity. E.g., the sparse connectivity here requires bipartite graph, where the number of source and destination vertices sets are different. Further, multiple layers can be sparse in this case with each layer having its own bipartite graph. Also, the graph object is part of sparse tensor, and not sparse data. Finally, the computation in this case is more like traditional sparse linear algebra, i.e. SpMM and SDDMM. On a different note, edge ID is still needed, if it involves edge-level tensors as in sparsely connected layers (Fig.~\ref{fig-pruning}).

% Fig.~\ref{fig-pruning} shows the weight pruning~\cite{han2015learning,han2016iclr} intuition for a fully connected layer, where the resultant layer becomes sparsely connected, can easily be represented as graph. 
Re-training, like training process, is mostly done using in-memory system today. Hence prior works that have used ad hoc methods to re-train such models, such as using a bitmask matrix 
% the punned layer is now a combination of a dense parameter matrix and a bitmask matrix.  it 
will still use the dense linear algebra of DL frameworks to perform re-training, and uses the bitmask to only filter out the computation results on pruned weights. Clearly, this re-training still uses same memory consumption, and performs almost the same number of computation that would have been done using the original model.

\begin{figure}[t]
  \includegraphics[scale= 0.5]{result/pruning-crop.pdf}
 \vspace{-6pt}
  \caption{\small Model compression here converted two fully connected layers to sparsely connected layers after weight pruning, and can now be represented using bipartite graphs.}
  \label{fig-pruning}
 \vspace{-6pt}
\end{figure}




However, if we can model the sparse tensors using graphs, we can provide huge memory saving for tensor storage where sparsity level is high, and achieve reduced computation. Thus, we can enable their re-training and deployment in resource constrained devices.
% while sparsity is achieved using bitmask on the computed results.


%To fix this gap, {\graphpy} supports bipartite graph and sparse tensor easily by its novel design. 


% While the support for GNN is an important use-case that we support, we would like to highlight the support for sparse tensors to store model parameters using graph as an out-of-box feature of {\graphpy}. Support of sparse tensors are needed during re-training phase of compressed layers, such as a fully connected layer after weight pruning. The primary vision behind model compression is to enable re-training and deployment in resource constrained devices. Since, deep learning training and re-training process are mostly done in-memory today, Hence if the sparsity level of the sparse tensors are high, using graphs can provide huge memory saving for tensor storage. Thereby, {\graphpy} enables the usage of resource-constrained devices or simply reduces the hardware requirement. Further, decades of research in sparse linear algebra is likely to improve the re-training time when using graph to compute sparse kernels.
%The sparse model uses the weight pruning technique (Fig.~\ref{fig-pruning} in \cref{sec.background}) to convert the fully connected layers to sparsely connected layers.

% To support the re-training procedure of sparsely connected layers, we implemented biparatite graph, the sparse kernel, and the layer, and rely on generated code similar to Listing \ref{list-spmm} to handle bipartite graph and call sparse layer spmm() and sddmm() kernels implemented in the {\graphpy-Kernel}. 
%It should be noted that the graph is this case models the sparse tensors for which no support exists in any prior DL frameworks.

%On the other hand, DGL/PyG does not provide support for sparse tensors. Since, supporting it require two new kernels and corresponding interfaces (apart from supporting bipartite graph), we have to learn details of interfaces and internals of DGL/PyG, and still have to work-around the limitations. Such internal system details are missing from their documentation. Hence, it is likely to take huge effort to implement.
%So, interfaces are important, and we think that no prior work has paid attention to interface design to make the kernel development independent. 


\subsubsection{Graph Data Science Eco-System}
A few deep learning applications
require some of traditional and ad hoc graph analysis. E.g. when
preparing the dataset for deep learning, GraphSage~\cite{graphsage17} first does sampling or community analysis to downsize the graph. Additionally,
it performs connected component analysis, and then does union of a few
components before performing the training on it. Today, such pre-processing is done using NetworkX~\cite{networkx08}, a purely Python Package. Clearly, this approach will not scale when the dataset size is larger, as evident in our measurements in ~\cref{sec.exp}.

We observe that isolated approach of solving different parts of a common problem requires huge efforts. We envision a new graph data science eco-system, that can bring high-performance to every part of such use-cases. Such eco-system should not only provide better performance, but must also allow modular design so that other system researchers can take advantage to develop other functionalities, and plug back their contributions easily. 


\subsection{Education}
There is a need to introduce system-level classes for DL education, as has been voiced in an NSF workshop~\cite{storage2025NSF} by industry partners. 
%Preparing the lectures to explain kernels, and GPU properties are easy. However, It is indeed hard to design kernel assignment that can be used in  end-to-end training without involving additional efforts. 
There exists several courses~\cite{dlsCMU, cs15884CMU, cse599wWashington,cs231nStandford} that teach deep learning. Their coding assignments that have a training loop do not have a system components. While, assignments that have system components allow Python implementation, such as pooling, softmax, batch normalization, etc., and are not evaluated in a training loop. 
%Others~\cite{dlsCMU, cs15884CMU, cse599wWashington} focus on the deep learning system, however, their code assignment is piece-wise (not an end-to-end approach like pacman), mainly focusing on individual components in Python and not in C++ without using them in an end-to-end training. 
%implementing computational graphs or gradient updates in a Python environment. \td 
%Therefore, there do not exist any education assignments which can provide potential c++/CUDA kernel implementation for DL systems.

We strongly believe that the learning remains incomplete, if students cannot see the impact of kernel developed as part of an assignment or semester long project in a training loop.
%Due to fixed duration of any coursework, students needs a software infrastructure to quickly do the assigned tasks. 
Further, we cannot expect students to write this integration task from scratch, as integration problem solving or taking care of storage management is not aligned with the teaching goal of every assignment. 
Moreover, the limited duration of coursework is likely to be a challenge in completing those parts.

%We see many other challenges in offering such infrastructure today. \textit{Firstly}, it is also difficult for students to design graph and tensor exchange between the environment and kernel.
%%That is because this procedure is not important for  systems teaching, but it 
%which is very important in GNN systems implementation because it links the Python environment with the C++/CUDA kernel. Without this link, the GNN system cannot work even if the remaining parts are correct.  However, as we explain in \cref{sec.science.challenges}, passing graph and tensor to a kernel is very different and challenging than passing data between Python and C++. \textit{Secondly},  %Students do not know where to start and how to design the infrastructure.
%Students may not learn deep learning when preparing the dataset and create the corresponding graph storage, which varies based on the type of GNN model, as well as based on one's conviction about which storage will result in better performance. Although there exists some third-party library that can generate the graph object, this graph object cannot be used to implement the GNN kernel. \cref{sec.science.challenges} explains the reason in detail. \textit{Lastly}, ideally GNN assignment platform should be a real-time assignment protocol to match the GNN systems. In other words, the ideally platform should be separated to different tasks(functionalities) easily. However, existing works are very complex and it is impossible to use them to teach students about GNN kernel as well as some CPU, and GPU optimization strategies. \red{not clear.}
 
%Our novel design (section 4) makes {\graphpy}  become an ideal education platform for the GNN system. To prove it, the {\graphpy} was introduced to a graduate-level course that we taught recently. Students were able to implement CPU and GPU versions of GCN in 4 weeks, and each student independently implemented another GNN in the semester-long project. We plan to introduce {\graphpy} in the undergraduate courses also.

% By devising tensor exchange method independent of DL framework, and allowing passing of any custom objects in Kernel APIs, {\graphpy} offers application in any deep learning domain. 

% By focusing on graph data science use-cases, {\graphpy} has made it very productive to educate learners in graph domain with a focus on Systems education. Since, {\graphpy} touches the very basic building block of end-to-end deep learning procedure, classroom assignments can be tuned to target different functionalities. 

% This novel design of {\graphpy} 
% let learners remained focused to complete DL programming assignments, as evident in a graduate level course that we taught recently. 
% Students were able to implement CPU and GPU version of GCN in 4 weeks, and each student independently implemented another GNN in the semester long project. We plan to introduce {\graphpy} in the undergraduate courses, and share it with wider audiences to fulfill the demand of the industry~\cite{storage2025NSF}.

% \noindent \textbf{Minimizing the Framework Overhead.}
% Avoid introducing overhead is an necessary requirement for a system so that the later optimization techniques will not try to minimize that overhead, and rather should focus exclusively on actual system optimization tasks. In other words, when compared against small overhead systems, it is not likely to get misleading benefits. However, in the traditional graph data science domain, Mcsherry et al~\cite{mcsherry2015scalability} point out that many systems introduce large system overhead, which is then also optimized as part of analytics performance optimization. Hence, actual performance improvement remains less.

% Our experiment measurements (\cref{sec.exp}) show that DGL introduces huge system overheads in the form of a one-time start up cost, and run-time overhead, which is also identified by DGL. And because of these two costs, DGL performs poorly (more than 2$\times$)  compared to reference implementation (not optimized) of {\graphpy} for GNNs on several dataset, despite DGL kernels performing better than {\graphpy} kernels. Since DGL has a large overhead, it is not surprising that many prior GNN systems~\cite{GNNAdvisor,huang2021understanding}, which do not use DGL for their integration, have a huge speedup.

% To this end, {\graphpy} through its lightweight design minimizes both the overheads, and hence is well-suited not only for future systems research prototypes, but also as a baseline to understand the true impact of prior system optimizations.

% %On the other hand, DGL/PyG takes only COO arrays as input in their initialization API. 
% %Further, the generation of critical boiler-plate code, makes integration effortless. 
% \noindent \textbf{Sparse Data.}
% We also implemented {\graphpy-Kernel} for GNN as proof of concept and reference. We mostly focused on CSR/CSC format for reference and comparison, 
% It includes an unweighted gSpMM kernel to support GCN and GIN; a weighted gSpMM kernel, and two versions of gSDDMM kernel for GAT as mentioned in Table~\ref{table-kernel}. 
% %Both of these are sufficient for a graph-specific softmax layer, and for edge-level attention score from vertex-level features.
% We use pull-style computation that avoids usage of atomic instructions: so CSC for forward and CSR for backward computation or wherever inverse graph is needed.
% We used OpenMP for vertex-level parallelism in CPU. % and use vertex-centric computation.
% To support GPUs, we implemented kernels in CUDA. The same {\graphpy-Workflow} works except that the model requires to be converted to GPU, which is achieved using $model.to(cuda)$, where cuda is the device context. Similarly, the adapter of {\graphpy-Workflow} allocates tensors directly on GPU.

% We also implemented another format borrowed from prior graph analytics work~\cite{gstore}, which is very different from CSR/CSC format to demonstrate that an entirely different format can be implemented with same ease, using the same set of Kernel APIs. We used the same {\graphpy-Workflow} code, including the GNN model, graph convolution layers. We do not use that format for comparison.
% % \noindent 
% % $\bullet$ \textbf{GPU Support.} 
% % The specialized kernel is also implemented in GPUs by using the same boiler-plate code. The same {$wrap\_graph$()} API instead of simply wrapping the CPU version of Numpy arrays, it copies them to GPU memory, and then wraps them up in $g$ object. Thus, the rest of the kernel APIs (Table~\ref{table-kernel}) get the GPU version of the graph, and Python binding code of the kernel invokes the GPU kernels. Thus, the same piece of {\graphpy-Workflow} works except that the model requires to be converted to GPU, which is achieved easily using $model.to(cuda)$, where cuda is the device context. Similarly, the {\graphpy-Workflow} allocates tensors directly on cuda or device memory.

\noindent \textbf{Observation \#1.}
General purpose DL frameworks' plugin development environment have interface  limitations that only allow their captive tensor data-structure and built-in scalar type but not a graph object to be used as kernel arguments. Due to such limitations, many works~\cite{pytorchg2019,spektral,graphnets,GNNAdvisor,gespmmsc2020,huang2021understanding} have devoted huge efforts due to critical thinking (\cref{sec.science.challenges}) in designing workarounds to pass graph storage to kernels. Clearly, such efforts have no research outcome, and are merely done to integrate the kernel. Some~\cite{pytorchg2019,spektral,graphnets} even chose inefficient COO format, as it can easily be passed as a pair of tensors, despite it being inferior to CSR/CSC format.

%(see \cref{sec.background.graph} for definition) 
%discarding the decades of research works on sparsity~\cite{zhang2015numa,gstore,libgraplus15DB,liu2015enterprise,wang2015gunrock,gorder16sigmod,rabbit16ipdps}.
%such as using specifically tailored data layout~\cite{zhang2015numa,gstore,libgraplus15DB}, graph-aware compression~\cite{libgraplus15DB,gstore}, fine-grained and workload-aware parallelism~\cite{liu2015enterprise,wang2015gunrock}, graph re-ordering~\cite{gorder16sigmod,rabbit16ipdps}, graph partitioning, etc. for CPUs and GPUs. 
%The limitation has clear implication in terms of critical thinking efforts about designing workarounds (\cref{sec.science.challenges}) on how to pass the CSR/CSC graph storage to kernel prototype as evident in~\cite{GNNAdvisor,gespmmsc2020,huang2021understanding}. 
%that could have been devoted to actual research. 
%while a few excellent DL system research did not show the impact on the end-to-end training
%or requires development of new tensor library along with its memory management.
%Sparsity has recently been handled for traditional graph data science use-cases ~\cite{malewicz2010pregel,gonzalez2012powergraph,roy2013x}, such as Breadth-First Search, PageRank, or unsupervised machine learning. 
% Due to its similarities with GNN (\cref{sec.gnn-background}), it is natural to use these techniques to handle the sparsity in DL.
%However, to use these code-bases in an end-to-end DL benchmarking, we need DL framework's crucial features, such as \textit{computation graph}, \textit{tensor management}~\cite{dgl2019}, and \textit{gradient back-propagation} (\cref{sec.background.dl}). 

%\noindent \textbf{Observation \#2.}
%It is insufficient to implement the new GNN kernels either on top of prior graph analytics code-bases or from scratch in isolation without integrating them in an end-to-end DL model training loop. The reason is that 
To bypass the integration, many system works focus on isolated approach of kernel implementation and evaluation. However, 
In DL, forward computation, and gradient back-propagation generate requirements for different graph storage and computation. E.g., GAT~\cite{gat18iclr}, the edge-level tensor should only be accessed using edge IDs that should be part of the graph storage (\cref{sec.background.dl}), and may be missed by such approach. %Unfortunately, an evaluation that only focuses on kernel optimization in isolation without evaluating the training accuracy is likely to skip such finer details of edge ID requirement, resulting in misleading performance comparison. 
We point out that performance benchmarking without evaluating the accuracy have resulted in errors in performance measurement in prior works~\cite{GNNAdvisor,huang2021understanding} (\cref{sec.gnn-background}). 
%Such observation outline the need to integrate the kernel optimization in an end-to-end training loop for accuracy evaluation, before performance evaluation can be performed.  
%Rather, we observe that a few prior works that still focuses on  
%As we explain in \cref{sec.science}, integration is a complex task, and requires work-around instead of being straight-forward. 


%Systems frameworks such as MPI, OpenMP, PGAS etc.
% \td maybe we talk a little bit more about GAS,(GAS can achieve the same performance as original algorithm?)
% While some difference does exist  between graph analytics and GNN, which we explain shortly, 
% Because of the similarity between graph analytics and GNNs, it becomes a natural desire to adapt the system designs from the success of the graph analytics to the GNN workloads to take advantage of the decades of system research work.
% It is imperative that the research community should be able to test the efficiency and applicability of the systems aspects that targeted graph analytics to the GNN workloads quickly, instead of repeating the decades of research work. This exercise is desired because, 

\noindent \textbf{Observation \#2.} Our measurements show that many prior works frequently show out-of-memory error on slightly larger dataset that has less than 230 million edges in a single GPU setup. Due to this, prior works have only evaluated smaller dataset. Our investigation finds that any performance improvement in training smaller dataset is purely due to framework overhead, and not because of better kernel performance. Hence, we hardly have any baseline system which allows training on larger dataset so that it can be used to authoritatively show performance benefit of better kernel design on end-to-end DL training tasks in a single GPU setup.

\noindent \textbf{Observation \#3.} 
Existing works handle the sparsity for data science use-cases in a piece-meal way. (a) GNN systems handle only sparse data, but not sparse tensors that can use graphs. (b) There is no support for many common tasks, e.g. graph storage preparation from raw data.
For different GNN models, graph storage differ a lot in terms of graph direction, edge ID, etc., thereby same tasks need to be repeated for different GNNs by users in ad hoc way. 

%Hence, a new abstraction is needed that can unify the support for diverse graph storage need to an independent module, and makes exchange of graph storage simple and standard without repeating the mundane tasks. 
%Hence, many GNN systems~\cite{GNNAdvisor,neugraph19atc} have chosen to demonstrate only simple GNNs, where graph is undirected and unweighted, ignoring the attention based GNNs such as GAT or sparse models. 
% (c) NetworkX ~\cite{networkx08}, a purely Python graph data science package, remains popular due to its ease of use by data scientists, but remains very slow due to absence of system languages like C++/CUDA. 
% Therefore, there is a gap between systems (C++/CUDA) research deployment for traditional graph data science (Python) use-cases.

%To fix this gap, we see an opportunity in unifying different use-cases under a single platform with open interfaces where independent high-performance back-end modules can be plugged easily including abstracting the common tasks to a single module. 
%and can exchange data using zero-copies.
% We argue that providing Python binding on top of such optimized systems will bring the performance advantage to data scientists, while it can help in abstracting away many mundane tasks in variety of data science use-cases.
% despite being an order of magnitude slower. 



% \noindent \textbf{Observation \#3.} Traditional graph analysis did achieve an incredible system performance, but NetworkX~\cite{networkx08}, which is purely a Python package, is still very popular and is maintained actively due to the ease of use of Python programming environment over system languages like C/C++/CUDA. We argue that providing Python binding on top such optimized systems will bring the performance advantage to data scientists.
% despite being an order of magnitude slower. 
% However, bridging the gap between systems researcher (C/C++/CUDA) and data-scientist (Python) is not possible without significant research and design effort (\cref{sec.multi}.



% Lets us talk about GraphOne in problem statement.
%Although there exists some graph analytics systems which includes the graph data engineering, such as GraphOne~\cite{kumar2017graphone} NetworkX~\cite{networkx08}, these works cannot be used in the graph data science directly. But GraphOne, A, B are mainly written in c++. These implementation incompatible also increase the difficulty for users to deploy the mechanism to re-use these graph representations. 
%Firstly, Graphone, A, B, NetworkX do create the graph representation structure, but if the user wants to use it, they need to figure out the graph structure details, which is not an easy job.

% \noindent \textbf{Observation \#3.}
% Existing GNN systems such as DGL, featgraph, GNNAdviosr  (need citation TODO)
% implement their kernel by using the c++/CUDA plugin of a specific DL framework backend. (Not sure whether DGL satisfies this or not TODO) This system design makes their kernel highly dependent on not only the DL framework backend but also the specific version of the DL framework backend.
% The DL framework backend dependency limits their kernel codebase to a specific DL backend, which makes their codebase cannot be re-used across different DL framework backends.
% The DL framework backend version dependency increases the manual effort to maintain the GNN systems because of the periodic update of DL framework backend versions.
% Moreover, the DL framework backend version dependency increases the difficulties and complexities of usage because there may exist package version conflicts when configuring the environment and compilation.
% Therefore, there is a need to provide a unified GNN system that is independent of backend versions and their codebase can be reused across different backends.


\noindent \textbf{Observation \#4.}
Industry partners have voiced concern on availability of candidates with good systems and data science knowledge~\cite{storage2025NSF}.
%However, DL frameworks limitations do not allow them to be used as educational platform for DL system learning. 
%There exists a void in terms of education tools to introduce deep learning system research to our future system engineers and researchers. 
In Operating Systems (OS), XV6~\cite{xv6} has become a popular tool for undergraduate teaching allowing OS kernel modification for learning. 
%Similarly, the Pac-Man~\cite{denero2010teaching}, Open AI gym~\cite{brockman2016openai}  and RLcard~\cite{zha2019rlcard}, etc. provide sufficient environment for evaluating reinforcement learning algorithms.
However, limitation in DL frameworks' plugin interfaces, that disallow passing custom objects, limits their usage. 
We observe that many deep learning system courses~\cite{cs224w,cse599wWashington,cs231nStandford,cs15884CMU,dlsCMU} in universities actually allow Python to prototype the kernel assignments without focus on its integration in a DL workflow. 
Hence, they not necessarily train students in data science and systems both.  
%Therefore, we believe a lightweight platform is the need of the hour to train students in data science and systems together. 
%Other approaches need huge efforts just to integrate kernels to deep learning training, while being severely limited the way data can which may not be suited for assignments in semester long courses.

% and it is not modular enough to easily implement them as explained in \cref{sec.background}.

% \vspace{1mm}
%\noindent \textbf{Proposition.} Evaluation of the system techniques proposed by traditional graph analysis for the DL use-cases, offering high performance to data scientists, and speeding up the systems research in graph data science are all related problems, and have a number of overlapping steps. While general-purpose DL frameworks are definitely not suited for such purpose due to poor support for sparse data and sparse tensors, even the current GNN frameworks are not ready yet, as they still lack the support for sparse tensors/layers. Moreover, it even does not handle a graph different from a plain homogeneous graph. Thus, sparse layers and ad hoc analysis cannot even be supported (\cref{sec.motivation}). Finally, only few are open-sourced, they are monolithic, lack design documentation for back-end and are frequently changing, and do not preclude writing many mundane tasks. Hence, modifying such monolithic and frequently changing code-base for prototyping system ideas is hard and time-consuming, and the resultant system will become even more complex.

% and it is not modular enough to easily implement them as explained in \cref{sec.background}.
%A platform is desired for quickly prototyping any new or old system idea without getting bogged down by the sheer complexity of learning undocumented code-bases or with dated documentations. Rather, a platform is also desired to introduce deep learning to our future systems engineers and researchers, which has been flagged as a concern in various forums[\td]. Modifying the back-end of general-purpose DL framework for educational or even research purpose is too time consuming. Following a restricted programming in the form of plugin development and their build system (e.g. in Pytorch) will result in a loss of general learning specifically how the interfaces work in such a large system. Further, these all method involves repeating many mundane steps that provide no value to research or learning. 
%At the same time, offering data-scientist high-performance APIs is needed. 


% A good platform for graph data science should clearly identify the boundary between different tasks, should provide all the mundane task for graph data science and offer boiler-plate code to integrate the third party kernels, and let the system programmer continue with their choice of tool-set and programming language. 




\noindent \textbf{Contribution.}
We present {\graphpy}, a modular and interface oriented lightweight platform to enable implementation of various graph data science use-cases for both research and educational purpose. Fig.~\ref{fig-arch} shows a high-level overview of {\graphpy}. Contributions are summarized as follows:

\noindent $\bullet$ \textbf{Tensor and Graph Exchange.} The innovations in interface design enables tensors to be passed to kernels as array-like structure, and allowing graphs or any custom objects to be passed to kernels directly, thereby avoiding the need of critical thinking that we discussed in observation \#1.
%same way that any dense data (such as images) are passed, thereby achieving uniformity without any limitations. Further, any arbitrary objects could be passed as well. 
Compared to current practices, {\graphpy} interfaces have no issues in passing any data-types in kernel invocation, and enable {\graphpy-Kernel} to gain full independence from any DL framework code, thereby
%and offer easier research prototyping and effortless deployment. 
introducing \textit{re-usability} of kernel code across many DL frameworks and their versions. 

\noindent $\bullet$ \textbf{Automatic Integration.}
{\graphpy} \textit{generates} critical boilerplate code to handle interfaces, memory management, and Python binding of kernels.  This results in zero effort in integration. 
%

\noindent $\bullet$ \textbf{Separation of Graph Storage, and standardization of its Exchange.} 
%to an independent high-performance {\graphpy-SM} module is achieved using \textit{Numpy dtype} that can supports specification of \textit{arbitrary multi-field graph properties}. The module exports the graph storage using \textit{zero-copy} Numpy arrays to other modules to free the data scientists and systems researchers from graph storage tasks. 
By separating the graph storage management, we allow innovation in interface design that let {\graphpy-SM} to handle multi-field graph properties using a single set of API by using \textit{NumPy Dtype}, while exporting the prepared graph storage to {\graphpy-Kernel} using \textit{zero-copy} NumPy arrays. 
By relying on  Dtype, {\graphpy} makes sparse matrix (i.e., graph) same as dense matrix (e.g., image data) for storage specification and exchange purpose. Interface design leaves enough room in {\graphpy-Kernel} to innovate on graph storage design without impacting {\graphpy-SM}.
We are unaware of any high-performance Python package that can support arbitrary multi-field graph properties. It also cannot be designed without significant innovations(\cref{sec.engg}). 






% NetworkX~\cite{networkx08} is the closest one, but is a pure python package, and hence lacks scalability, performance, and cannot handle big graphs. 
% It also supports the arbitrary edge features which is important in knowledge bases graph GNNs. Besides this, the graph creation module also provides flexible choice for users to determine whether create the edge ID or whether procedure(forward/backward) the edge should be created. 

% Furthermore, it generates boiler-plate code to integrate independent kernels of different data science use-cases to keep the efforts minimal while integrating them to Python and provides an extensible architecture to support various computations that makes it easy to implement new system idea. 



% {\graphpy-Kernel} module is an independent plug-and-play module responsible for kernel implementation in CPU/GPU by using the above prepared graph, while {\graphpy-Workflow} uses general-purpose DL frameworks to offer computation graph, and gradient back-propagation, and uses Python APIs of {\graphpy-Kernel}.
% To integrate these without much dependency, {\graphpy} generates the required critical boiler-plate code for Python binding of kernels, and tensor handling code in {\graphpy-Workflow} using our proposed domain-specific language (DSL). The generated code does the memory management of tensors and passes them as flat arrays to {\graphpy-Kernel}. Hence, this separation and generated code reduces the end to end development cost of any DL layer and corresponding kernels. 

% 3.{\graphpy} supports dynamic graph by incrementally update the graph representation. Some optimizations techniques are also adopted so that it can support large graph. 





% 7. {\graphpy}support extensible wrapped python APIs. {\graphpy}is optimized to only use c++ as the bottom implementation language in kernel module and graph creation module and wrapped them out to python to interact with remaining modules. In other words, we use python for modules without high performance requirement instead of implementing all modules in c++ but provides some high level python APIs. This implementation strategy can let graph neural network researchers extend or add new customized graph DL framework easily. 

% The contributions of our work are summarized as:
% \begin{itemize}
% %\item Unifying the graph data engineering with graph DL leads to one integrated graph neural network system, and provides end-to-end control over data engineering and machine learning operations resulting into greater synergy and performance.
% \item {\graphpy} supports graph creation with arbitrary vertex and edge properties, which make it more flexible for multiple types of graphs, and GNN models. It is mainly written in c++, but provide python user interface, which make it possible to use more cores and distributed systems to handle larger graphs.

% \td do we also need to mention that graphPy is a end-to-end work that users do not need to worry about how to read raw data?
% \noindent $\bullet$
% {\graphpy} unifies the GNN system research by its novel memory management design and framework design. 
% Unlike existing systems, {\graphpy} does not limit to a specific DL framework version or a specific DL framework backend.  Therefore, System researchers only need to focus on kernel implementation and optimization instead of worrying about environment configuration.
 

%Further, combination of two entirely different languages: compilation oriented C++/CUDA with interpretation oriented Python, creates further challenges. 
\noindent $\bullet$
\textbf{Modular and Lightweight.} {\graphpy} is inspired from the Unix Philosophy~\cite{mcilroy1978unix} as opposed to monolithic design.
Hence, custom use-cases for handling sparsity can easily be developed, optimized and deployed independently.
%By using graphs to model the sparsity, {\graphpy} opens a new research direction where the plethora of work done in graph analytics can be extended to GNN, and to support sparse tensors that can be modeled using graphs.
%Further, focus on interface design minimizes the framework overhead that other systems~\cite{dgl2019} often encounter
%\footnote{See \url{https://arxiv.org/pdf/1909.01315.pdf} for DGL overhead} 
%making {\graphpy} an excellent framework for research.
Bare minimum code-base, and support for graph storage make {\graphpy} an excellent tool for deep learning system education, 
%as system learners only need to focus on kernel implementation and optimization, 
while automatic integration allows system code evaluation in actual graph data science use-cases, that we believe is a strong motivation for learners to stay invested. 
%Further, the lightweight design leads to less framework overhead, while our reference implementation consumes less memory that makes {\graphpy} an ideal baseline system. 



% {\graphpy} helps in easy prototyping any DL layer as well as performing systems research where the plethora of work done in graph analytics or new systems ideas can easily be tried for deep learning.
% Due to such flexibility, we are able to offer a high-performance implementation for GNNs, sparse models, and traditional graph analysis that all are usable from Python. 
% For evaluation, we use our reference vanilla implementation, and leave the evaluation of optimizations as future work. 




% \noindent $\bullet$
% From the view of the flexibility of sparsity use-cases, {\graphpy}  can be used in multiple levels of sparsity situations due to its novel design. For example, existing DL frameworks, such as DGL and PyTorch Geometric, can only support data level of sparsity (e.g., Sparse data, the data itself is sparse). However, {\graphpy} not only supports data level sparsity but also can support model level sparsity (e.g., the Sparse model, the compressed deep learning model itself is sparse, which means many model weights are set to 0).


We demonstrate the usefulness of {\graphpy} with the implementation of at least two different storage format for many GNN kernels as well as support sparse tensors that can be modeled using graphs, and using {\graphpy} in a graduate-level course. Empirical evaluations show that our \textit{reference implementation} achieves 1.62$\times$ and 1.35$\times$ over DGL and PyTorch for various GNN models on many datasets in GPU, and 1.55$\times$ and 1.88$\times$ on CPU respectively with similar accuracy readings.
%on an average 1.64$\times$ and 1.42$\times$ speedup and 1.30$\times$ and 2.29$\times$ speedup over DGL, and PyTorch Geometric for various GNN models in GPU and CPU respectively. 
Investigation of accuracy and speedup together brings several critical observations, which question some of the measurement practices of prior works: focusing purely on performance gain without measuring accuracy is a recipe of disaster for this new area of GNN research for which we do not have complete system understanding, including graph storage requirement, role of framework overhead, etc.  
%Further, frequent out-of-memory condition by DGL, Pytorch-Geometric, and GNNAdvisor forces measurements to be performed on smaller dataset only. Measurements on smaller prevalent dataset do not show advantage of kernel optimization due to framework overhead.
To this end, our measurements show that focus on interface design minimizes the framework overhead of {\graphpy} by 1.46$\times$, and 1.28$\times$ than DGL and PyG.
Low memory consumption allows {\graphpy} to run GCN, GIN, and two versions of GAT on all the datasets, while DGL, PyG, GNNadvisor all have many out-of-memory conditions.
%\footnote{See \url{https://arxiv.org/pdf/1909.01315.pdf} for DGL overhead} 
%making {\graphpy} an excellent framework for research. 
A better GNN performance using the reference implementation, less framework overhead, low memory consumption make {\graphpy} an ideal baseline for performance benchmarking for future research. 
%as prior works show out-of-memory conditions even on a moderate sized dataset on which evaluation is mandatory, as measurements on smaller prevalent dataset do not show advantage of kernel optimization. 


\begin{figure}[t]
  \includegraphics[scale= 0.5]{result/overview-crop.pdf}
 \vspace{-6pt}
  \caption{ \small {\graphpy} Platform: {\graphpy-Kernel} is plug-and-play, which can be customized to implement any novel system design to handle sparse data and model. {\graphpy-Workflow} provides the DL support including tensor management and computation graph.} 
  %{\graphpy-SM} prepares graph.}
  \label{fig-arch}
%   \vspace{-12pt}
\end{figure}

%We show that the speedup with respect to DGL is the result of less framework start up and run-time overhead, as DGL kernel performs better than the {\graphpy} reference kernels. We also show the implication of DGL's framework overhead on evaluations of prior works, and why its design and overhead discourage researchers to use DGL for research prototyping. 
%This result confirms that latest GNN works have benefitted from while proposing new system optimizations have not compared against well-known but simple parallelization techniques. Hence, we establish new baseline for GNNs that can be used for evaluating impact of future optimizations.

Moreover, we show that using graphs for re-training compressed LeNet-300-100 (sparse model) on MNIST dataset leads to 17.5\% speedup in CPU, while minimizing the memory need of the compressed layers.
For the graph creation procedure, {\graphpy} is more than 5$\times$ and 10$\times$ faster than DGL and NetworkX respectively on various datasets. 
For traditional graph analysis from Python programming environment, {\graphpy} is up to an order of magnitude faster than NetworkX.



%}
% system with a high-performance graph creation module and pluggable, neural kernels modular as well as the transparent, extensible python Graph DL APIs. It also outlines the steps to keep the efforts minimal while integrating the techniques of prior graph analytics systems to {\graphpy}.
% \td figure one words is not the same as we discussed below, do we need to modify it?

% \textit{{\graphpy-DE}} is a high-performance graph data engineering module which will create the graph representation directly from the raw graph data from Python programming environment, and exports it to be used by any module. % It also uses zero-copy mechanism to export the prepared graph out to any other module in the CSR, or COO format.
% \textit{{\graphpy-Kernel}} is a \textit{plug-and-play} high-performance module, where each instance is is responsible for implementing kernels using the prepared graph and boiler-plate code for a specific use-case. 
% \textit{{\graphpy-Workflow}} provides all the support for DL workflow. It uses the DL framework to provide computation graph creation, tensor management, and gradient computation, and allows the specialized version of {\graphpy-Kernel} to be called during forward and backward computation both without doing any single tensor related operations inside the kernel.


% (b) between graph analytics and DL. We present {\graphpy}, that provides a ready to use python package for data engineering efficiently, but also outlines the steps and provides solutions to keep the efforts minimal while integrating the prior graph analytics systems. 
%this gap by presenting an end to end pipeline to support graph data science and graph data engineering. 

\noindent $\bullet$
\textbf{Support Sparse Tensors.}
{\td add the sparse tensor in background}
Except for the GNN, many model compression works involve a different level of sparsity. (Our section \td ) These sparsity differences prohibit the existing works to apply to this problem anymore. In this work, Our modular-based design lets us be the first one to provide memory saving and performance speed-up for this type of sparsity, which can deploy them to the limited-source device.
\subsection{Sparse Model Retraining Performance}

We choose the LeNet-300-100 \cite{lecun1998gradient}, a fully connected neural network with 300 and 100 as the hidden layers as the DL architecture. After weight pruning, all three fully connected layers become sparse with sparsity ratio of 4.46\%, 4.45\% and 7.78\% respectively, i.e., keeping less than 10 connections for every 100 connections in the fully connected layer. We use MNIST dataset which includes 60000 training and 10000 testing handwritten digits examples.  Each image in the dataset has 784 features, while the last fully connected layer produces prediction corresponding to 10 digits (0--9), which are sent to the softmax layer. 
We set the retraining epochs as 100 and the batch sizes as 50. In other words, in each training epoch, the model will iterate 1200 times.
% and apply tensor-based operations for state-of-art model and the sparse layers computation for {\graphpy}.
{\graphpy} finishes the retraining in 16 minutes and 17 seconds, compared to 20 minutes and 1 second for the state-of-the-art model that uses the bitmask matrix to achieve sparsity, achieving 17.5\% speedup, and huge memory saving.

%The reason for this speedup is the reduced computation which {\graphpy} could achieve due to its system-level support for sparsity. 
On the other hand, prior works have used bit-mask matrix at the Python level for achieving sparsity where the underlying kernel still uses dense matrix for sparse layer computation. Again, the improvement is only 17.5\% as LeNet-300-100 is not a large neural network, as the bipartite graph has vertex counts in the range of 784 and 10. Hence, the sparse weight matrices are not as large as the graph data set we had above for GNN case. This affects the vertex-level parallelism for SpMM. With better technique, we expect better performance, as our implementation is only for reference. 

Secondly, it is not just the performance improvement, but the huge memory saving that allows the compressed model to fully fit in the resource constrained devices. Hence, model inference can now be done fully in such devices.
% Also, the sparse layers computation procedures contain mostly random reads instead of sequential reads. 


==> tex/others.tex <==
\vspace{1mm}
\noindent \textbf{Proposition.}
However, these graph deep learning system cannot directly read the graph structure from the raw data, instead, they rely on some pre-implemented python graph structure, NetworkX ~\cite{networkx08}, or a list of python objects. This design will make the users need to do more graph preprocessing jobs and lack scalability, performance, and cannot handle big graphs. Moreover, NetworkX cannot support dynamic graph representation, which means even if the graph is updated by a small number of edges, the NetworkX needs to re-create the whole graph representation instead of increment updating. This triggered us to design an end-to-end graph deep learning system with a high-performance graph creation modular which can support dynamic graph. 
 
As we mentioned in the introduction, the GNN research area is young, which means many new GNN frameworks with different variant tensor operations or some customized message-passing paradigms maybe proposed in the future. Therefore, the extensibility of graph deep learning systems become important. A good graph deep learning system should be flexible enough to extend to new GNN operations and should be able to add in new customized message passing kernels easily without worry about the code dependency. 
 
Although DGL does provide some extensibility by providing 4 scatter choice ‘sum, sub, multiple, divide’ and 3 gather options ‘max and min, sum’ for users to choose, the message passing paradigms is fixed. If users want to apply a customized message passing paradigms, they need to modify the whole message-passing paradigms as well as the dependent codes in other submodules. This design pattern may limit its usage because graph neural networks are more familiar with machine learning operations and it is hard for them to handle system code dependency.  From the above observation, we put all message-passing paradigms in a pluggable, neural kernels modular and minimize code dependency between different modular. 
 
For some knowledge bases graph GNNs[NEED ADD SOME CITATIONS], the edge information is also captured when applying the graph deep learning. Unlike the traditional edge information which normally treated as the edge weight or a float number, the edge information in the knowledge bases graph can be extended to a vector.[Not sure whether  I understand it correctly or not] Therefore, there is a need for a graph deep learning system to support the customized edge. 


Moreover, different GNNs have different aggregations. GCN uses the unweighted sum as the aggregation. But GAT uses the weighted sum version to assign a weight for each corresponding edge. In other words, edge ID is not necessary for GCN but necessary for GAT. It is unnecessary to always create the edge ID for GNNs. Moreover, the backward procedure of message passing paradigm need to integrate more computation than the forward. If the edge Id can be stored based on the backward procedure, the performance will be improved. Therefore, it is necessary for a graph deep learning system to provide flexible edge choice to users, such as whether creating the edge ID and which procedure the edge ID should be stored. 




\noindent 
$\bullet$ \textbf{New Sparse Formats and Data Sharing}
While we discussed that Numpy arrays will be used to allow zero-copy sharing of graph structured data, and hence it becomes very easy to share CSR/CSC format. However, once a system researcher comes up with an entirely different format~\cite{gstore,mosiacEuroSys17,hicoosc18}, one can think that {\graphpy-DE} as well as the data sharing APIs become non-usable. 
It should be noted that G-Store~\cite{gstore} calls the format Smallest-number-of-bits (SNB), and Mosaic~\cite{mosiacEuroSys17} calls it tile format. HiCoo~\cite{hicoosc18} reduces to the same format when dealing with sparse matrices, but it also extends this to higher dimension sparse data. We use SNB format as it was published first, and explain how the same set of API can be used for graph preparation and data exchange.

\begin{figure}[h]
  \includegraphics[scale= 0.22]{result/zero_tile.pdf}
  \caption{{\graphpy} SNB format.}
  \label{fig-snb}
\end{figure}

 \textbf{Solution: CSR as an Indexing Structure.}
To solve it, we came up with a generalized theory about graph data preparation and sharing that can capture graph in various formats. 
Fig.\td shows the SNB format, which we have re-arranged to make it look like CSR structure. This established the fact that CSR can be used as a general purpose indexing structure, wherever we have one-to-many relationship. 
Clearly, all the data exchange format remains same as it is, e.g. we can still use the 4 Numpy arrays with slightly different dtype to share the graph between {\graphpy-DE}, and {\graphpy-Kernel}, as shown in Listing \ref{list-snb}. It only required one cosmetic change at both the line number 6 and 10. 
%We also needed to modify the $get\_graph$() API that also returned vertex count as we cannot rely on offset array for the vertex count. This also require that we pass vertex count in the $init\_graph$() API. However, all these changes are cosmetic from the user point of view as we provide different version of $prep\_graph$() API.


%Python code highlighting
\begin{lstlisting}[language=Python, caption= Illustration of graph creation in SNB format, label={list-snb}]
import numpy as np
import graphpy as gp
def prep_graph():
  edge_dt=np.dtype([('src', np.int32), ('dst', np.int32), ('wt1', np.float), ('wt2', np.int32)]
  #Directed and SNB graph. 
  G=gp.create_graph(gp.eDdir|gp.eSNB, edge_dt) #Changed code 
  #space is delimiter
  G.add_edges_from_dir('./input_dir/', ' ')
  #Get graph as numpy array using SNB dtype.
  snb_dt=np.dtype([('src', np.int16), ('src', np.int16), ('wt1', np.float), ('wt2', np.int32)]) #Changed code
  csr_offset, csr_neighbor, csc_offset, csc_neighbor = G.get_graph(csr_dt)
\end{lstlisting}

To implement it in {\graphpy-DE}, we still utilized the same infrastructure, but had to adjust the \textit{CSR creation routine} in Fig.~\ref{fig-parallel_pa} to offer graph in SNB formats without changing its APIs.

Off-course, {\graphpy-Kernel} has to implement all the GNN kernel code, but it can still utilize the boiler-plate code. For the proof-of-concept, we integrated G-Store code which also had in-memory processing routine. We also implemented the spmm kernel for GCN. It should be noted that we did not require any changes to the {\graphpy-Workflow}.
%Should this format result into better GNN performance, but we leave it to the respective authors to implement the kernel and find out the details.





\subsubsection{\#2: Integrating Graph Analytics System Research with GNN}

Since existing graph analytics systems usually include optimized high-performance graph computation engine. A straightforward way to test their innovating ideas is to integrate these graph analytics systems with Graph neural networks by simply implementing the new GNN kernels on top of them.

\noindent \textbf{Gap between Kernel and DL Framework.}
One approach to integrate newly written kernel code to current DL framework is to port them to DL Frameworks. However, current DL frameworks does not have support for sparse linear algebra, and hence it is not easy to integrate these system enhancements to improve GNN performance, as it will involve huge efforts not only in integrating into the back-end but also require python binding as per the limitation of these frameworks. Such frameworks allow python binding of limited types.

%To this, end, we list down some basic building blocks, that can guide researchers from graph analytics field to quickly prototype additional functionality on top of the existing code base to test whether those techniques are beneficial or not, before we jump to brand new implementation.
One can try to integrate those code-bases to existing GNN frameworks by porting the existing design and code to them. However, such porting generally requires huge effort to understand the existing development environment and framework. Moreover, their code-base is still nascent, does not have documentation on how one can integrate the code in the back-end, and their code base is constantly changing. Without active involvement of the system maintainer, it seems not possible to integrate new ideas to current GNN frameworks~\cite{featgraphsc20}.
%and as well as  E.g. \td. what are the problems if we integrate in C++ way with Pytorch?  

Hence a more lightweight approach is required, where the job of system researcher should remain limited to implement the required kernels using their design without being restricted to follow a specific development style or any changes to the framework. Yet, it should immediately become part of the whole deep learning workflow. 
This will lead us to a flexible and generic infrastructure that will allow an independently developed pluggable modules, yet taking care of managing computation graph and tensors.


\subsection{Opportunities and Challenges}

The forgone decade saw incredible performance improvement to graph analytics tasks, such as Breadth First Search (BFS) or Page Rank due to various novel system designs, such as better data layout, improved utilization of hardware caches, NUMA-aware data partitioning, structure-aware compression, re-ordering to introduce data locality, integration with various hardware platforms, such as GPUs, FPGAs, customized hardware, etc. 
They improved the performance of graph analytics by orders of magnitude. Many of the techniques are highly graph-aware to take care of its irregularity in the structure and computation both.

On the other hand, GNN computations are very new with the first system level framework appearing recently~\cite{dgl2019}. So, there are plenty of opportunities to improve the performance, and is already being tried~\cite{featgraphsc20}. This is now even more important as deep learning training procedures are  more compute intensive than the tradition graph analysis. So, we are likely to see a number of research direction to optimize the GNN training time including using the techniques mentioned above.

% not all the techniques are possibly applicable to GNN eco-systems due to differences in the requirement between graph analysis and GNN.Graph analytics system researchers were highly influenced by Graph500~\cite{graph500} ranking, which benchmarked BFS or other graph traverse algorithms only. Each iteration of graph traverse algorithms operates on an active vertex set only and contains scalar vertex-level metadata only. However, 

However, trying system system techniques in the context of deep learning is not so easy.
These graph traverse algorithm workloads are very different from the GNNs as GNN have 2 procedures, \textit{forward procedure}, \textit{backward procedure} in each epoch of the training. 
Further, the GNN kernel uses vector metadata and trainable parameters for each vertex and edge in forward procedure and calculate the loss based on the prediction result. In backward procedure, GNN kernel computes the gradient and updated the training parameters based on the loss we calculated before. 
In other words, we can view traditional Graph Analytic works as performing the forward procedure only.
% but do not need the backward procedure.
% \td maybe backward also need to store the gradient information? 
As we discussed in Figure~\ref{fig-forward}, backward procedure has additional requirements, including saving and operating on the tensors produced by forward computation, referred as tensor \textit{states}, and many times operating on the inverse of the graph.

%Nonetheless, considering the variety of work it is natural that  we must test the efficacy of such techniques before putting the verdict out. 

So, if one wants to develop GNN on top of prior graph analytics systems, he or she has to take care of data engineering tasks, implementation of GNN kernels on top of their GAS framework, and the deep learning specific workflow including computation graph and gradient calculations. These tasks have system challenges and involves huge efforts as we discuss next.

% Specifically, many of the techniques focused purely on optimizing the BFS due to benchmarking established by Graph500. BFS is very different than GNN kernels. The former is very compute light, and only a few vertices participate in each iteration. Apart from that the computation only happens in the forward direction in graph analytics as it does not involve gradient computation.



%system which can support graph deep learning features. To be more specific, given the raw input data, such as the CSV, Jason, text or binary data, the graph deep learning system should build the dynamic graph representation data structure automatically and also provides python APIs for users to perform traditional graph topology analysis as well as the graph deep learning operations. 
 
%All the previous works cannot support these requirements, this trigger our work {\graphpy}, which unify the graph data engineering with graph deep learning leads to one integrated graph neural network system and provides end-to-end control over data engineering and machine learning operations resulting in greater synergy and performance.





\subsubsection{Traditional Graph Data Science}


With the advent of data-science as a field, people from many fields are attracted to it. One of the important reason of is easy to program using Python programming language, and the ease with which DL frameworks can be programmed at least in a single node/GPU setup.




==> tex/overview.tex <==
% \noindent \textbf{New Kernels Definition and A Better GNN Baseline.}
% The majority of the prior works have focused on class A GNN only, leaving the entire class B models out. This observation along with issues with prior works makes DGL the only baseline that can be used for performance comparison on both the classes of GNN.
% However, it still suffers from various overheads that do make DGL an ideal baseline, while it works with CuSparse Kernels that are not well-suited for GNN. 
% %may still require the latest GPU, otherwise, we will be limited to the smaller dataset evaluations, which are impacted due to framework overhead. 
% %Even in the latest GPU, the \textit{requirement mismatch overhead}, as discussed earlier does not make DGL an ideal baseline. 
% Further, for GCN evaluation, it may be possible to find an existing system~\cite{tian2020pcgcn} that might perform better than DGL, as researchers from various domains have implemented GCN, however, we do not find other systems which have an end-to-end implementation of all the GNN classes. 
% %Moreover, we need to provide new kernel definition and implementation based on GNN system requirements so that which will serve as a well-optimized baseline for future optimizations. 
% \textit{Clearly, kernels focused on GNN requirements are needed to be defined and designed that can provide an optimized GNN baseline to evaluate future system optimizations so that the state-of-the-art can actually advance.}


%such as other systems do not have correct accuracy, do not implement all the representative GNN classes, and have no implementation of end-to-end training. While PyG cannot be run on slightly larger dataset, it is mostly DGL that researchers use to compare performance. And, since DGL has framework-level overhead, requirement mismatch overhead, and huge memory consumption; systems work can easily show performance improvement as it can bypass one of the problems. 


%\subsubsection{Larger Dataset: Requirement Mismatch Overhead}
%We now discuss the issues in performance benchmarking the large dataset on DGL, as it seems DGL is the only system that can reliably be used to evaluate large datasets.
%\noindent \textbf{Kernel Problem.}
%Besides the overhead on small datasets, We find that existing GNN systems work cannot achieve end-to-end performance improvement even if its kernel itself is well optimized. 
%A straightforward example is DGL\cite{wang2019deep}. 


% \noindent \textbf{Requirement Mismatch Overhead.}
% DGL adopts the gSpMM kernel of CuSparse, a CUDA library optimized and provided by Nvidia over decades, that is used by GNNs.
% CuSparse provides only gSpMMve kernel, which has the following deficiencies as far as its match with GNN is concerned. 



% For the sake of discussion, we call these additional costs as \textit{requirement mismatch overhead}. While they definitely cause huge memory consumption and  explain why DGL consumes so much memory. We now explain the implication of the overhead on performance.





%So, performance gain by prior work is whether due to this overhead or they really advanced the state-of-the-art in limited way, such as a better kernel design despite having issues in model training. 
% 2.08 (reddit GCN), 1.15 (ogb reddit), 2.63 (reddit GAT), 1.49 (ogb GAT)

% \begin{table}[h]
% \small
% \vspace{-6pt}
% \caption{kernel time for different works (in Seconds)} % title of Table
% \vspace{-6pt}
% \centering % used for centering table
% \begin{tabular}{|l| c cccc|} 
%     \hline\hline 
%     Graph & Huang et al & GNNAdvisor & GE-SpMM & CuSparse & DGL \\ [0.5ex] % inserts table
%     %heading
%     \hline % inserts single horizontal line
%     Reddit & 0.0 &  0.0 & 1.0 & 1.0  & 0.0 \\ 
%     OGB-product & 0.0 & 0.0 & 1.0 & 1.0 & 0.0 \\
%     % & 76.47 &  76.52 & & \\
%     \hline %inserts single line
% \end{tabular}
% \vspace{-6pt}
% \label{table-kernel-time} % is used to refer this table in the text
% \end{table}





% %In case of GCN, DGL suffers from point \#1 and \#2 only. 
% For GE-SpMM gSpMMv, we clearly see that it does not perform better than CuSparse. Its kernel is designed using row-major tensors eliminating the requirement mismatch \#2, and hence performs better than DGL.
% %However, we ask again (for Vanilla GCN), does GE-SpMM really advanced the state-of-the-art, as the performance benefit is due to removal of the mismatches (point \#1 and \#2) and not due to the systems technique that it described in the paper. 
% However, once GE-SpMM introduces the edge-level tensor in its gSpMMve yielding the overhead \#1, it  performs slower than  CuSparse. 
% For Vanilla GCN, GE-SpMM gains performance due to removal of the mismatches (point \#1 and \#2) and not due to the system techniques that are described in the paper. 
% We do not discuss GAT, as the paper has not shown GAT results, and its graphs do not contain edge ID. However, GE-SpMM does show that for feature lengths multiple of 32, it does perform better than CuSparse, hence it does advance the state-of-the-art in some meaningful ways. 
% %However, if we extrapolate the results for GAT, 





%The table \ref{table-exp-kernel} shows 
%That is because the GSpMM in DGL is designed for both unweighted aggregation and weighted aggregation. It needs to apply one shuffle kernel each time before launching the CuSparse to support edge id indirection(refer to next section). Moreover, since CuSparse library can only accept column-level input, DGL needs to transpose the input tensor before using the CuSparse library. 

%These two more steps, eshuffle and transpose, cost huge extra time. Hence, if researchers compare the performance with gSpMM of DGL without paying attention to these additional requirements, they are likely to misled by the performance evaluations. 



%We focused on feature length 16 for GE-SpMM to derive the important research question (has state-of-the-art advanced due to the techniques described or due to requirement mismatch, that was a by-product and not identified in the previous papers). However, the conclusion is also true of other feature lengths such as 32. \td. 

%When reading the codebase of Huang et al~\cite{huang2021understanding}, we noticed many errors which is purely attributed to unclear understanding of the requirements. So, we take this opportunity to show that the scope of performance improvement due to  better gSpMMve kernel implementation. They have provided a gSpMMve kernel which again do not include edge ID indirection in their graph, and thus are similar to CuSparse except that it accepts row-major tensors. Clearly, the gSpMMve performance improvement is 16.2\%, and 37.4\% for Reddit and OGB-Product. However, its correct integration will still need eShuffle kernel. Therefore, overall benefit of better but equivalent of CuSparse kernel will have a diminishing return on GNN training.

% We cannot draw any observation for GAT, because papers that  evaluate GAT, have a giant fused kernel~\cite{fu2022tlpgnn,huang2021understanding}, with issues outlined earlier. 
% %However, for systems that have a kernel similar to CuSparse without edge ID support, will have to suffer from eShuffle overhead which is almost similar to gSpMMve kernel time. 
% Hence, at this moment, they did not advance the state-of-the-art.




%Further, the complexities in end-to-end implementation, such as Python binding, memory management (allocated memory in forward may be accessed during backward computation due to state requirement), argument passing (PyTorch only allows tensors and scalars to be passed in its back-end and not custom objects, e.g., graph), learning new build systems (Ninja in case of PyTorch) will make life hard for students. 
% Rather we are still struggling to enable a debug build of code-base of Huang et al~\cite{huang2021understanding} that used Ninja.

%We envision that creating such a tool/template code to aid the end-to-end deep learning requires systems architect efforts from the teacher side, but does the academic community value it as a research task or simply as an engineering effort? This is because such effort in creating a tool is unlikely to use performance as a key metric. This is clear from the fact that a lot of teaching tools, such as XV6~\cite{xv6} have not been published in any conference, but are used across many universities for teaching operating systems. 
%when the community is not able to find the flaws in the papers published in the reputed conferences.

% level optimization works, GNNAdvisors\cite{wang2021gnnadvisor}, Huang et al \cite{wang2019deep}, GE-SpMM~\cite{gespmmsc2020} read the DGL code base to understand the requirement. ( need some reference email them) 
% However, GNN model works, such as GCN, and GAT(these papers just provides the basic mechanism of the dense matrix) and GNN System works, such as DGL do not provide clear system-level requirement description. It is not guaranteed that all people can understand them correctly. 

% For example, to support the edge id indirection requirement (\ref{sec.edgeid}), DGL provides an extra shuffle kernel to reorder the edge id list each time before fetching the edge score tensor. After that, DGL transposes the input tensor and uses the CuSparse library to perform the computation. This extra shuffle kernel, transpose computation, and the system overhead time between them lead to extra time cost at the end-to-end training process. (\td find the line of code with shuffle + GSpMM) 
% If the requirement(above process) is not fully understood by researchers, even if they replaced the CuSparse library with an optimized kernel, the overall end-to-end training process will not be optimized. 
% Hardly do these previous papers discuss this edge id indirection requirement. Instead, Their kernel implementation can only support specific types of GSpMM, such as GCN\cite{kipf2016semi} and GIN \cite{xu2018powerful}. 
 

% Huang et al \cite{wang2019deep} does not consider this requirement when implementing the kernel also. It fetches the edge tensor in sequence, this incorrect fetching will lead to the wrong aggregation result.
% Although the integration between the kernel and the GNN model is correct, the overall simulated GNN has Some mistakes. (\td Not sure what this problem is: Input tensor and output send them as the same tensor)
% Because of these mistakes, even if the simulated end-to-end training time shows improvement, this result is not trusted and cannot represent real-world GAT training. 
% GE-SpMM~\cite{gespmmsc2020} forgets to consider edge id indirection also.



% \noindent \textbf{A Tool for Education and Research is Needed.}
% %\textbf{Misunderstanding the Requirements.}
% By avoiding training accuracy measurements, researchers may be totally unaware of the mistakes in their code. That said,  many works also avoided implementing the backward kernels altogether.
% %Moreover, we also suspect that the domain knowledge of deep learning, such as GNN, has different learning goals then let us say graph data analytics domains. 
% %Back-propagation creates requirements that impacts the forward computation, and may limit what kernels can be fused, and dictates the content of graph storage. 
% %hence performance benchmarking just the forward computation can be erroneous. As we saw in case of Huang et al~\cite{huang2021understanding}, it compared against DGL's GAT, but its graph neither had edge ID, nor did it explain how to do back-propagation of the giant single kernel that it implemented by merging all the kernels in the forward direction for GAT.
% It is possible that they may be unaware of DL/GNN nuances, specifically about the need for state tensors, and hence did not take care of this additional restriction while optimizing the forward computation. 
% Unfortunately, we really do not have end-to-end assignments to teach such requirement gathering and plugging the developed code base to an end-to-end training system. For instance, Many deep learning systems courses~\cite{dlsCMU, cs15884CMU, cse599wWashington,cs231nStandford} at reputable universities have assignments for forward computation of an operation, and in Python only. 
% %Students may not learn end-to-end requirement gathering from such assignments. 

\section{ {\graphpy}: Use Cases and Overview} \label{sec.usecase}

%\subsection{Use-Cases}  \label{sec.usecase}
%We presented a number of observations for a single GPU GNN system. 
%\textbf{Use Cases.}
{\graphpy} focuses on two use cases, which are very clear by now: 1) a platform to integrate the GNN system to a DL framework to enforce  end-to-end model prototyping and accuracy measurement; and 2) in-depth focus on correct requirement gathering beyond the state tensor requirement to understand the memory footprint and performance opportunities. We first introduce the issues faced by prior works when handling these use cases which motivates the need for {\graphpy}.
%We use \textit{Kernel} to mean the module that contains systems code.
%while \textit{Workflow} module wraps the Kernel module to make it available to data scientists in Python. It invokes low-level CUDA kernels.
%We focus on two aspects, passing tensors and graph objects.


%actionable items are very clear: (a) complete GNN model implementation is needed to accurately capture the accuracy and performance that can help justify the proposed optimization techniques and make researchers aware of DL/GNN nuances, such as the need for state tensors. (b) We need to understand the source of huge memory consumption and focus on developing a new baseline that can allow us to easily train various GNN models on larger datasets. 

%The majority of the prior works have focused on class A GNN only, leaving the entire class B models out, hence a system with diverse models is needed. 
%This observation along with issues with prior works makes DGL the only baseline that can be used for performance comparison on both the classes of GNN.


\subsection{Use-Case\#1: A Platform for GNN Research} 
%A complete GNN model implementation is needed to capture the accuracy and performance that can help justify the proposed system optimization and make researchers aware of GNN nuances, e.g., the need for state tensors.
We analyze DL frameworks and DGL for their integration capability and explain their limitations or productivity issues.
%which makes while integrating system optimization into a DL framework.

\subsubsection{DL Framework's Plugin Architecture}
We analyze the system API between the DL framework and the GNN system  to study their interface-level limitations.
We first study the PyTorch plugin which is used by many prior works~\cite{fu2022tlpgnn,wang2021gnnadvisor,huang2021understanding,pytorchg2019} to implement their GNN system. 
%to figure out the complexities in the integration.

%There are many challenges in using these  approaches because of their restrictive programming environment, framework and its version dependency, and unclear documentation.
%which make {Kernel} highly dependent on PyTorch environment and its specific version, which does not allow sharing the Kernel code with other DL frameworks, while necessitating the compilation process for each major version of the same DL frameworks. Further, the plugin provides very restrictive environment for development that limits how we pass the tensor and data to during kernel invocation. We explain its implication below.
%becomes impossible and also increase the difficulties and complexities of implementation.

%and therefore how to provide the tensor support to the underlying {Kernel} becomes a new problem because a good design should make the {Kernel} module truly independent. We categories the existing approaches into three ways.



\noindent \noindent $\bullet$
\textbf{TensorFlow Analysis.}
While we did not perform the same in-depth analysis on TensorFlow, a high-level study clearly indicates that its plugin also restricts passing custom objects, unless additional steps are performed using its \textit{experimental.extensionType} plugin, which is conceptually similar to the smart pointer approach of the PyTorch plugin. Hence, many prior works~\cite{graphnets,spektral} use COO format in TensorFlow.

%LibTorch's restrictive interfaces, the need for a captive graph storage preparation, and other workarounds result in non-productive efforts for integration tasks, and the researchers may get exhausted. Ultimately, the experience discouraged us to use these approaches to design programming exercises in the graduate-level course. 
 
%Actually, we keep encountering new errors including run-time errors that cost us a lot of time to debug, but the fixes were not genuine bug fixes but needed a better understanding of the interface limitation and special conventions that are not very explicit in the documentation.
%Based on these observations, although the two approaches are very related, these two have similar issues. The developments which use these two ways need to implement the Workflow and Kernel for each DL framework separately as well as each major version separately. They also need to follow an ad hoc method to handle the graph object. 


\subsubsection{DGL Integration} \label{sec.dgl}
%\textbf{Custom Kernel and Requirement Mismatch.} 
%Most systems~\cite{gespmmsc2020,featgraphsc20}\td[more citation] that integrate their system works to DGL have not performed any kernel fusion. 
DGL has no documentation on system integration. 
Hence prior works have followed different approaches. 
%and we could run two popular works of GE-spMM~\cite{gespmmsc2020} and FeatGraph~\cite{featgraphsc20} end-to-end.
GE-SpMM~\cite{gespmmsc2020} provides the source code files to replace the same-named DGL source files. However, those named files are now  missing in DGL due to its complete code re-organization, a trait of a monolithic system. Further, the DGL code-base has included one such file\footnote{\scriptsize \url{https://github.com/dmlc/dgl/blob/master/src/array/cuda/ge_spmm.cuh}} but did not integrate it. Our integration and evaluation revealed functionality bugs with this code. Hence we did not proceed with it.
We also could not run FeatGraph~\cite{featgraphsc20} end-to-end despite trying many GitHub branches as suggested by their authors (see appendix for our communication), though it is officially integrated by DGL using a compile-time flag. So, questions remain on the modality of integration.
%though they claimed that the proposed techniques have been integrated into DGL's own kernels.
%while we have not encountered any prior work that has written a custom interface in DGL. 

\noindent \textbf{Amount of Modification Needed.}
DGL offers one generic system API each for gSpMM and gSDDMM interface to the DL framework. So any attempt at kernel fusion needs a \textit{custom system API}, and almost full re-write of the DGL backend including the new fused kernels. 
Further, supporting a custom graph storage needs to change many public system APIs of DGL, such as \textit{successors()} and \textit{predecessors()}, which are not even used by GNN systems. An advanced system researcher may be able to understand and modify the internals and APIs completely despite the absence of integration-related and backend documentation.
However, DGL integrated systems~\cite{gespmmsc2020,featgraphsc20} have not even fused obvious kernels of gSpMMv and normalization by degree. 


%the way we understood advanced features of PyTorch to pass graphs as a custom object using the smart pointer approach\footref{foot.time}.  
%Then, they can prototype a custom kernel and can support custom graph storage.
Moreover, spending additional effort may be of no use if the whole backend and system APIs need to be replaced. History indicates that such types of optimization works~\cite{huang2021understanding,wang2021gnnadvisor,fu2022tlpgnn,spektral} have rather relied on plugin environment, developed their own model code, system APIs, and system code despite the interface-level limitation.
We reached out to some authors of GNN papers to understand why they did not use DGL. 
One of the authors of a prior GNN system aptly described the limitations of working with DGL: \textit{``We didn't use DGL, because some of its design is inefficient but is also embedded in the system design in a complex way''} %\footnote{Personal communication using email}, 
confirming our observation on using DGL. 
%for GNN system optimizations. 
%This response points towards the complex monolithic design that does not encourage innovations in custom storage format or kernel fusion. 

% allows prototyping of the system idea easily.
%We now study if DGL can be used productively to support system integration of GNN optimizations, and presents the following challenges.
%It has neither advertised that is a tool for \textit{systems} research and education nor has any documentation to aid in integrating systems work to it. Clearly, integration with DGL requires additional effort in understanding its back-end system design and code base. 
%Additionally, DGL suffers from two critical limitations if it is used for performing system research.
%In absence of documentation on integrating different systems to DGL, researchers have taken an approach based on its code-study, and success do have been reported~\cite{gespmmsc2020,featgraphsc20} \td[more citation]. However, 
%DGL is a monolithic system,   
% The official DGL integrated code of FeatGraph~\cite{featgraphsc20} (hosted by DGL) has not implemented graph partitioning as described in the original paper.
% %is not exactly a framework designed with systems research and education in mind.
% %DGL internally prepares CSR/CSC format with an edge ID as its fixed edge property irrespective of whether needed or not, and 
% DGL is a monolithic system that supports a variety of APIs on graph objects, such as \textit{successors()} and \textit{predecessors()}, whose implementation will involve  additional effort if a custom graph storage is implemented which is not useful when the aim is just kernel optimization through a better storage format.
% %Hence DGL integrated systems either use or force to use vanilla CSR/CSC format for integration purposes unless all the APIs are correctly implemented.
% Not implementing these APIs will leave the whole DGL code in a broken state due to its monolithic nature.
%implying that the monolithic nature may reject merging other past and future research if it involves storage format change.
% Similarly, GE-SpMM~\cite{gespmmsc2020} is CSR/CSC based GNN system to be integrated into DGL.




\subsection{{\graphpy} Overview} \label{sec.overview}


%\noindent \textbf{Motivation.}{\color{red}
% There are many similarities in traditional graph analysis and modern graph data science as both aggregates the features of neighboring vertices to update the feature of the vertex. 
% Hence, prior system-level optimization techniques such as specific tailored data layout~\cite{zhang2015numa,gstore,libgraplus15DB}, graph-aware compression~\cite{libgraplus15DB,gstore}, fine-grained and workload-aware parallelism~\cite{liu2015enterprise,wang2015gunrock}, graph reordering~\cite{gorder16sigmod,rabbit16ipdps}, graph partitioning, etc. may be applicable to DL use-cases also. 
% However, none of these prior works are extended to DL use-cases because the DL use-cases need to integrate many DL-specific components, such as computation graph, and tensor management. 
% Therefore, there is a gap between the traditional graph analysis and DL use-cases. 

% Though, this paper discusses graph use-cases, the problem is more generic in nature, as we explain about the critical interfaces that allows plugging system research (e.g., kernel optimization) back to an end-to-end DL training is very complex today. The problems that we encountered while plugging our reference GNN kernel implementation were many including unclear documentation, introduction of additional efforts due to critical thinking in the integration part (not in kernel implementation), and huge dependency with third party tensor library, such as Pytorch that limits the usage of the developed kernel to the other DL framework, etc. We discuss them in detail in next section.

% Moreover, we realize that existing GNN systems are either hard to modify or limit to a specific DL framework backend. For example, DGL, PyG implement their tensor management during kernel computation directly, which increases their module dependency and makes their code hard to modify. (Not sure whether this is True TODO)
% GNNAdvisor\cite{GNNAdvisor} only works for the Pytorch backend and its kernel codebase cannot be reused for other DL framework backends, such as Tensorflow and MXNet\cite{mxnet2015}. 
% Based on this observation, there is a need for a kernel-independent and backend-independent platform which can let researchers prototype new system-level ideas for DL-specific use-cases easily. 
 
% We also observe that there is a synergy and ease-of-use in bringing the diverse graph data science use-cases together within the Python environment, as many of them may be performed together, or there are many common tasks among them, such as preparing graphs from raw data, writing Python binding, and handling tensors. 
% For example, DL applications also require some of the traditional and ad hoc graph analysis. GraphSage~\cite{graphsage17} does sampling or community analysis to downsize the graph when preparing the dataset for deep learning. 
% It also performs connected component analysis and does the union of a few components to get the representative dataset. 
% Performing these from Python environment is needed, but having a high-performance back-end will provide faster execution to all the tasks. Unfortunately, there is no high-performance back-end supporting arbitrary multi-field edge properties.
 
 
% On the other hand, educating the next generation of system researchers on deep learning requires a modular-based and easily modified platform, something similar to the small code base of XV6 Operating System. that is used to train undergraduate students on Operating Systems. Our work is motivated by this fact that one case use Linux for practical hands on and coding assignments for teaching OS, we have observed that many universities prefer small operating systems such as XV6 in undergraduate courses.

%}

% We show that a system researcher can easily take advantage of {\graphpy} to modify or re-write kernel implementation to learn the system level ideas in deep learning. 
% As we explain, this platform is not just useful for deep learning on graph, but can be extended easily for other domains including for dense linear algebra.


% faces many challenges, specifically (a) how to design interfaces in a simple and extensible way that can be taken out of critical learning path from system researchers or learners; (b) how to pass tensors to kernel code using zero-copy for read and write (\cref{sec.science}) as tensors are very specific data structure of each DL framework, while their conversion to NumPy arrays results in data copy, therefore cannot be used as a mechanism; (c) how to support arbitrary multi-field edge properties seamlessly across Python and C++ which is required to support diverse graph data science applications.



%{\td add how to view it from education view}
%Both of these use cases are related, the first one explores the high-level interfaces between data science and GNN systems, and the second one explores the low-level interfaces between the system framework and the actual kernel of GNN systems.

\noindent \textbf{The Platform.}
{\graphpy} provides a productive platform for the integration of GNN systems to DL frameworks for end-to-end model prototyping. The architecture is shown in Fig.~\ref{fig-arch}.
We make {\graphpy-GNN} fully \textit{independent} of the DL framework to which it is integrated by using the proposed \textit{Half DLPack protocol}.
The independence allows system APIs of {\graphpy-GNN} to support all the custom classes that are possible between Python and C++. 
%therefore it has no interface-level limitations.
%Hence, by modeling graphs as a custom object, its interfaces do not require any change when the underlying graph storage format changes. 

Moreover, \textit{{\graphpy-SM}} supports multi-field graph edge properties to offer diverse graph storage needs of both GNN classes. It prepares CSR/CSC graphs from the raw data and exports them using zero-copy Python Numpy arrays to support multi-field graph edge properties. This allows us to support edge ID for class A GNN models. {\graphpy-GNN} can directly convert the NumPy array to any custom format or simply wraps them to return a kernel-graph object (\textit{g}) that can be used in follow-up system API calls (Table~\ref{table-kernel}). 
%We are unaware of any system that can support arbitrary multi-field edge properties. It also cannot be designed without significant innovations.

Taking advantage of these mechanisms, \textit{\graphpy-Workflow} integrates the same {\graphpy-GNN} with PyTorch and TensorFlow. 
Moreover, system integration codes are automatically generated by specifying the API signature using a simple DSL. 
These APIs require changes only when fusion is attempted on system APIs, and not for any storage format changes, which can be regenerated again.


%In any case, the generation of integration code makes end-to-end system development productive without any workaround. 


%and hence any third-party graph analytics tools can take this boilerplate code, and provide the kernel implementation.

\begin{figure}[t]
\includegraphics[scale= 0.4]{result/overview.pdf}
\vspace{-12pt}
\caption{\small {\graphpy-GNN} is an independent module, hence no interface limitations exist thanks to {\graphpy-Workflow} that provides integration to DL frameworks in a framework agnostic way.} 
  %{\graphpy-SM} prepares graph.}
  \label{fig-arch}
%   \vspace{-12pt}
\end{figure}

%To support arbitrary vertex and edge properties of any size or custom structure, {\graphpy} utilizes \textit{Numpy Dtype}. Its C++ back-end has a generic infrastructure that allows supporting almost arbitrary, multi-field properties once deployed. 

\noindent \textbf{\graphpy-Kernel}.
{\graphpy} internally defines and designs GNN-specific kernels, e.g. in CUDA, which are directly invoked by {\graphpy-GNN} APIs (Table~\ref{table-kernel}) to avoid the requirement mismatch. 
Hence, the proposed internal CUDA kernel signature follows a similar signature as the system API to directly map the requirements. This was needed to show that avoiding the generalization cost of prior kernel design can save memory and gain performance.
For example, 
gSpMMveid invokes just one kernel that directly expects a graph with edge ID to avoid the need for a separate eShuffle CUDA kernel and never generates additional intermediate results.
Similarly, \textit{gSpMMv} system API invokes a kernel definition that does not need any dummy edge-level tensors and supports normalization by degree as an option. 




% \begin{table}[ht]
% \caption{Comparison between different graph analytic systems} % title of Table
% \centering % used for centering table
% \begin{tabular}{c c c c} % centered columns (4 columns)
% \hline
% \hline %inserts double horizontal lines
% Graph  & Python & GNN & Graph Data \\ %[0.7ex]
% Systems & APIs & operations & Engineering \\ %[0.7ex]
% %heading
% \hline % inserts single horizontal line
% NeuGraph &  & + &  \\ % inserting body of the table
% DGL & + & + & \\

% NetworkX &  &  & + \\ 
% Graphone &  & + & \\
% {\graphpy} & + & + & + \\ 
% [1ex] % [1ex] adds vertical space
% \hline %inserts single line
% \end{tabular}
% \label{table:nonlin} % is used to refer this table in the text
% \end{table}




% To let the data scientist use it easily, we wrapped these core functions out to python. By combining the python wrapped graph data structure, Pytorch framework, and the tensor operations, data scientists and machine learning engineers can treat and use the {\graphpy} as a normal python package. 
% By using these wrapper core functions, users can write their own graph DL algorithm if they want. {\graphpy} also provides some pre-implemented graph DL python modules, GCN, GAT. 

%Though performance is an important metric that we would be striving for, we argue that memory overhead is equally important to enable training on larger datasets using one GPU. This will minimize the need for more GPUs  to save energy and resources while not forcing a distributed deployment unless necessary which has its own learning curve. because a new optimized baseline requires system integration to a DL framework to evaluate GNN training for accuracy and performance.


%{\graphpy} makes system integration simple and productive, and can be used for extensive research as system researchers can independently think and implement any idea rather than critically thinking about workarounds. 

\noindent \textbf{Applicability.}
Beyond research, we have already used {\graphpy} to teach end-to-end GNN systems to a graduate class, and the response was overly positive, where students fully understood and gathered complete system requirements with focusing on forward and backward computation both.
In comparison, publicly listed assignments on DL/GNN \textit{systems} courses offered by other universities~\cite{dlsCMU, cs15884CMU, cse599wWashington,cs231nStandford} \textit{focus only on the forward kernel} of an operator, and in Python without its integration in an end-to-end DL/GNN system. 
We see {\graphpy} as a general-purpose DL \textit{systems} education and research tool due to innovations in interface design and automatic system integration as its interfaces are independent of graphs. Through this paper, we plan to popularize the tool and will be open-sourcing the developed education material. 
%We also developed another module fully dedicated to traditional graph analytics use cases, such as BFS, Connected Component, PageRank, etc. to show that {\graphpy-SM} is useful beyond GNN. 

% To demonstrate the extensibility, we have implemented the sparse tensor which results during weight pruning~\cite{han2016iclr} the fully connected layer. In this case, the tensor itself is sparse and not the data. So the model retraining, which is needed after weight pruning, requires a graph object to be associated with the tensor. 
%\noindent \textbf{A Possible Teaching Tool.}
%It also benefits teaching by empowering students to integrate their kernel prototype with a negligible effort so that they can understand the end-to-end system. 
%E.g., 

%Hence, students cannot fully understand, appreciate, and gather complete system requirements without focusing on its backward kernel. 
%Rather, industry partners have voiced concern about the availability of candidates with good systems and data science knowledge in an NSF workshop~\cite{storage2025NSF}.


%and evaluated the claim yet, we remain committed to it.

%We also argue that {\graphpy} or its components  can be used by any graph data science applications. For example, 
{\graphpy-SM} can support graphs with arbitrary edge properties, so we were able to use it to pass the graph across many systems that we evaluate: GE-SpMM~\cite{gespmmsc2020}, GNNAdvisor~\cite{wang2021gnnadvisor}, FeatGraph~\cite{featgraphsc20}, Huang et al~\cite{huang2021understanding}, and CuSparse.  We expect that it can be used with other graph data science applications as well.

% Further, we auto-generate all the boiler-plate code where a 
%To extend the system, one only needs to provide the specification for a new kernel using the proposed DSL. 


%Hence, {\graphpy} will help in advancing the state-of-the-art in deep learning \textit{systems} in general and GNN \textit{systems} in particular, while correctly training the future generations of systems engineers. 


% Overall, {\graphpy} has great promise for graph data science \textit{systems} education and research due to its smaller code-base size, auto-generation of the critical system integration code, and {\graphpy-GNN's} independence of any third-party tensor library or memory management. 


%The data scientist can directly import {\graphpy} components and use it to perform many graph data science use-cases in Python.
% Being a purely Python module, the {\graphpy-Workflow} is flexible and easy for data scientists to modify it or add new Python code for new customized graph DL models or otherwise.

% We believe it can be extended as the educational platform for other deep learning domains, e.g. computer vision, which we leave as future work.
% though it remains a work in progress. 

% Works done on higher level sparsity~\cite{graham2015sparse, graham20183d,notchenko2017large,wang2019efficient}, do not have system-level support yet. {\graphpy} has only focused on two dimensional sparsity that can easily be represented using graph data model. However, {\graphpy} can be extended in the future to provide that support.





==> tex/related.tex <==
\section{Related Work} \label{sec.related}

% \subsection{Traditional graph analysis system}

\noindent \textbf{Static Graph Analytics System.}
Traditional graph analytics systems focus on creating graph representation and performing traditional graph analysis. Some works \cite{roy2013x} \cite{liu2017graphene,powerlyra2015eurosys,gstore, nguyen2013lightweight,
zheng2015flashgraph,mosiacEuroSys17, roy2015chaos, han2013turbograph, kumar2017falcon, zhu2015gridgraph,hong2012green, wu2015g, ai2017squeezing, zhu2016gemini,liu2015enterprise} 
can only support the graph topology analysis on the static graph. These works pre-process the raw input data to create the graph representation and then perform the graph topology analysis. None of them, are able to support arbitrary edge properties. They allow at max one additional field for edge weights.

\vspace{1mm}
\noindent \textbf{Dynamic Graph Analytics System.}
Grace~\cite{grace12atc}, LLAMA~\cite{macko2015llama}, Stinger~\cite{ediger2012stinger}, Graphone~\cite{kumar2017graphone,kumar2020graphone}, Aspen~\cite{dhulipala2019low} can support dynamic graph but it is implemented mainly in C++ and did not provide any wrapped python APIs. Further, except GraphOne, others does not provide arbitrary edge properties. Moreover, GraphOne uses template meta-programming to support arbitrary edge properties, however it is almost impossible to enable python binding for arbitrary edge properties. {\graphpy-DE} fixed this gap between C++ and Python, and also took advantage of the fact that it has to support only static graphs. Hence, provides many new optimization that does not require the data consistency support.

\vspace{1mm}
\noindent \textbf{Python based Graph Analytics System}. NetworkX~\cite{networkx08} is a popular python based graph system. However, it is very slow due to its purely python based implementation. We believe that {\graphpy-DE} can become a back-end to take advantage of the huge analysis code-base of NetworkX.

\noindent \textbf{Graph Neural Network (GNN)} system, such as DGL~\cite{dgl2019}, NeuGraph~\cite{neugraph19atc}, Pytorch-Geometric~\cite{pytorchg2019} perform deep learning on graph data. DGL \cite{dgl2019} is an open-source,  DGL is a monolithic GNN framework, and, and supports only a limited set of graph preparation, and does not export the graph representation to third party module, so it is hard to quickly prototype any new system idea. It also does not support bipartite graphs, hence it cannot support sparse models.
% purely c++ implemented graph deep learning system. 
NeuGraph is a not open-sourced, and does not support attention based models such GAT. Pytorch-Geometric is tightly integrated with Pytorch~\cite{pytorch2019}. Hence, integrating new system design involves huge efforts.

Although these works support graph deep learning features, data scientists need to pre-process the raw input data themselves. It is not clear how will they convert the raw string identifier to a numeric vertex ID in such cases. Possibly, they force the data-scientist to do more ad hoc processing.  
% to create the graph representation themselves. 

% On the other hand, {\graphpy} is a full-fledged systems for complete data-science need on graph like data, including graph preparation from raw-data in parallel and high-performance way, traditional graph analysis, and graph deep learning. Moreover, it export the internal graph data as numpy arrays, on which any ad hoc graph analysis including graph deep learning can be performed.  
